RoVaR: Robust Multi-agent Tracking through Dual-layer Diversity in Visual and RF Sensor Fusion

The plethora of sensors in our commodity devices provides a rich substrate for sensor-fused tracking. Yet, today's solutions are unable to deliver robust and high tracking accuracies across multiple agents in practical, everyday environments - a feature central to the future of immersive and collaborative applications. This can be attributed to the limited scope of diversity leveraged by these fusion solutions, preventing them from catering to the multiple dimensions of accuracy, robustness (diverse environmental conditions) and scalability (multiple agents) simultaneously. In this work, we take an important step towards this goal by introducing the notion of dual-layer diversity to the problem of sensor fusion in multi-agent tracking. We demonstrate that the fusion of complementary tracking modalities, - passive/relative (e.g., visual odometry) and active/absolute tracking (e.g., infrastructure-assisted RF localization) offer a key first layer of diversity that brings scalability while the second layer of diversity lies in the methodology of fusion, where we bring together the complementary strengths of algorithmic (for robustness) and data-driven (for accuracy) approaches. RoVaR is an embodiment of such a dual-layer diversity approach that intelligently attends to cross-modal information using algorithmic and data-driven techniques that jointly share the burden of accurately tracking multiple agents in the wild. Extensive evaluations reveal RoVaR's multi-dimensional benefits in terms of tracking accuracy (median of 15cm), robustness (in unseen environments), light weight (runs in real-time on mobile platforms such as Jetson Nano/TX2), to enable practical multi-agent immersive applications in everyday environments.

==> abstract.tex <==
The plethora of sensors (both visual and RF) in our commodity devices provides a rich substrate
for sensor-fused tracking. Yet, today's solutions are unable to deliver robust and high tracking
accuracies across multiple agents in practical, everyday environments -- a feature central 
to the future of immersive and collaborative applications.
This can be attributed to the limited scope of diversity leveraged by these fusion solutions, 
preventing them from catering to the multiple dimensions of {\em accuracy}, {\em robustness} 
(varied environments) and {\em scalability} (multiple agents) simultaneously.\\
%Future immersive and collaborative applications on our smart devices will significantly benefit from the ability to robustly and accurately track multiple devices simultaneously  in everyday environments. While the plethora of sensors (both visual and RF) in our devices, provides a rich substrate for sensor-fused tracking,  today's solutions are yet to deliver robust and high tracking accuracies across multiple targets (agents) in everyday environments that are plagued with both sensor noise and environmental artifacts.  This can be attributed to the limited scope of diversity leveraged by these fusion solutions that prevents them from catering to the multiple dimensions of {\em accuracy}, {\em robustness} (various environments) and {\em scalability} (multiple agents) simultaneously.      
%In this work, we take an important step towards this goal by introducing the notion of {\em dual-layer diversity} to the problem of sensor fusion in multi-agent tracking. 
%We demonstrate that the fusion of complementary tracking {\em modalities}, namely passive/relative (e.g. visual odometry) and active/absolute (e.g.infrastructure-assisted RF localization) tracking, offers a key first layer of diversity to provide accurate tracking across multiple agents, but often comes at the expense of robustness, i.e. degraded performance in new, unseen environments. Delivering robustness without sacrificing tracking accuracy, in turn requires another layer of diversity in the {\em methodology} of fusion, where we bring together the complementary strengths of algorithmic (for robustness) and data-driven (for accuracy) approaches. \system is an embodiment of such a dual-layer diversity approach that enables light-weight, real-time sensor fusion. Its design elements bring together the complementary benefits of RF (UWB) and visual (stereo cameras) tracking through an intelligent combination of  algorithmic and data-driven techniques that jointly share the burden of accurately tracking multiple agents in the wild.  Extensive evaluations reveal its multi-dimensional benefits over prior art that employ a single layer of diversity.  

In this work, we take an important step towards this goal by introducing the notion of dual-layer 
diversity to the problem of sensor fusion in multi-agent tracking. We demonstrate that the fusion
of complementary tracking modalities, namely passive/relative (e.g. visual odometry) and active/absolute
(e.g.infrastructure-assisted RF localization) tracking, offers a key first layer of diversity to 
provide accurate tracking across multiple agents, but often comes at the expense of robustness,
i.e. degraded performance in new, unseen environments. Delivering robustness without sacrificing 
tracking accuracy, in turn requires another layer of diversity in the methodology of fusion, where 
we bring together the complementary strengths of algorithmic (for robustness) and data-driven 
(for accuracy) approaches. \system is an embodiment of such a dual-layer diversity approach that enables 
light-weight, real-time sensor fusion. Its design elements bring together the complementary benefits 
of RF (UWB) and visual (stereo cameras) tracking through an intelligent combination of algorithmic 
and data-driven techniques that jointly share the burden of accurately tracking multiple agents in the 
wild. Extensive evaluations reveal \system’s ability to achieve median tracking errors < xxcm in 
real-time far exceeds prior art that employ a single layer of diversity.



==> background-related1.tex <==
\subsection{Background and Related Work} \label{label:background}
Current solutions used for tracking and localization can broadly be 
categorized as either active or passive. 
\subsubsection{Active Tracking}
Infrastructure assisted active tracking techniques use one or more 
pre-deployed anchors at known locations to localize a UE. Distances
from the UE to each anchor is individually estimated and subsequently
these estimated ranges (to at least 3 anchors) are combined using multilateration techniques~\cite{}
to determine the UE's absolute location. Accuracy of such anchor-based tracking schemes
depend entirely on the accuracy of the individual distances estimated. Consequently, 
researchers in the past have proposed a plethora of solutions that leverage 
optical (e.g., IR beacons~\cite{}, VLC~\cite{}), acoustic (audible and ultrasound) or RF technologies 
to estimate distances between two devices. However, while optical based solutions are
limited to only LoS locations, acoustic signals are sensitive to ambient noise~\cite{}, 
propogation material~\cite{} and environmental conditions (e.g., temperature, humidity etc.) and require
complex signal processing techniques to process the received signal. Relatively,
RF signals are more robust in indoor locations, and consequently researchers have proposed 
solutions using various RF technologies like WiFi~\cite{}, Bluetooth~\cite{}, mmWaves~\cite{} 
and UWBs~\cite{}. The mmWaves and UWBs, compared to WiFi and Bluetooth use wider channels, and
hence are capable of providing more accurate (centimeter-level accuracy) ranging estimations (\S\ref{sec:tracking-mod}). 
However, the UWBs possess more object penetrability than the mmWaves, making them more
apt for indoor tracking and localization. 

\subsubsection{Passive Tracking} 
Passive tracking are odometry based solutions that do not require any pre-deployed infrastructure.
Visual and inertial odometry solutions are perhaps the most popularly 
used passive tracking techniques. 
Visual Odometry (VO) algorithms (e.g., SFM~\cite{}, VSLAM~\cite{} etc) use a stream of 
camera images to track the motion. Changes in texture, color, shape (a.k.a image features) in successive 
camera images of a static environment 
are sufficient to track the motion. Although VO can potentially offer
high precision tracking (cm scale granularity), often in indoor locations due to either poor lighting, 
lack of texture or due to perceptual aliasing coditions~\cite{}, VO's accuracy can signficiantly degrade. Inertial odometry 
is thus used as an auxillary data source to the VO, to improve tracking accuracy. 

\emph{Visual Simultaneous Localization and Mapping (vSLAM)} algorithms like 
ORB-SLAM~\cite{}, RTABMAP-SLAM~\cite{} implement VO in realtime.  
These algorithms continuously localize a UE within an environment while incrementally 
constructing and updating the map of that environment. The environment maps are 
subsequently used to correct the VO drifts via loop closure detection~\cite{} 
and bundle adjustment optimizations~\cite{}. vSLAM based VO solutions are currently
used widely both in academia~\cite{} and industry~\cite{}.

\subsubsection{Choice of tracking techniques:}
\label{sec:tracking-mod}
In this work, we use UWBs for active tracking while using ORB-SLAM3~\cite{} 
vSLAM-algorithm for passive tracking. 

\emph{UWB based active tracking:} The graph in Fig.~\cite{} shows the accuracy of 
UWB ranging in LoS and NLoS locations. In LoS,
UWB's two-way-ranging~\cite{} provides median range errors of only {\color{red}XXcm} upto 30m. However, in  
NLoS the maximum distance UWBs can range reduces signficantly to 20m and the errors
in range estimates increase to {\color{red}YYcm}, specially for distances > 20m. Nonetheless, the UWBs
are still relatively more accurate than other RF modalities for indoor tracking (see table~\ref{}). 

\emph{ORB-SLAM3} (built upon ORB-SLAM2~\cite{} and ORB-SLAM~\cite{}) is a feature based vSLAM algorithm,
robust to motion clutter and can work with monocular,
stereo or RGB-D images. The ORB-features~\cite{} are easy to extract and allow for fast matching 
across camera frames enabling the algorithm to implement realtime VO based tracking. 
ORB-SLAM3 is the first vSLAM algorithm able to perform multi-map
SLAM with monocular, stereo and RGB-D cameras, using pin-hole andfisheye  lens  models. Previous
studies~\cite{} show that ORB-SLAM algorithms can outperform other popular realtime SLAM algorithms
like RTABMAP-SLAM in odometry detection. Our own evaluation (Fig.~\ref{}) shows that ORB-SLAM3 can
perform signficantly better than commercial VO implementation like ARCore~\cite{} when it comes to
trajectory and odometry detection. 

Lidar based SLAM algorithms (e.g., cartographer slam~\cite{}, GMapping~\cite{}) work similar to vSLAM 
algorithms taking in lidar streams as input. However, unlike outdoor lidars (e.g., Velodyn lidar~\cite{}) which are
heavy, expensive and require huge data processing computations, indoor lidars~\cite{} (and cameras with 
depth sensors, e.g., Intel lidar cameras~\cite{}) are lightweight with depth estimation
capability of upto only a few meters (e.g., 5m for Intel lidar cameara). 
Performance of these sensors degrade considerably in large indoor spaces (see Fig.~\cite{}) affecting the
SLAM algorithms' performance as well.

\begin{table}[t]
  \centering
     \caption{Choice of Passive Tracking solutions.}
  \begin{tabular}{|l|c|c|c|}
  \hline
      \textbf{ } & \textbf{Mean} & \textbf{Std} & \textbf{Max} \\
    \hline
    %\hline
    Phone Camera &  &        &  \\ \hline
    Realsense T265 & &   & \\ \hline
    Depth camera &  &   &  \\ \hline
    Lidar & & & \\ \hline
  \end{tabular}   \label{tab:choiceofpassivetracking}
\end{table}
\begin{table}[t]
  \centering
     \caption{Choice of Active Tracking solutions.}
    \begin{tabular}{|l|c|c|c|c|}
  \hline
      \textbf{ } & \textbf{Mean} & \textbf{Std} & \textbf{Max} & \textbf{Range} \\
    \hline
    %\hline
    LTE &  &    &    &  \\ \hline
    WiFi & &  & & \\ \hline
    UWB & & &  & \\ \hline
    mmWave &  & &  &  \\ \hline
  \end{tabular}   \label{tab:choiceofactivetracking}
\end{table}


\subsection{Motivation - Case for a hybrid approach:}

\subsubsection{Accuracy Vs. Robustness:}
VO provides high precision (cm-scale granularity) tracking, but
is vulnerable to aggressive motions (e.g., running, hopping etc)~\cite{} and 
adverse environmental conditions. On the other hand, RF ensures 
robust active tracking but can only afford coarse location accuracy.
The Fig.~\ref{} (above) shows ORB-SLAM3 and UWB's performance
for a simple trajectory, part of which is dimly lit (adverse to ORB-SLAM), 
and part of it contains NLoS anchors (adverse to UWB). The error graph shows the
individual errors for the two methodologies. While ORB-SLAM3's VO performs exceedingly
well in well-lit areas, it starts accumulating errors as the user navigates
through dim-lit areas. Due to the nature of the odometric solution, the VO errors
propogates across the trajectory even when the user navigates through the well-lit areas,
until the algorithm detects as loop and corrects the drift. The UWB has the luxury
of localizing the user afresh each time ranging occurs, and hence does not carry forward
the errors that accumulate in the region of NLOS anchors. However, the granularity of 
the localization itself is at sub-meter scale, which is significantly higher than
the finer (cm-scale) granular tracking VO provides in well-lit ideal conditions.
An effective fusion (see error graph between time XXsec - YYsec) between the two 
can potentially bring complementary benefits to deliver a robust system that 
is capable of high-precision tracking.

%\subsubsection{Case for a Hybrid Approach} \label{label:hybridcase} Results to motivate
%deficiencies of isolated passive and active tracking approaches. 
%As discussed in (\S \ref{label:background}), there have been several recent 
%tracking solutions (active and passive) proposed in the research literature with a goal 
%towards achieving a fine-grained cm-scale tracking~\cite{}. Active tracking such as RF 
%(UWB in our case)-based solutions deploy a set of anchors in the environment, with users
%carrying a tag. A two-way ranging protocol is used to estimate the distance between the 
%tags (i.e., users) and the anchors, and localize the user with a multilateration algorithm
%from the measured ranges. State-of-the-art ranging methods provide up to a cm-scale ranging
%under specific conditions such as when most of the anchors are in line of sight (LOS) of the tracked
%users. However, the ranging can be noisy in case of a subset of anchors are under non-line-of-sight
%(NLOS) of users, consequently resulting in poor tracking accuracy under such conditions. 
%Figure \ref{fig:nlosvsranging} quantifies the ranging accuracy under LOS and NLOS for a single
%anchor and single tag in the UWB 6GHz band. Figure shows that, as the user moves far from the anchor
%in LOS, we find the ranging is consistent until 30m distance with a maximum of XX standard deviation. 
%Whereas for NLOS, the noise as high as YY within 20m and reaches to physical limitations of signal 
%propagation going out of range thereafter. As we show later, such noise in range measurements from 
%NLOS anchors can decrease the tracking accuracy by ZZ when compared with all anchors in LOS.
%Similarly, the passive tracking such as VO-based solutions exhibit such deficiencies while 
%providing a sub-centimeter level tracking accuracy under good environmental conditions. These 
%passive tracking solutions are primarily feature-based methods i.e., from the images captured 
%from the environment, similar features are estimated in consecutive images and the relative motion 
%is estimated from one image to another. Because of this dependence on features of consecutive images, 
%the tracking can fail if there are sudden changes or very few key features in the environment. Best 
%known such examples are--- lighting conditions, plain feature-poor environment (e.g., white walls),
%random motion (running or quick jerky motion in case of games), etc. Figure \ref{fig:vo-limitations} 
%shows a qualitative example trajectory with the VO tracking under bright and dim light conditions. 
%As shown, the tracking under bright-light light consistently follows the ground-truth trajectory, 
%the dim-light trajectory is off by almost XXm. The problem becomes more acute when the tracking is 
%under combined adverse conditions such as running with random motions under dim-light environment. 

\begin{figure}[t]
\centering
        \subfloat[RF]{%
      \includegraphics[width=0.5\linewidth]{figs/range-accuracy-los-nlos-exp.png}\label{fig:nlosvsranging}
     }
        \subfloat[VO]{%
      \includegraphics[width=0.5\linewidth]{figs/vo-perf.png} \label{fig:vo-limitations}
     }

           \subfloat[Complementary benefits of VO and RF]{
                 \includegraphics[width=\linewidth]{figs/fusioncase.png} \label{fig:fusioncase}
           }
      \caption{Deficiencies of Active and Passive Tracking}
     \label{fig:limitations1}
\end{figure} 

%Despite the broader interest in tracking arena, there has been very little attention given to the potential of active and passive tracking together. Each aforementioned active and passive tracking  solutions work well under specific environmental assumptions and fail in case of respective adverse conditions (i.e., NLOS for RF and lack of features for VO). To dive into a more closure look how each of these tracking solutions, we show the tracking error for both RF and VO together under different environmental conditions (i.e., both favourable and adverse). Figure \ref{fig:fusioncase} shows the tracking error for RF and VO on a timeline. The first half of the trajectory is under a well-lit area with good features in the environment, and hence the VO error is well under 50cm. The second half of the trajectory is under dim-lit area with fewer features, resulting in high error. Similarly, for RF wherever there higher errors, most of the anchors are in NLOS. The figure shows an interesting pattern--- while each method seen in isolation outperform with each other under their best respective environmental conditions, there is a significant potential to reduce the error when seen them together because of the complementary action at different parts of the trajectory. Combining both RF and VO can eliminate the limitations of each individual sensor and provide a robust tracking irrespective of the aforementioned deficiencies for each sensor. Building on these insights, we take a hybrid approach to provide a general framework to combine both active and passive solutions for a fine-grained and robust tracking.
%
% \% Graph that shows UWB ranging and localization accuracy in LoS Vs. NLoS - one sender one receiver sufficient\\
% \% Graph that shows VO performance in bright light walking Vs. dim light walking -- a rectangular track.
% x\&Y axes should be in meters. Show just the trajectory\\
% \% Graph that shows the errors of UWB and VO can be complementary. \\

\begin{figure}[t]
\centering
        \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/globalview-trajectory.png}\label{fig:globalview-trajectory}
     }
        \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/globalview-error.png} \label{fig:globalview-error}
     }
     
    \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/globalview-disperror.png} \label{fig:globalview-disperror}
     }

      \caption{Global view benefits of RF-tracking for multi-user scenarios.}
     \label{fig:globalview}
\end{figure}

\subsubsection{Multi-user collaborative tracking:}
VO algorithms track users with respect to their individual starting position (origin). In order
to track multiple users with respect to one-another VO algorithms require all users to have: (a) common
origin(e.g., multiplayer gaming using Google AR-Core~\cite{}) and (b) significant scenery 
overlap~\cite{} - two impractical requirements for many AR/VR and gaming applications. 
RF based active localization, on the other hand, tracks and localizes users with respect
to physical anchor locations providing VO with a global frame of reference to 
transform its local position estimates into global co-ordinates. Unlike currently
used fiducial visual anchors that require dense deployment (depth estimation of 
cameras is limited to a few meters) and could potentially suffer from occlusions; 
RF anchors can provide global location estimates at fine timescales (15-20Hz) with only 
few sparsely distributed anchors.

%Graphs to relative error in user tracking with different percentages of overlap between users.
%RF-based tracking brings a direct advantage of global view for users that allows a quick recovery from unfavorable environmental conditions. Unlike VO tracking methods, where the tracking is 'relative' to the previous estimates, RF tracking is based on absolute localization. Because of the relative motion estimation, VO tracking is susceptible to a complete lose of tracking making it not recoverable when faced with feature less environments. While RF solutions are also affected by the NLOS anchors (as described in \S\ref{label:hybridcase}), the location estimates are independent and hence are quickly recoverable when moved to environments with LOS anchors. Figure \ref{fig:globalview-trajectory} an example such scenario where the VO started drifting at a corner due to a quick turn. The tracking continues to drift away from the groundtruth after the turn even though the environment is feature-rich because the quick turn caused a directional change as well. See Figure \ref{fig:globalview-disperror}, the displacement error after the turn quite low, but the tracking continues to shift away from the groundtruth because of the changed direction. As a result, the VO tracking error increases significantly after the turn (see Figure \ref{fig:globalview-error}). However, the RF tracking continues to follow the groundtruth even after facing some NLOS anchors and therefore can provide more robust recovery.
%
% \subsubsection{Can Lidars help?:}
% \%Graph to show deficiency of depth sensors and also some graph to show the case for multi user. 

\begin{figure}[t]
\centering
        \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/ekf-limitations1.png} \label{efk-limitation}
     }
        \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/ekf-limitations2.png} \label{bb-limitation}
     }
     
    \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/purelearning-limitations1.png} \label{efk-limitation}
     }
        \subfloat[]{%
      \includegraphics[width=0.5\linewidth]{figs/purelearning-limitations2.png} \label{bb-limitation}
     }
      \caption{Limitations of Tracking Algorithms and Pure Learning-based Fusion Methods in Seen and Unseen environments.}
     \label{fig:limitations2}
\end{figure} 

\subsubsection{Deficiency in current solutions:}
Traditional algorithm based data-fusion approaches like Kalman~\cite{} and Bayesian
filters~\cite{} aim to minimize statistical noise using time series data from individual
sensors. However, Kalman filters require system model to be linearized, which is often
not the case for VO and RF solutions. On the other hand, in indoor environments 
Bayesian filters like particle filter requires very large number of samples to 
estimate the posterior probability density of the system, and still can lead to the
case of \emph{particle depletion}~\cite{}. The Fig~\cite{} shows the performance of
Kalman and Particle filters for fusing ORB-SLAM3 and UWB datasets for a simple
trajectory, and the potential room for improvement (see ideal case of fusion).

%These methods rely only on the position estimations by individual sensors, without
%necessarily taking into account 



 % Results to motivate deficiencies of a pure learning or algorithmic approach.
%\subsubsection{Role of Algorithm-assisted Learning} % Results to motivate deficiencies of a pure learning or algorithmic approach.
%Given the ubiquity of the diverse sensors in the market, there has been an extensive work in combining one or more sensors to provide accurate tracking solutions~\cite{}. At a high level, these solutions can be divided into two categories: i) algorithmic models, ii) data-driven learned models. In the literature, both the active and passive tracking solutions have been individually realized using algorithmic and data-driven variants. For example, algorithmic active tracking RF solutions such as ranging and multilateration is more robust to unseen environment than pure deep learning based localization while the latter is more accurate in seen environments~\cite{}. Similarly, algorithmic VO-tracking methods such as ORBSLAM3 is more robust in unseen environments compared to its pure learning counterparts although being more accurate in some seen environments~\cite{}. 
%
%Generally speaking, learning has a significant potential to understand the latent relationship in raw sensor features and can produce more accurate tracking in seen environments while hard generalize for unseen environments. This classical dichotomy also exists in the recent multi-modal tracking solutions that are based on algorithms and pure learning. 
%
%For example, several algorithmic solutions proposed for fusing one or more sensor data for tracking using Kalman or Particle Filters that are limited to different types of distributions~\cite{}. Similarly, pure learning-based multi-model fusion has become more common because of success in deep learning-based NLP tasks, multimedia applications, and including tracking solutions such as ~\cite{}. To ascertain the aforementioned trade-off of robustness, accuracy, and generalization with the algorithmic and pure learning methods, we study combining the RF and VO sensor data using the two variants and show their individual limitations.

Figure \ref{efk-limitation} 

% \% Show results to a simple EKF approach. We can argue why EKF is not sufficient. - Trajectory graph for the same rectangular path\\
% \% Graph to show why blackbox approach will fail too. Show results to the same trajectory for blackbox. We don't have to give 
% details of BB here, but will say we will explain later.


==> background-related2.tex <==
\subsection{Background and Related Work} \label{sec:background}
%Current tracking solutions can broadly be 
%categorized as either active (infrastructure-assisted) or passive (odometry-based). 

%\subsubsection{Active Tracking:}
{\bf Active Tracking:}
Active tracking techniques leverage infrastructure-assistance through one or more 
pre-deployed anchors at known locations to continuously localize and track a device.  
The distance from the device to each anchor (a.k.a. ranging) is first estimated and 
subsequently, the estimated distances (to at least 3 anchors) %, or a single anchor with multiple antennas that can also estimate angle) 
are combined %with anchor(s) own locations 
using multi-lateration techniques~\cite{cheung2006constrained, hua2014geometrical} 
to determine the device's absolute location. 
%Accuracy of such anchor-based solutions
%depend  on the accuracy of the individual distance-angle estimations. Consequently, 
Prior works have proposed a plethora of solutions that leverage 
optical (e.g., IR beacons~\cite{kumar2014improving, jung2004ubitrack}, 
VLC~\cite{luo2017indoor}), acoustic (audible and ultrasound~\cite{chunyi2007, lollmann2018locata, constandache2014daredevil}) or RF technologies 
for effective ranging between the device and the anchor.
While optical solutions are perhaps the most accurate in ranging, they are
limited to LoS locations. Acoustic solutions are sensitive to ambient noise~\cite{jia2014soundloc}, 
larger material attenuation (e.g., wood, concrete)~\cite{tarzia2011indoor, constandache2014daredevil}, and certain environmental conditions 
(e.g., temperature, humidity) limiting them to room-level applications. % and additionally require
%complex signal processing techniques to process the received signal. 
%Compared to both optical and acoustic solutions,
In comparison,
RF signals are more robust in (LoS and NLoS) indoor environments, resulting in prior art %has proposed solutions using 
leveraging various RF technologies like WiFi~\cite{kotaru2015spotfi}, Bluetooth~\cite{chen2017locating}, 
mmWave~\cite{zeng2016human, palacios2018communication} 
and UWB~\cite{gezici2005localization, neuhold2019hipr} for effective ranging. mmWave and UWBs due to their wider channels (~1 GHz or more), 
provide more accurate (cm-level accuracy) range estimations (\S\ref{sec:tracking-mod}). 
Further,  UWBs (operating in lower frequencies of 3-10 GHz) offer better object penetrability than mmWave, making them more 
suitable for indoor tracking and localization.  \\
%This has led to their wide adoption in consumer smartphones (e.g. Apple iPhone 12, Samsung Galaxy S21, etc.), with commercial UWB chips also offering multi-antenna solutions that enable both range and AoA (angle-of-arrival) estimation. This reduces the infrastructure needs to a single anchor, that could be easily fulfilled by another stationary smart-phone/assistant or access point in the environment. 
%\subsubsection{Passive Tracking:} 
{\bf Passive Tracking:} 
Passive tracking solutions are odometry-based that do not require any pre-deployed infrastructure.
Visual and inertial odometry solutions are perhaps the most popular in this category. 
%used passive tracking techniques. 
Visual Odometry (VO) algorithms use a stream of 
camera images to track the motion. Changes in texture, color, shape (a.k.a image features) in successive 
camera images of a static environment 
are sufficient to track the motion with high precision (cm-scale). 
However, they suffer in environments with poor lighting, 
lack of texture or in conditions that enable perceptual aliasing~\cite{song2015high, taketomi2017visual}. Inertial odometry 
can thus be optionally used as an auxillary data source to VO, to improve tracking accuracy. 
\emph{Visual Simultaneous Localization and Mapping (vSLAM)} algorithms like 
ORB-SLAM~\cite{campos2021orb}, RTABMAP-SLAM~\cite{ragot2019benchmark} implement VO in realtime, by
continuously localizing a device within an environment, while incrementally 
constructing and updating the map of that environment. In addition, vSLAM algorithms 
implement optimizations like loop closure detection~\cite{labbe2014online} 
to correct VO drifts over time.\\
%and bundle adjustment optimizations~\cite{}. %vSLAM based VO solutions are currently
%used widely both in academia~\cite{} and industry~\cite{}.
%\subsubsection{Multi-sensor fusion for tracking:}
{\bf Multi-sensor fusion for tracking:}
\label{sec:sensor-fusion}
In addition to the individual active and passive tracking techniques discussed above, there has been a
plethora of work in fusing data from multiple sensors to improve tracking accuracy. The idea is to effectively combine data from 
two or more sensors to compensate for the noise from individual sensors.
Solutions in this space have
embraced either an algorithmic (e.g.,WiFi+Camera~\cite{hashemifar2019augmenting}, 
IMU+UWB~\cite{corrales2008hybrid}, 
IMU+WiFi~\cite{venkatnarayan2019measuring}) or a pure machine-learning approach (e.g.,mmWave+IMU~\cite{lu2020milliego}, 
Camera+IMU~\cite{clark2017vinet}, IMU+GPS~\cite{yao2017deepsense}, Camera+IMU\cite{chen2019selective}, Thermal+IMU~\cite{saputra2020deeptio}) 
for data fusion.
As we discuss below in \S~\ref{sec:dual-layer-fusion}, while the algorithmic approaches struggle to deliver high
tracking accuracies, the machine-learning solutions are largely limited to fusing sensors
for passive tracking, and %.  
often fail to generalize and perform robustly in untrained environments.  Different from these 
isolated approaches, \system leverages the opportunities of algorithmic as well as the learning 
based fusion to provide accurate, robust and scalable tracking simultaneously.
Lastly, works like~\cite{niranjini2019, magicol} leverage multiple 
sensors (RF+MagneticField) for localization, but also rely on elaborate mapping/finger-printing.
\system supports adhoc deployments in unseen environments with no prior-mapping.

\subsection{Choice of Tracking Techniques:}
\label{sec:tracking-mod}
While \system's design is applicable to numerous RF and visual tracking modalities, we rationalize the following choices.   

\noindent {\bf UWB-based active tracking:}  
%UWB employs a relatively wider
%bandwidth to other RF technologies to enabling highly accurate ranging. 
UWB's two-way ranging (TWR) protocol~\cite{dalce2014experimental}, coupled with its large bandwidth, provides robustness to indoor multipath and high ranging accuracies 
of a few tens-of-centimeters. Our experiments show that in indoor environments,
UWB can accurately measure ranges up to about 35-40m (comparable to WiFi) in LoS and about 25m in NLoS, with the accuracies degrading beyond 25m in NLoS. % However, the accuracy
%of NLoS ranges suffers for distances around 20m. 
Nonetheless, UWB still offers better accuracy compared to other RF modalities for indoor tracking (see table~\ref{tab:choiceofactivetracking}).
This has led to its wide adoption in consumer smartphones (e.g. Apple iPhone 12, Samsung Galaxy S21, etc.), with future UWB chips~\cite{nxpsinglechip} also offering multi-antenna solutions that enable both range and AoA (angle-of-arrival) estimation. The latter reduces the infrastructure needs to a single anchor -- easily fulfilled by a stationary smart-phone/assistant or access point.  
 Note that, with a similar ranging mechanism, \system can easily accommodate WiFi FTM~\cite{ibrahim2018verification} (in sub-6 GHz or mmWave band) as well.
%Note that our subsequent solution can be equally applied to WiFi as well (using its fast time measurement akin to UWB's TWR) either in lower frequencies or mmWave (60 GHz). 
%shows the accuracy of 
%ranges estimated by a pair of UWB radios in LoS and NLoS locations. In LoS,
%UWB provides median range errors of only {\color{red}XXcm} upto 30m. However, in  
%NLoS the maximum distance UWBs can range reduces signficantly to 20m and the errors
%in range estimates increase to {\color{red}YYcm}, specially for distances > 20m. 

\noindent {\bf ORB-SLAM3 for passive tracking:} ORB-SLAM3 (built upon ORB-SLAM2~\cite{mur2017orb} and ORB-SLAM~\cite{mur2015orb}) is a feature-based vSLAM algorithm,
 that is robust to motion clutter and can work with monocular,
stereo or RGB-D images. The ORB-features~\cite{rublee2011orb} are easy to extract and allow for fast matching 
across camera frames to enable real-time tracking. 
Previous studies show that ORB-SLAM algorithms can outperform other popular real-time SLAM algorithms
like RTABMAP-SLAM in odometry detection~\cite{ragot2019benchmark, campos2021orb}. Further, as we show later in \S~\ref{DESIGN}, \system
can just as easily be used to support other vSLAM (and Lidar-SLAM) algorithms.
%ORB-SLAM3 is the first vSLAM algorithm able to perform multi-map SLAM using pin-hole and fisheye  lens  models. 
%Our evaluation (Fig.~\ref{}) shows that ORB-SLAM3 can
%perform signficantly better than commercial VO implementation like ARCore~\cite{} when it comes to
%trajectory and odometry detection. 

%\emph{Camera Vs. Lidar:}
%Indoor Lidars (and depth sensors), unlike the 
%outdoor 360 deg industrial lidars (e.g., Velodyne Lidars~\cite{}), are designed for low-power hand-held devices and thus have
%limited Field-of-View, lower point density (fewer beams) and capable of depth-estimation for only up to a few meters 
%(e.g., 5m for Intel lidar cameara~\cite{}). Depth estimation of these sensors degrade considerably in 
%large indoor spaces (see Fig.~\cite{}) affecting the SLAM algorithms' VO performance. Consequently, we have
%made a conscious choice of excluding depth measurements in \system models. 
%Lidar SLAM algorithms (e.g., cartographer slam~\cite{}, GMapping~\cite{}) work similar to vSLAM 
%algorithms but with lidar streams as input. 

\begin{table}[t]
  \centering
     \caption{Choice of Passive Tracking solutions.}
     \vspace{-0.5cm}
  \begin{tabular}{|l|c|c|c|}
  \hline
      \textbf{ } & \textbf{Mean} & \textbf{Std} & \textbf{Max} \\
    \hline
    %\hline
    ARCore (Pixel2 Phone)~\cite{lanham2018learn} & 1m & 50cm & > 5m \\ \hline
    %Intel Realsense Tracking (T265 Stereo Cam)~\cite{} & 50cm & 20cm & 2m \\ \hline
    ORBSLAM3 (KITTI Dataset)~\cite{campos2021orb} & 10cm & 5cm & 1.5m\\ \hline
    RGBD SLAM (Intel D435 Depth Cam)~\cite{campos2021orb} & 50cm & 20cm & 2m \\ \hline
    Lidar (Intel L515)~\cite{zhang2014loam} & 40cm & 20cm & 2m \\ \hline
  \end{tabular}   \label{tab:choiceofpassivetracking}
\vspace{-0.2cm}
\end{table}
\begin{table}[t]
  \centering
     \caption{Choice of Active Tracking solutions.}
     \vspace{-0.5cm}
    \begin{tabular}{|l|c|c|c|c|}
  \hline
      \textbf{ } & \textbf{LTE~\cite{ni2017accurate}} & \textbf{WiFi~\cite{ibrahim2018verification}} & \textbf{UWB~\cite{ruiz2017comparing}} & \textbf{mmWave~\cite{palacios2017jade}} \\
    \hline
    %\hline
    Accuracy & 20m & 5m & 25cm & 1cm \\ \hline
    Range & 1km & 40m & 30m & 10m \\ \hline
  \end{tabular}   \label{tab:choiceofactivetracking}
\end{table}

\subsection{Case for Dual-layer Diversity in Fusion}
\label{sec:dual-layer-fusion}
\noindent \subsubsection{{Diversity in Tracking Modality (Active + Passive:)}}
\textbf{{Relative vs. Absolute Accuracy:}}
Although VO (ORB-SLAM3) provides highly accurate odometry ({\em relative} tracking),
they are vulnerable to error accumulation over time. Once an error sets in, the
relative measurements of  VO propagate  the error forward, resulting
in significant drifts in the estimated trajectories (Fig.~\ref{fig:vo-limitations}). UWB-based active
tracking is immune to such drifts as each location estimation is independent of the previous ones.
Errors that occur due to incorrect ranging estimates (e.g., NLoS anchors) do not propagate, 
allowing UWB to provide better accuracy in {\em absolute} tracking over time. 
%To that end, the UWBs active tracking is robust. 
However, UWB can only provide sub-meter scale coarse location estimates compared to VO's cm-scale finer
estimates. An effective fusion between the two sensors can bring complementary 
benefits to one-another, delivering a system capable of highly accurate absolute tracking over a sustained period of time. Fig~\ref{fig:fusioncase}
shows the significant potential for fusion between UWB and ORB-SLAM3 for a simple trajectory (details of our testbed and experiments are in Sec~\ref{IMPL}),
part of which is dimly lit (adverse to ORB-SLAM3), while another part contains NLoS anchors 
(adverse to UWB).


%While ORB-SLAM3's VO performs exceedingly
%well in well-lit areas, it starts accumulating errors as the user navigates
%through dim-lit areas. Due to the nature of the VO solution, the errors 
%propogates into the parts of the trajectory which is in well-lit areas,
%until the algorithm detects as loop and corrects the drift. The UWB has the luxury
%of localizing the user afresh each time ranging occurs, and hence does not carry forward
%the errors that accumulate in the region of NLOS anchors. However, the granularity of 
%the localization itself is at sub-meter scale, which is significantly higher than
%the finer (cm-scale) granular tracking VO provides in well-lit ideal conditions.
%An effective fusion (see error graph between time XXsec - YYsec) between the two 
%can potentially bring complementary benefits to deliver a robust system that 
%is capable of high-precision tracking.
%
%\subsubsection{Case for a Hybrid Approach} \label{label:hybridcase} Results to motivate
%deficiencies of isolated passive and active tracking approaches. 
%As discussed in (\S \ref{label:background}), there have been several recent 
%tracking solutions (active and passive) proposed in the research literature with a goal 
%towards achieving a fine-grained cm-scale tracking~\cite{}. Active tracking such as RF 
%(UWB in our case)-based solutions deploy a set of anchors in the environment, with users
%carrying a tag. A two-way ranging protocol is used to estimate the distance between the 
%tags (i.e., users) and the anchors, and localize the user with a multilateration algorithm
%from the measured ranges. State-of-the-art ranging methods provide up to a cm-scale ranging
%under specific conditions such as when most of the anchors are in line of sight (LOS) of the tracked
%users. However, the ranging can be noisy in case of a subset of anchors are under non-line-of-sight
%(NLOS) of users, consequently resulting in poor tracking accuracy under such conditions. 
%Figure \ref{fig:nlosvsranging} quantifies the ranging accuracy under LOS and NLOS for a single
%anchor and single tag in the UWB 6GHz band. Figure shows that, as the user moves far from the anchor
%in LOS, we find the ranging is consistent until 30m distance with a maximum of XX standard deviation. 
%Whereas for NLOS, the noise as high as YY within 20m and reaches to physical limitations of signal 
%propagation going out of range thereafter. As we show later, such noise in range measurements from 
%NLOS anchors can decrease the tracking accuracy by ZZ when compared with all anchors in LOS.
%Similarly, the passive tracking such as VO-based solutions exhibit such deficiencies while 
%providing a sub-centimeter level tracking accuracy under good environmental conditions. These 
%passive tracking solutions are primarily feature-based methods i.e., from the images captured 
%from the environment, similar features are estimated in consecutive images and the relative motion 
%is estimated from one image to another. Because of this dependence on features of consecutive images, 
%the tracking can fail if there are sudden changes or very few key features in the environment. Best 
%known such examples are--- lighting conditions, plain feature-poor environment (e.g., white walls),
%random motion (running or quick jerky motion in case of games), etc. Figure \ref{fig:vo-limitations} 
%shows a qualitative example trajectory with the VO tracking under bright and dim light conditions. 
%As shown, the tracking under bright-light light consistently follows the ground-truth trajectory, 
%the dim-light trajectory is off by almost XXm. The problem becomes more acute when the tracking is 
%under combined adverse conditions such as running with random motions under dim-light environment. 

\begin{figure}[t]
\centering
\vspace{-0.1cm}
        \subfloat[RF]{%
      \includegraphics[width=0.5\linewidth]{figs/range-accuracy-los-nlos-exp.png}\label{fig:nlosvsranging}
     }
        \subfloat[VO]{%
      \includegraphics[width=0.5\linewidth]{figs/vo-perf.pdf} \label{fig:vo-limitations}
     }

           \subfloat[Complementary benefits of VO and RF]{
                 \includegraphics[width=\linewidth]{figs/fusioncase.pdf} \label{fig:fusioncase}
           }
      \vspace{-0.3cm}
      \caption{Deficiencies of Active and Passive Tracking}
     \label{fig:limitations1}
\vspace{-0.4cm}
\end{figure} 

%Despite the broader interest in tracking arena, there has been very little attention given to the potential of active and passive tracking together. Each aforementioned active and passive tracking  solutions work well under specific environmental assumptions and fail in case of respective adverse conditions (i.e., NLOS for RF and lack of features for VO). To dive into a more closure look how each of these tracking solutions, we show the tracking error for both RF and VO together under different environmental conditions (i.e., both favourable and adverse). Figure \ref{fig:fusioncase} shows the tracking error for RF and VO on a timeline. The first half of the trajectory is under a well-lit area with good features in the environment, and hence the VO error is well under 50cm. The second half of the trajectory is under dim-lit area with fewer features, resulting in high error. Similarly, for RF wherever there higher errors, most of the anchors are in NLOS. The figure shows an interesting pattern--- while each method seen in isolation outperform with each other under their best respective environmental conditions, there is a significant potential to reduce the error when seen them together because of the complementary action at different parts of the trajectory. Combining both RF and VO can eliminate the limitations of each individual sensor and provide a robust tracking irrespective of the aforementioned deficiencies for each sensor. Building on these insights, we take a hybrid approach to provide a general framework to combine both active and passive solutions for a fine-grained and robust tracking.
%
% \% Graph that shows UWB ranging and localization accuracy in LoS Vs. NLoS - one sender one receiver sufficient\\
% \% Graph that shows VO performance in bright light walking Vs. dim light walking -- a rectangular track.
% x\&Y axes should be in meters. Show just the trajectory\\
% \% Graph that shows the errors of UWB and VO can be complementary. \\

% \begin{figure}[t]
% \centering
%         \subfloat[]{%
%       \includegraphics[width=0.5\linewidth]{figs/globalview-trajectory.png}\label{fig:globalview-trajectory}
%      }
%         \subfloat[]{%
%       \includegraphics[width=0.5\linewidth]{figs/globalview-error.png} \label{fig:globalview-error}
%      }
     
%     \subfloat[]{%
%       \includegraphics[width=0.5\linewidth]{figs/globalview-disperror.png} \label{fig:globalview-disperror}
%      }

%       \caption{Global view benefits of RF-tracking for multi-user scenarios.}
%      \label{fig:globalview}
% \end{figure}

\noindent\textbf{{Scalability vs. Accuracy -- Multi-user collaborative tracking:}}
Camera-based multi-user collaborative applications (e.g., AR/VR and gaming applications) are becoming increasingly popular across
multiple industries. Accurately tracking users with respect to one another, even in NLoS, is the key
to realizing such collaborative applications. However, VO algorithms track users with respect 
to their own individual starting position (origin). Unless all users start at a common origin and are in visual LoS of each other
(unrealistic expectation), it is infeasible to estimate users' locations with respect to one another. 
Hence, it is important to transform the VO's local position
estimates into global co-ordinates based on a common frame of reference.
In contrast, UWB's active tracking provides absolute location estimates of each user with
respect to a known UWB anchor's physical location. Fusing VO and UWB enables tracking users with respect to a
global reference point (UWB anchor), and thus with respect to one-another.

%#In order
%#to track multiple users with respect to one-another VO algorithms would require all users to have either a common
%#origin(e.g., multiplayer gaming using Google AR-Core~\cite{}) or a significant scenary 
%#overlap~\cite{}. Unfortunately, for many AR/VR and gaming applications, these requirements would not scale. 
%#UWB based active localization, on the other hand, tracks users with respect
%#to the physical anchor locations providing VO with a global frame of reference to 
%#transform its local position estimates into global co-ordinates. 
%#Unlike currently used fiducial visual anchors that require dense deployment (depth estimation of 
%#cameras is limited to a few meters) and could potentially suffer from occlusions; 
%#RF anchors can provide global location estimates at fine timescales (15-20Hz) with only 
%#few sparsely distributed anchors.

%Graphs to relative error in user tracking with different percentages of overlap between users.
%RF-based tracking brings a direct advantage of global view for users that allows a quick recovery from unfavorable environmental conditions. Unlike VO tracking methods, where the tracking is 'relative' to the previous estimates, RF tracking is based on absolute localization. Because of the relative motion estimation, VO tracking is susceptible to a complete lose of tracking making it not recoverable when faced with feature less environments. While RF solutions are also affected by the NLOS anchors (as described in \S\ref{label:hybridcase}), the location estimates are independent and hence are quickly recoverable when moved to environments with LOS anchors. Figure \ref{fig:globalview-trajectory} an example such scenario where the VO started drifting at a corner due to a quick turn. The tracking continues to drift away from the groundtruth after the turn even though the environment is feature-rich because the quick turn caused a directional change as well. See Figure \ref{fig:globalview-disperror}, the displacement error after the turn quite low, but the tracking continues to shift away from the groundtruth because of the changed direction. As a result, the VO tracking error increases significantly after the turn (see Figure \ref{fig:globalview-error}). However, the RF tracking continues to follow the groundtruth even after facing some NLOS anchors and therefore can provide more robust recovery.
%
% \subsubsection{Can Lidars help?:}
% \%Graph to show deficiency of depth sensors and also some graph to show the case for multi user. 

\subsubsection{{Diversity in Fusion Methodology (Algorithm + Data-driven)}}

\textbf{Robustness vs. Accuracy:} Current solutions for multi-sensor fusion can broadly be divided 
into either algorithm-driven or data-driven machine learning models.
The algorithmic solutions include the filter-based data-fusion
approaches (e.g., Kalman~\cite{venkatnarayan2019enhancing} and Bayesian
filters like particle filters~\cite{wang2017imu}), which aim to minimize 
statistical noise using time series data from individual sensors. 
However, we observe that these approaches consistently under-perform with degraded accuracy, when
fusing UWB and ORB-SLAM3. The Kalman filters require system model to be linearized and noise distributions to be Gaussian, 
which often do not hold for VO and RF data, either due to sensor (e.g. hardware issues) and/or environmental artifacts (e.g. scene and/or NLoS related issues). 
On the other hand, Bayesian filters like particle filter require a very large number of samples to 
accurately estimate the posterior probability density of the system.  In complex indoor
environments, this does not scale, resulting in particle depletion and consequently poor performance.  
Fig~\ref{efk-limitation} shows the performance of
Extended Kalman Filter (EKF) for fusing ORB-SLAM3 and UWB dataset for an indoor
trajectory in one of our testbeds (\S\ref{EVAL}). It reveals that the fused location is
still erroneous (with a large median error of \texttt{80 cm}), with a lot of
room for improvement.

The pure data-driven machine learning solutions (a.k.a Black-Box, BB) that target multi-sensor
fusion have largely focused on passive tracking -- 
e.g., VO-IMU fusion~\cite{clark2017vinet}, mmWave-IMU fusion~\cite{lu2020milliego}. These BB models
are trained to interpret and transform the input sequence of  raw sensor data
into relative location or pose estimates. Porting these solutions to fuse UWB's range estimates  
and VO's camera images, to predict {\em absolute} position estimates is challenging, putting a lot of burden 
 on the model in capturing the complex geometric problem structure that is inherent to RF and camera based localization.
This in-turn makes the model heavily reliant on input data distributions, resulting in 
poor performance in untrained environments. 
Fig~\ref{bb-limitation} shows the performance of a BB model
that fuses UWB ranges and camera images to estimate absolute device location in an unseen environment. 
The details of this model are deferred to section~\ref{sec:bbdesign}. 
It is evident that pure data-driven models trained with raw data inputs, while delivering superior 
performance in trained environments (see \ref{efk-limitation}), fail to generalize when deployed on unseen environments in the wild.

\begin{figure}
\centering
\vspace{-0.1cm}
      \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/ekf-limitations.png} \label{efk-limitation}
     }

    \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/purelearning-limitations.png}\label{bb-limitation} \label{bb-limitation}
     }
      \vspace{-0.2cm}
      \caption{Limitations of Tracking Algorithms and Pure ML-based Fusion Methods in Seen and Unseen environments.}
     \label{fig:limitations2}
\vspace{-0.4cm}
\end{figure} 


To summarize, while algorithmic solutions bring robustness to operation in various (untrained) environments but are unable to deliver effective fusion and hence high accuracy, data-driven approaches deliver very high accuracies through superior sensor fusion, albeit primarily in trained environments.
This motivates the need for a second layer of diversity that brings together the strengths of both algorithmic (generalizability from robustness) and data-driven (high accuracy from effective fusion) approaches. 
%they are unable to performance of algorithmic solutions are independent of operating environments, 
%need no training, but potentially can underperform. On the contrary, data-driven 
%models need extensive training, can deliver very good performance, but may not scale well to untrained environments. 
%Ideally, we would need a solution that is precise and scalable. \system is geared towards
%achieving this effectively.
%\subsubsection{Challenges in Realizing Dual-layer Diversity}
\underline{\bf Challenges in Realizing Dual-layer Diversity:}
A typical sensor fusion solution involves sensor measurements, processing of measurements, and the fusion mechanism itself. 
Building a fusion approach that incorporates this dual-layer diversity entails addressing several critical questions.\\
\noindent \textbf{(1)} Given the pros and cons of active and passive tracking, how should their measurements be fused to automatically overcome sensor hardware and environmental artifacts and deliver both accuracy and scalability?\\
\noindent \textbf{(2)}  How should the algorithmic and data-driven approaches split the burden of the sensor fusion pipeline to complementarily bring together their accuracy and robustness benefits?\\
\noindent \textbf{(3)}  Can the resulting approach be light-weight for real-time operation on resource-constrained device platforms?\\
\system adopts a systematic approach towards addressing these challenges %questions 
to deliver a robust, accurate and scalable tracking solution.

%\subsubsection{Challenges in UWB and ORB-SLAM3 data fusion:} 
%Fusing UWB's absolute location estimates with ORB-SLAM3's relative position estimates is tricky.
%Typically, fusion at data-level involve aggreagting 
%
%\subsubsection{A lightweight model that can scale:} While it is 

%These methods rely only on the position estimations by individual sensors, without
%necessarily taking into account 
 % Results to motivate deficiencies of a pure learning or algorithmic approach.
%\subsubsection{Role of Algorithm-assisted Learning} % Results to motivate deficiencies of a pure learning or algorithmic approach.
%Given the ubiquity of the diverse sensors in the market, there has been an extensive work in combining one or more sensors to provide accurate tracking solutions~\cite{}. At a high level, these solutions can be divided into two categories: i) algorithmic models, ii) data-driven learned models. In the literature, both the active and passive tracking solutions have been individually realized using algorithmic and data-driven variants. For example, algorithmic active tracking RF solutions such as ranging and multilateration is more robust to unseen environment than pure deep learning based localization while the latter is more accurate in seen environments~\cite{}. Similarly, algorithmic VO-tracking methods such as ORBSLAM3 is more robust in unseen environments compared to its pure learning counterparts although being more accurate in some seen environments~\cite{}. 
%Generally speaking, learning has a significant potential to understand the latent relationship in raw sensor features and can produce more accurate tracking in seen environments while hard generalize for unseen environments. This classical dichotomy also exists in the recent multi-modal tracking solutions that are based on algorithms and pure learning. 
%For example, several algorithmic solutions proposed for fusing one or more sensor data for tracking using Kalman or Particle Filters that are limited to different types of distributions~\cite{}. Similarly, pure learning-based multi-model fusion has become more common because of success in deep learning-based NLP tasks, multimedia applications, and including tracking solutions such as ~\cite{}. To ascertain the aforementioned trade-off of robustness, accuracy, and generalization with the algorithmic and pure learning methods, we study combining the RF and VO sensor data using the two variants and show their individual limitations.

% \% Show results to a simple EKF approach. We can argue why EKF is not sufficient. - Trajectory graph for the same rectangular path\\
% \% Graph to show why blackbox approach will fail too. Show results to the same trajectory for blackbox. We don't have to give 
% details of BB here, but will say we will explain later.


==> background-related3.tex <==
\subsection{Background and Related Work}
\label{sec:background}
%Current tracking solutions can broadly be 
%categorized as either active (infrastructure-assisted) or passive (odometry-based). 

%\subsubsection{Active Tracking:}
{\bf Active Tracking:}
Active tracking techniques use pre-deployed anchors 
at known locations to continuously localize and track a device. Distances (a.k.a ranges) to
one or more (at least 3) anchors is estimated and subsequently these
distances are combined using multi-lateration techniques~\cite{cheung2006constrained, hua2014geometrical} 
to determine the device's absolute location. A plethora of prior works
have proposed using optical
(e.g., IR beacons~\cite{kumar2014improving, jung2004ubitrack}, 
VLC~\cite{luo2017indoor}), acoustic (~\cite{chunyi2007, lollmann2018locata, constandache2014daredevil}) or RF technologies 
for effectively ranging between the device and anchors.
While optical solutions are the most accurate for ranging, they are
limited to LoS locations. Acoustic solutions are sensitive to ambient noise~\cite{jia2014soundloc}, 
material attenuation (e.g., wood, concrete)~\cite{tarzia2011indoor, constandache2014daredevil}, and certain environmental conditions 
(e.g., temperature, humidity) limiting them to a room-level applications.
In comparison, RF signals are more robust in LoS and NLoS indoor environments. Consequently, prior works %has proposed solutions using 
have leveraged various RF technologies like WiFi~\cite{kotaru2015spotfi}, Bluetooth~\cite{chen2017locating}, 
mmWave~\cite{zeng2016human, palacios2018communication} and UWB~\cite{gezici2005localization, neuhold2019hipr} 
for effective ranging. While both mmWave and UWBs use wider channels (~1 GHz or more) to
provide accurate (cm-level accuracy) range estimations (\S\ref{sec:tracking-mod}), 
UWBs operating in lower frequencies (3-10 GHz) offer better object penetrability than mmWave, making them more 
suitable for indoor tracking.  \\
{\bf Passive Tracking:}
These are odometry-based solutions that do not require pre-deployed infrastructure.
Visual and inertial odometry are perhaps the most popular in this category. 
Visual Odometry (VO) algorithms rely on changes in texture, color and shape %(a.k.a image features)
in successive camera images of a static environment to track the motion with high-precision (cm-scale).
However, they suffer in environments with poor lighting, 
lack of texture or in conditions that enable perceptual aliasing~\cite{song2015high, taketomi2017visual}. Inertial odometry 
can thus be optionally used as an auxillary data source to VO, to improve tracking accuracy. 
\emph{Visual Simultaneous Localization and Mapping (vSLAM)} algorithms like 
ORB-SLAM~\cite{campos2021orb}, RTABMAP-SLAM~\cite{ragot2019benchmark} implement VO in realtime by
continuously localizing a device within an environment, while incrementally 
constructing and updating the map of that environment.\\ %In addition, vSLAM algorithms 
%implement optimizations like loop closure detection~\cite{labbe2014online} 
%to correct VO drifts over time.\\
%and bundle adjustment optimizations~\cite{}. %vSLAM based VO solutions are currently
%used widely both in academia~\cite{} and industry~\cite{}.
%\subsubsection{Multi-sensor fusion for tracking:}
{\bf Multi-sensor fusion for tracking:}
\label{sec:sensor-fusion}
In the past,
there has been a plethora of work that propose fusing data from multiple sensors to 
compensate for the noise originating from individual sensors. 
Solutions in this space have
embraced either an algorithmic (e.g., WiFi+Camera~\cite{hashemifar2019augmenting}, 
IMU+UWB~\cite{corrales2008hybrid}, 
 IMU+WiFi~\cite{venkatnarayan2019measuring}) or a pure machine-learning approach (e.g., mmWave+IMU~\cite{lu2020milliego}, 
 Camera+IMU~\cite{clark2017vinet,chen2019selective}, IMU+GPS~\cite{yao2017deepsense}, Thermal+IMU~\cite{saputra2020deeptio}).
While the algorithmic approaches struggle to deliver high
tracking accuracies, the machine-learning solutions are largely limited to fusing sensors
for passive tracking, and
often fail to robustly generalize to untrained environments(see \S~\ref{sec:dual-layer-fusion}). Different from these 
isolated approaches, \system leverages the opportunities of algorithmic as well as the learning 
based fusion to provide accurate, robust and scalable tracking simultaneously.
Lastly, unlike works like ~\cite{niranjini2019, magicol}, \system does not require
prior mapping/finger-printing, and supports adhoc deployments in unseen environments.

\subsection{Choice of Tracking Techniques:}
\label{sec:tracking-mod}
Although \system's design is applicable to numerous RF and visual tracking modalities, we rationalize the following choices.   

\noindent {\bf UWB-based active tracking:}  
UWBs, compared to other RF technologies, offer a good balance between coverage 
(35-40m in LoS and 25-30m in NLoS) and ranging accuracy (see table~\ref{tab:choiceofactivetracking}).
Consequently, there has been a spurt of consumer devices (e.g., IPhone 12, Samsung Galaxy S21 etc.)
using UWB chips for indoor tracking. Future UWB chips~\cite{nxpsinglechip} are expected to offer
multi-antenna solutions that enable both ranging and AoA estimation. The latter reduces
the infrastructure need to a single anchor (e.g., an access pont).\\
%Note that, with a similar ranging mechanism, \system can easily accommodate WiFi FTM~\cite{ibrahim2018verification}
%(in sub-6 GHz or mmWave band) as well.
%UWB's two-way ranging (TWR) protocol~\cite{dalce2014experimental} coupled with its large 
%bandwidth provides robustness against indoor multipath, achieving high ranging accuracies 
%of a few tens-of-centimeters. Our experiments reveal that in indoor environments,
%UWBs can accurately measure ranges up to about 35-40m (comparable to WiFi) in LoS 
%and about 25m in NLoS, with the accuracies degrading beyond 25m in NLoS.
%Nonetheless, UWB still offers better accuracy compared to other
%other RF modalities(see table~\ref{tab:choiceofactivetracking}).
%This has led to its wide adoption in consumer smartphones (e.g. Apple iPhone 12, Samsung Galaxy S21, etc.), 
%with future UWB chips~\cite{nxpsinglechip} offering multi-antenna solutions that enable both range and AoA (angle-of-arrival)
%estimation. The latter reduces the infrastructure needs to a single anchor -- easily fulfilled by a stationary smart-phone/assistant or access point.  
%Note that our subsequent solution can be equally applied to WiFi as well (using its fast time measurement akin to UWB's TWR) either in lower frequencies or mmWave (60 GHz). 
%shows the accuracy of 
%ranges estimated by a pair of UWB radios in LoS and NLoS locations. In LoS,
%UWB provides median range errors of only {\color{red}XXcm} upto 30m. However, in  
%NLoS the maximum distance UWBs can range reduces signficantly to 20m and the errors
%in range estimates increase to {\color{red}YYcm}, specially for distances > 20m. 
\noindent {\bf ORB-SLAM3 for passive tracking:} ORB-SLAM3~\cite{}
%(built on ORB-SLAM2~\cite{mur2017orb} and ORB-SLAM~\cite{mur2015orb}) 
is a feature-based vSLAM algorithm, robust to motion clutter and can work with monocular,
stereo or RGB-D images. The ORB-features~\cite{rublee2011orb} are easy to extract and allow for fast matching 
across camera frames to enable real-time tracking. 
Previous studies show that ORB-SLAM algorithms can significantly outperform other popular real-time SLAM algorithms
in odometry detection~\cite{ragot2019benchmark, campos2021orb}. (Please refer to 
to our technical report~\cite{} for performance comparisons between VSLAM algorithms).
Nonetheless, in \S~\ref{DESIGN} we discuss how \system can just as easily support other vSLAM algorithms.
%ORB-SLAM3 is the first vSLAM algorithm able to perform multi-map SLAM using pin-hole and fisheye  lens  models. 
%Our evaluation (Fig.~\ref{}) shows that ORB-SLAM3 can
%perform signficantly better than commercial VO implementation like ARCore~\cite{} when it comes to
%trajectory and odometry detection. 
%\emph{Camera Vs. Lidar:}
%Indoor Lidars (and depth sensors), unlike the 
%outdoor 360 deg industrial lidars (e.g., Velodyne Lidars~\cite{}), are designed for low-power hand-held devices and thus have
%limited Field-of-View, lower point density (fewer beams) and capable of depth-estimation for only up to a few meters 
%(e.g., 5m for Intel lidar cameara~\cite{}). Depth estimation of these sensors degrade considerably in 
%large indoor spaces (see Fig.~\cite{}) affecting the SLAM algorithms' VO performance. Consequently, we have
%made a conscious choice of excluding depth measurements in \system models. 
%Lidar SLAM algorithms (e.g., cartographer slam~\cite{}, GMapping~\cite{}) work similar to vSLAM 
%algorithms but with lidar streams as input. 
%\begin{table}[t]
%  \centering
%     \caption{Choice of Passive Tracking solutions.}
%     \vspace{-0.5cm}
%  \begin{tabular}{|l|c|c|c|}
%  \hline
%      \textbf{ } & \textbf{Mean} & \textbf{Std} & \textbf{Max} \\
%    \hline
%    %\hline
%    ARCore (Pixel2 Phone)~\cite{lanham2018learn} & 1m & 50cm & > 5m \\ \hline
%    %Intel Realsense Tracking (T265 Stereo Cam)~\cite{} & 50cm & 20cm & 2m \\ \hline
%    ORBSLAM3 (KITTI Dataset)~\cite{campos2021orb} & 10cm & 5cm & 1.5m\\ \hline
%    RGBD SLAM (Intel D435 Depth Cam)~\cite{campos2021orb} & 50cm & 20cm & 2m \\ \hline
%    Lidar (Intel L515)~\cite{zhang2014loam} & 40cm & 20cm & 2m \\ \hline
%  \end{tabular}   \label{tab:choiceofpassivetracking}
%\vspace{-0.2cm}
%\end{table}
\begin{table}[t]
  \centering
     %\caption{Choice of Active Tracking solutions.}
     \caption{Comparison of RF technologies - Coverage Vs. Accuracy.}
     \vspace{-0.5cm}
    \begin{tabular}{|l|c|c|c|c|}
  \hline
  \textbf{ } & \textbf{LTE~\cite{ni2017accurate}} & \textbf{WiFi~\cite{ibrahim2018verification}} & \textbf{UWB~\cite{ruiz2017comparing}} & \textbf{mmWave~\cite{palacios2017jade}} \\
    \hline
    %\hline
    Accuracy & 20m & 5m & 25cm & 1cm \\ \hline
    Range & 1km & 40m & 30m & 10m \\ \hline
  \end{tabular}   \label{tab:choiceofactivetracking}
\end{table}

\subsection{Case for Dual-layer Diversity in Fusion}
\label{sec:dual-layer-fusion}
\noindent \subsubsection{{Diversity in Tracking Modality (Active + Passive:)}}
\textbf{{Relative vs. Absolute Accuracy:}}
VO (ORV-SLAM3) algorithms' {\em relative} tracking -- despite some of its 
intrinsic optimizations (e.g., loop closure detection) -- are vulnerable to 
error accumulation over time. 
Once an error sets in, the relative measurements of the VO propagate the error forward, resulting
in significant drifts in the estimated trajectories (Fig.~\ref{fig:vo-limitations}). UWB-based active
tracking is immune to such drifts as each location estimation is independent of the previous ones.
Errors that occur due to incorrect ranging estimates (e.g., NLoS anchors) do not propagate, 
allowing UWB to provide better accuracy in {\em absolute} tracking over time. 
However, UWB can only provide sub-meter scale coarse location estimates compared to VO's cm-scale finer
estimates. An effective fusion between the two sensors can bring complementary 
benefits to one-another, delivering a system capable of highly accurate absolute tracking 
over a sustained period of time. Fig~\ref{fig:fusioncase}
shows the significant potential for fusion between UWB and ORB-SLAM3 for a simple trajectory 
(details of experimentation are in \S\ref{IMPL}),
part of which is dimly lit (adverse to ORB-SLAM3), while another part contains NLoS anchors 
(adverse to UWB).

\noindent\textbf{{Scalability vs. Accuracy -- Multi-user collaborative tracking:}}
Accurately tracking users with respect to one another (even in NLoS) is the key to
realizing camera-based multi-user collaborative applications (E.g., AR/VR gaming applications).
However, VO algorithms track users with respect 
to their own individual starting point. Unless all users start at a common origin and are in visual LoS of each other
(unrealistic expectation), it is infeasible to estimate users' locations with respect to one another. 
%Hence, it is important to transform the VO's local position
%estimates into global co-ordinates based on a common frame of reference.
In contrast, UWB's active tracking provides absolute location estimates of each user with
respect to a known UWB anchor's physical location. 
Fusing VO's relative locations with UWB's absolute location estimates enables tracking users accurately with respect to a
global reference point (UWB anchor), and thus with respect to one-another.
%While ORB-SLAM3's VO performs exceedingly
%well in well-lit areas, it starts accumulating errors as the user navigates
%through dim-lit areas. Due to the nature of the VO solution, the errors 
%propogates into the parts of the trajectory which is in well-lit areas,
%until the algorithm detects as loop and corrects the drift. The UWB has the luxury
%of localizing the user afresh each time ranging occurs, and hence does not carry forward
%the errors that accumulate in the region of NLOS anchors. However, the granularity of 
%the localization itself is at sub-meter scale, which is significantly higher than
%the finer (cm-scale) granular tracking VO provides in well-lit ideal conditions.
%An effective fusion (see error graph between time XXsec - YYsec) between the two 
%can potentially bring complementary benefits to deliver a robust system that 
%is capable of high-precision tracking.
%
%\subsubsection{Case for a Hybrid Approach} \label{label:hybridcase} Results to motivate
%deficiencies of isolated passive and active tracking approaches. 
%As discussed in (\S \ref{label:background}), there have been several recent 
%tracking solutions (active and passive) proposed in the research literature with a goal 
%towards achieving a fine-grained cm-scale tracking~\cite{}. Active tracking such as RF 
%(UWB in our case)-based solutions deploy a set of anchors in the environment, with users
%carrying a tag. A two-way ranging protocol is used to estimate the distance between the 
%tags (i.e., users) and the anchors, and localize the user with a multilateration algorithm
%from the measured ranges. State-of-the-art ranging methods provide up to a cm-scale ranging
%under specific conditions such as when most of the anchors are in line of sight (LOS) of the tracked
%users. However, the ranging can be noisy in case of a subset of anchors are under non-line-of-sight
%(NLOS) of users, consequently resulting in poor tracking accuracy under such conditions. 
%Figure \ref{fig:nlosvsranging} quantifies the ranging accuracy under LOS and NLOS for a single
%anchor and single tag in the UWB 6GHz band. Figure shows that, as the user moves far from the anchor
%in LOS, we find the ranging is consistent until 30m distance with a maximum of XX standard deviation. 
%Whereas for NLOS, the noise as high as YY within 20m and reaches to physical limitations of signal 
%propagation going out of range thereafter. As we show later, such noise in range measurements from 
%NLOS anchors can decrease the tracking accuracy by ZZ when compared with all anchors in LOS.
%Similarly, the passive tracking such as VO-based solutions exhibit such deficiencies while 
%providing a sub-centimeter level tracking accuracy under good environmental conditions. These 
%passive tracking solutions are primarily feature-based methods i.e., from the images captured 
%from the environment, similar features are estimated in consecutive images and the relative motion 
%is estimated from one image to another. Because of this dependence on features of consecutive images, 
%the tracking can fail if there are sudden changes or very few key features in the environment. Best 
%known such examples are--- lighting conditions, plain feature-poor environment (e.g., white walls),
%random motion (running or quick jerky motion in case of games), etc. Figure \ref{fig:vo-limitations} 
%shows a qualitative example trajectory with the VO tracking under bright and dim light conditions. 
%As shown, the tracking under bright-light light consistently follows the ground-truth trajectory, 
%the dim-light trajectory is off by almost XXm. The problem becomes more acute when the tracking is 
%under combined adverse conditions such as running with random motions under dim-light environment. 

\begin{figure}[t]
\centering
\vspace{-0.1cm}
        \subfloat[RF]{%
      \includegraphics[width=0.5\linewidth]{figs/range-accuracy-los-nlos-exp.png}\label{fig:nlosvsranging}
     }
        \subfloat[VO]{%
      \includegraphics[width=0.5\linewidth]{figs/vo-perf.pdf} \label{fig:vo-limitations}
     }

           \subfloat[Complementary benefits of VO and RF]{
                 \includegraphics[width=\linewidth]{figs/fusioncase.pdf} \label{fig:fusioncase}
           }
      \vspace{-0.3cm}
      \caption{Deficiencies of Active and Passive Tracking}
     \label{fig:limitations1}
\vspace{-0.4cm}
\end{figure} 


%#In order
%#to track multiple users with respect to one-another VO algorithms would require all users to have either a common
%#origin(e.g., multiplayer gaming using Google AR-Core~\cite{}) or a significant scenary 
%#overlap~\cite{}. Unfortunately, for many AR/VR and gaming applications, these requirements would not scale. 
%#UWB based active localization, on the other hand, tracks users with respect
%#to the physical anchor locations providing VO with a global frame of reference to 
%#transform its local position estimates into global co-ordinates. 
%#Unlike currently used fiducial visual anchors that require dense deployment (depth estimation of 
%#cameras is limited to a few meters) and could potentially suffer from occlusions; 
%#RF anchors can provide global location estimates at fine timescales (15-20Hz) with only 
%#few sparsely distributed anchors.

%Graphs to relative error in user tracking with different percentages of overlap between users.
%RF-based tracking brings a direct advantage of global view for users that allows a quick recovery from unfavorable environmental conditions. Unlike VO tracking methods, where the tracking is 'relative' to the previous estimates, RF tracking is based on absolute localization. Because of the relative motion estimation, VO tracking is susceptible to a complete lose of tracking making it not recoverable when faced with feature less environments. While RF solutions are also affected by the NLOS anchors (as described in \S\ref{label:hybridcase}), the location estimates are independent and hence are quickly recoverable when moved to environments with LOS anchors. Figure \ref{fig:globalview-trajectory} an example such scenario where the VO started drifting at a corner due to a quick turn. The tracking continues to drift away from the groundtruth after the turn even though the environment is feature-rich because the quick turn caused a directional change as well. See Figure \ref{fig:globalview-disperror}, the displacement error after the turn quite low, but the tracking continues to shift away from the groundtruth because of the changed direction. As a result, the VO tracking error increases significantly after the turn (see Figure \ref{fig:globalview-error}). However, the RF tracking continues to follow the groundtruth even after facing some NLOS anchors and therefore can provide more robust recovery.
%
% \subsubsection{Can Lidars help?:}
% \%Graph to show deficiency of depth sensors and also some graph to show the case for multi user. 

\subsubsection{{Diversity in Fusion Methodology (Algorithm + Data-driven)}}
\textbf{Robustness vs. Accuracy:} Current solutions for multi-sensor fusion can broadly be divided 
into either algorithm-driven or data-driven machine learning models.
Algorithmic solutions (e.g., Kalman Filter (KF)~\cite{venkatnarayan2019enhancing} and Bayesian
filters like particle filters~\cite{wang2017imu}) aim to minimize 
statistical noise using time series data from individual sensors. 
However, we observe that these approaches consistently under-perform when
fusing UWB and ORB-SLAM3. The KF requires system model to be linearized and noise distribution to be Gaussian, 
which often is not true for VO and RF data, either due to sensor (e.g. hardware issues) and/or 
environmental artifacts (e.g. scene and/or NLoS related issues). 
Bayesian filters like particle filter require a very large number of samples to 
accurately estimate the posterior probability density of the system.  In complex indoor
environments, this does not scale, resulting in particle depletion and consequently poor performance.  
Fig~\ref{efk-limitation} shows the performance of
Extended Kalman Filter (EKF) for fusing ORB-SLAM3 and UWB dataset for an indoor
trajectory in one of our testbeds (\S\ref{EVAL}). It reveals that the fused location is
still erroneous (with a large median error of \texttt{80 cm}), with a lot of
room for improvement.\\
The pure data-driven machine learning solutions (a.k.a Black-Box, BB) that target multi-sensor
fusion have largely focused on passive tracking -- 
e.g., VO-IMU fusion~\cite{clark2017vinet}, mmWave-IMU fusion~\cite{lu2020milliego}. These BB models
are trained to interpret and transform the input sequence of raw sensor data
into relative location or pose estimates. Porting these solutions to fuse UWB's range estimates  
and VO's camera images, to predict {\em absolute} position estimates puts a lot of burden 
on the model in capturing the complex geometric problem structure inherent to RF and camera based localization.
This in-turn makes the model heavy (require large processing power),
and overly reliant on input data distributions resulting in 
poor performance in untrained environments. 
Fig~\ref{bb-limitation} shows the performance of a BB model
that fuses UWB ranges and camera images to estimate absolute device location in an unseen environment. 
(Details of this model are in \S\ref{sec:bbdesign}). 
It is evident that pure data-driven models trained with raw data inputs, while delivering superior 
performance in trained environments (see \ref{efk-limitation}), fail to 
generalize when deployed on unseen environments in the wild.

\begin{figure}
\centering
\vspace{-0.1cm}
      \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/ekf-limitations.png} \label{efk-limitation}
     }

    \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/purelearning-limitations.png}\label{bb-limitation} \label{bb-limitation}
     }
      \vspace{-0.2cm}
      \caption{Limitations of Tracking Algorithms and Pure ML-based Fusion Methods in Seen and Unseen environments.}
     \label{fig:limitations2}
\vspace{-0.4cm}
\end{figure} 

To summarize, while algorithmic solutions bring robustness to operation in various (untrained) environments 
but are unable to deliver effective fusion and hence high accuracy, data-driven approaches deliver 
high accuracies through superior sensor fusion, albeit primarily in trained environments.
This motivates the need for a second layer of diversity that brings together the strengths of both 
algorithmic (generalizability from robustness) and data-driven (high accuracy from effective fusion) 
approaches. \\
%they are unable to performance of algorithmic solutions are independent of operating environments, 
%need no training, but potentially can underperform. On the contrary, data-driven 
%models need extensive training, can deliver very good performance, but may not scale well to untrained environments. 
%Ideally, we would need a solution that is precise and scalable. \system is geared towards
%achieving this effectively.
%\subsubsection{Challenges in Realizing Dual-layer Diversity}
\underline{\bf Challenges in Realizing Dual-layer Diversity:}
Building a fusion approach that incorporates this dual-layer diversity entails addressing several critical questions.\\
\noindent \textbf{(1)} Given the pros and cons of active and passive tracking, how should their measurements be fused to automatically overcome sensor hardware and environmental artifacts and deliver both accuracy and scalability?\\
\noindent \textbf{(2)}  How should the algorithmic and data-driven approaches split the burden of the sensor fusion pipeline to complementarily bring together their accuracy and robustness benefits?\\
\noindent \textbf{(3)}  Can the resulting approach be light-weight for real-time operation on resource-constrained device platforms?\\
\system adopts a systematic approach towards addressing these challenges %questions 
to deliver a robust, accurate and scalable tracking solution.

%\subsubsection{Challenges in UWB and ORB-SLAM3 data fusion:} 
%Fusing UWB's absolute location estimates with ORB-SLAM3's relative position estimates is tricky.
%Typically, fusion at data-level involve aggreagting 
%
%\subsubsection{A lightweight model that can scale:} While it is 

%These methods rely only on the position estimations by individual sensors, without
%necessarily taking into account 
 % Results to motivate deficiencies of a pure learning or algorithmic approach.
%\subsubsection{Role of Algorithm-assisted Learning} % Results to motivate deficiencies of a pure learning or algorithmic approach.
%Given the ubiquity of the diverse sensors in the market, there has been an extensive work in combining one or more sensors to provide accurate tracking solutions~\cite{}. At a high level, these solutions can be divided into two categories: i) algorithmic models, ii) data-driven learned models. In the literature, both the active and passive tracking solutions have been individually realized using algorithmic and data-driven variants. For example, algorithmic active tracking RF solutions such as ranging and multilateration is more robust to unseen environment than pure deep learning based localization while the latter is more accurate in seen environments~\cite{}. Similarly, algorithmic VO-tracking methods such as ORBSLAM3 is more robust in unseen environments compared to its pure learning counterparts although being more accurate in some seen environments~\cite{}. 
%Generally speaking, learning has a significant potential to understand the latent relationship in raw sensor features and can produce more accurate tracking in seen environments while hard generalize for unseen environments. This classical dichotomy also exists in the recent multi-modal tracking solutions that are based on algorithms and pure learning. 
%For example, several algorithmic solutions proposed for fusing one or more sensor data for tracking using Kalman or Particle Filters that are limited to different types of distributions~\cite{}. Similarly, pure learning-based multi-model fusion has become more common because of success in deep learning-based NLP tasks, multimedia applications, and including tracking solutions such as ~\cite{}. To ascertain the aforementioned trade-off of robustness, accuracy, and generalization with the algorithmic and pure learning methods, we study combining the RF and VO sensor data using the two variants and show their individual limitations.

% \% Show results to a simple EKF approach. We can argue why EKF is not sufficient. - Trajectory graph for the same rectangular path\\
% \% Graph to show why blackbox approach will fail too. Show results to the same trajectory for blackbox. We don't have to give 
% details of BB here, but will say we will explain later.


==> design.tex <==
%design

\subsection{Overview of \system}
\% Dual-layered fusion approach that (a) at one level, employs an algorithm-driven approach for feature engineering and a data-driven approach for fusion of the sensor features through cross-modal attention, and (b) at another level, fuses and leverages the complementary nature of active (RF) and passive (visual) tracking sensors, to deliver robust and  accurate, multi-agent tracking. Algorithmic approach allows for embedding of the physical and geometrical nature of the localization problem by providing the absolute (RF) and relative (visual) location estimates from the respective sensors as features. These estimates, along with other features specific to the sensors (RF channel quality, camera inter-frame keypoints, etc.) that in turn determine the certainty of these estimates, together form a robust set of features that drive the data-driven fusion of these sensors to predict the final absolute location estimate of the device with a high accuracy even under challenging environment conditions. Leveraging the initial location estimates from algorithms as features, alleviates the need for the data-driven fusion module to do the heavy-lifting in capturing the physical-geometrical embedding inherent to the sensors, thereby resulting in two key benefits: (i) scalability and generalizability:  delivering accurate tracking even in unseen challenging environmental conditions, and (ii) real-time tracking: significantly reduces the compute-intensive nature of the end-to-end processing pipeline to enable real-time operation. 

% \begin{figure}[t]
% \centering
%         \subfloat[P2P Ranging]{%
%       \includegraphics[width=0.35\linewidth]{figs/ranging-a.png} 
%      }
%         \subfloat[TWR Protocol Message Exchange]{%
%       \includegraphics[width=0.65\linewidth]{figs/ranging-b.png}  
%      }
%     % \subfloat[Trilateration]{%
%     %   \includegraphics[width=0.4\linewidth]{figs/trilateration.png}  
%     %  }
%       \caption{IEEE 802.15.4 TWR ranging protocol to measure the range between two nodes.}
%      \label{fig:extreme}
% \end{figure}

\subsection{Algorithm-driven Feature Engineering}
The first stage of our dual-layer fusion is feature engineering from individual sensor tracking algorithms. In the following, we provide the details of the feature extraction from RF and VO tracking algorithms.

\subsubsection{RF Path} %selection of range estimates, algorithm details, composition of features 
As mentioned before, we use UWB for RF tracking modality. UWB nodes use time of flight (ToF) to measure the range (i.e., distance) between two nodes by multiplying the signal's ToF with speed of light. At each time instance, the collected ranges and the respective fixed positions of the anchors (as <$location_i$, $range_i$> tuples) are fed to the multilateration algorithm and and solve for \textit{\underline{absolute location}} estimate. To estimate a 2D location, three non-collinear anchors are sufficient while more anchors may improve the estimate further. Assuming there are $n$ anchors deployed in the environment, each with fixed position ($x_i$, $y_i$) with $i=1..n$, and original location of the tag as ($x, y$), the location can be estimated by minimizing the error $f_i = R_i - \sqrt{(x_i-x)^2+(y_i-y)^2}$, where $R_i$ is the range between tag and anchor $i$. Ideally, we want the $f_i$ to be zero. Therefore, by setting the error equation to zero, we can solve for an optimal ($\mathcal{X}$, $\mathcal{Y}$) that gives overall minimum error for all anchors. 

%There are a variety of optimization solutions available in the literature~\cite{}. We adopt a simple least square error optimization with geometric constraints in order to force the solutions to be in the intersection areas of all multilateration circles.

\smallskip
\noindent \textbf{Challenges of UWB Localization:} A key problem with the above direct optimization is the localization accuracy is influenced by the environmental conditions. Recall from \S\ref{label:background}, the range estimates under LOS and NLOS differ significantly, with NLOS anchors having high variance in range estimates event at short distances. Such inaccurate range estimates will influence the optimization to minimize its range error, and estimate a sub-optimal location. For example, Figure \ref{fig:errorvlosnlos} shows the impact of various combinations of anchors in LoS and NLoS on localization. The median error is 0.2m and 1m when all anchors are under LoS and NLoS respectively. The max error for NLoS case is as high as 3m. This shows that noisy anchors with poor range estimates can result in huge localization errors.  

\begin{figure}[!h]
\centering
    \subfloat[Error vs. received power.]{%
    \includegraphics[width=0.5\linewidth]{figs/losvsnloserror.pdf}\label{fig:errorvlosnlos}
    }
    \subfloat[Best case error]{%
      \includegraphics[width=0.5\linewidth]{figs/besterror.pdf} \label{fig:besterror}
     }
    \caption{Localization error under LOS and NLOS scenarios.}
\end{figure} 

To ascertain this finding, we study a more practical scenario by deploying the anchors in a mixed LoS and NLoS combination. We compute the error with all the anchors (Mixed), and also under a best case. The best case error is computing by populating all possible combinations of anchors out of deployed 5 anchors having at least 3 (i.e., $5 \choose 3$=10) and selecting a best combination (approx all LoS) for each point measurement that gives minimum error when compared against the groundtruth trajectory. Figure \ref{fig:besterror} shows the difference in error with the mixed set of anchors versus best selected anchors. The median difference between both cases XXcm while the max error under best case is well under a meter. While this suggests that filtering out NLoS anchors brings down the error significantly, selecting the best anchors is nontrivial without knowing the ground truth trajectory in advance, a challenge we address next.

%One way to identify these noisy anchors is by as by \textit{learning} to select the best anchors by training the model with ranges from all the anchors offline using the available groundtruth. However, this will lead to generalization issues ....

\noindent \textbf{Selecting best anchors:} As the problem space involves selecting anchors from only a few anchors (we deploy only 7 anchors in our system), we leverage simple learning-but explainable ML models (e.g., SVM and Logistic regression) to classify the best anchors. To this end, we derive a separate anchor classification dataset from our collected data to train a classifier that selects the best $K$ anchors for localization. We fit a model by inputting the ranges from all anchors along with their corresponding certainty features (described in \S \ref{}), and the best anchors as output binary vector. We create this dataset with best anchors offline by localizing with all possible combinations of anchors and selecting a combination that gives the minimum error when compared to the groundtruth. We fit a multi-output classification model to predict the best anchor binary vector using classifier chains~\cite{} to exploit the correlation among the anchors rather than independently selecting each anchor. We fit three models--- SVM, Logistic Regression, and a RandomForests classifier and perform a grid search on each of them to tune the best parameters. After the grid search, we select a best performing model (SVM in our case) and its optimal parameters from the search. Figure \ref{fig:anchorselection} shows the prediction performance in terms of mean accuracy when prediction a subset of anchors from 7 anchors in our system. As shown, the model performance is highly accurate with the accuracy increasing when selecting more anchors. 

\begin{figure}[!h]
\centering
\begin{minipage}{.47\linewidth}
\centering
  \includegraphics[width=\linewidth]{figs/anchor-selection.pdf}
  \caption{Selecting different no of anchors out of 7.}
\end{minipage}\hspace{0.3cm}%
\begin{minipage}{.47\linewidth}
  \includegraphics[width=\linewidth]{figs/anchor-selection2.pdf}
  \caption{Selecting 3 out of different no of anchors.}
\end{minipage}
\label{fig:anchorselection}
\end{figure}

\noindent \textbf{Predicting best anchors improves accuracy but not sufficient for fusion:} Using the above anchor selection model, we can improve the location estimate by filtering out some NLoS anchors. However, the localization error is still as high as 1m (see Figure \ref{}) even after the selecting the best anchors. Ideally, if the anchors are deployed in such a way that we can always predict at least 3 LoS anchors out of all the anchors, the location estimate from the multi-lateration algorithm is sufficiently accurate (see \ref{fig:errorvlosnlos}). However, guaranteeing LoS anchors throughout the users' trajectory is not practical. Consequently, leveraging the absolute location estimates alone that are at-times erroneous under unfavourable environment (i.e., NLoS) misguide the fusion framework to inefficiently adapt to different RF environmental conditions. To counter this challenge, we need to incorporate additional features to fusion framework along with the absolute location estimate. These features should be  environment-dependent to adapt the fusion to different environmental conditions and provide a certainty measure in the location estimates. We explore a variety of certainty metrics that quantify the impact of RF environmental conditions and leverage these metrics along with the location estimates from the algorithm for the fusion.

\noindent \textbf{Feature composition:} The localization error mainly results from two sources--- i) from the accuracy of range estimates (recall from \S\ref{}), ii) from the algorithmic optimization when the circles of ranges of anchors do not overlap at a single location. While the algorithmic error can be obtained directly after the minimization, determining the accuracy of range estimates require the understanding of fundamental signal characteristics. As shown in the Figure \ref{} in \S\ref{}, the range estimates are significantly poor under NLOS scenario compared to LOS event at shorter distances. We investigate several link related metrics (e.g., first path power, amplitude, impulse power etc) to identify this behaviour, and find that the received signal power shows complementary behaviour for range estimates. The received signal power can be estimated using the below equation.

\begin{equation}
    P_{rx} = 10 \times \log_{10}\left({\frac{C \times 2^{17}}{N^2}}\right) - A \hspace{0.1cm}dBm
\end{equation}

where, $C$ is the Channel Impulse Response Power, $N$ is a preamble accumulation count~\cite{}, $A$ is a constant that is determined with the pulse repetition frequency~\cite{}. Figure \ref{fig:rangevsrxp} shows the impact of range versus power under LoS and NLoS conditions for one anchor. The figure shows that as we move away from the anchor, the received power under NLOS goes below -95dBm within 15m whereas the power remains above -90dBm even after 30m. Furthermore, Figure \ref{fig:errorvsrxp} shows that the received power has a strong negative correlation with the localization error having a Pearson correlation coefficient of -0.63. This gives us an insight in understanding the accuracy of ranging under both scenarios, although, with a nonlinear relationship. We leverage these ranges and received power estimates together as a form of certainty measures in modeling our anchors as LoS and NLoS and combine these certainty features with the absolute location estimates from the multi-lateration algorithm as a composed RF input to our fusion framework. Formally put, the input from the RF path to our fusion is given as $<\mathcal{X} \oplus R_i | L_i, <\mathcal{Y} \oplus R_i | L_i>$, where $\oplus$ is the concatenation operation of the location estimates with the range and link quality of each anchor.

\begin{figure}[t]
\centering
    \subfloat[Range vs. received power.]{%
      \includegraphics[width=0.5\linewidth]{figs/range_vs_rx_power.png} \label{fig:rangevsrxp}
     }
    \subfloat[Received power vs. Error]{%
      \includegraphics[width=0.5\linewidth]{figs/overall_correlation.pdf} \label{fig:errorvsrxp}
     }
     \caption{Received power vs. ranging and localization error.}
\end{figure} 

\subsubsection{Visual Path} % algorithm details, composition of features
Most of the visual SLAM solutions have mainly three components--- i) Tracking, ii) Local Mapping, iii) Loop closing~\cite{}. The Tracking module uses a stream of stereo frames to incrementally localize the camera on a frame-by-frame basis. This is accomplished by extracting unique features from the images and establishing matching keypoint correspondences between frames. Typical features can be SIFT, SURF, ORB or corners~\cite{}. In ORBSLAM3, ORB features are used. These features are defined in such a way that they are invariant to scale, rotation, translation properties i.e., for example, a corner in one image can be larger and slightly oriented in a different direction compared to the same feature in another image. At a given time instance ($t$), these features are extracted from two or more stereo frames ($V^s_t$) and are reprojected on to a real world to estimate the depth of each feature, which is used to estimate the scale of the tracking. Once the features are extracted from each stereo frame, final features are counted by matching the features across all the stereo images. The tracking module then uses these matched features to find correspondences with a previous reference image ($V^s_{t-1}$) and create a set of matching keypoints. Based on the correspondences in features between the two frames, it calculates the relative estimates in terms of the distance ($v_x$) and the heading ($v_y$) (labeled frame-to-frame alignment) between the reference keyframe and the current frame, and computes the final position.

%The other two components are related to building a map environment and thus their details are not needed for our work. 

\noindent \textbf{Challenges of directly using the relative position in fusion:} One of our goals is to eliminate the drift issues faced by the passive odometry approaches during the fusion leading to two challenges. First, when we combine these relative position estimates directly with the RF absolute location estimate, the end result from the fusion is also influenced by the long-term drift of relative estimates. Second, these relative estimates in itself are erroneous even when there is no drift, for example, short-term changes in environmental conditions can result in inaccurate short-term relative estimates and the tracking error can be up to 1m even under best visual feature rich conditions. To compensate for such inaccurate estimates, we need additional certainty metrics to provide the confidence in tracking. We address these challenges next.

\system address the first challenge by using the relative displacement in translation ($r$) and the heading ($\theta$) rather than using the final relative estimates to drive the fusion. By using the translational displacement and the heading, if when odometry loses tracking, the error propagation in displacement is transient while the direction of trajectory is captured by the heading. Together with the RF absolute estimates and these polar coordinates ($(r, \theta)$), the drift can practically vanish and result in robust tracking. To address the second challenge, we compose additional features similar to RF path, as described below.

\begin{figure}[t]
\centering
    \subfloat[Well-lit (568 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-well-lit.pdf} 
     }
    \subfloat[Dim-lit (252 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-dim-lit.pdf}  
     }
     
    \subfloat[Matches vs. Error]{%
      \includegraphics[width=\linewidth]{figs/matches-vs-error.pdf}  
     }
      \caption{VO matching keypoints (markers in green color) vs. error under different environmental conditions.}
     \label{fig:visualfeatures}
\end{figure}

\begin{figure*}[t]
\centering
      \includegraphics[width=0.9\linewidth]{figs/rovar-fusion.pdf}
      \caption{\system Hybrid Fusion.}
     \label{fig:rovarfusion}
\end{figure*} 

\smallskip
\noindent \textbf{Feature composition:} Essentially, the features extracted from the images guide the SLAM algorithm in terms of accuracy and the robustness of tracking. We dissect the tracking component and extract several certainty metrics that are directly related to the tracking performance. For example, a straightforward metric is the number of ORB features that are matched across all the stereo frames. Fundamentally, the SLAM algorithm relies on the matching features across all the stereo images. However, there can be spurious matches and outliers that can be determined based on their estimated depth and can be removed before feeding them to the tracking algorithm. After the cleaning the outliers, the final matching keypoints are used for tracking. We study the effect of matching keypoints on tracking performance under different environmental conditions and find that the tracking error is directly influenced by the number of matching keypoints. For example, Figure \ref{fig:visualfeatures} shows the number of matching keypoints under well-lit (568) and dim-lit (252) conditions qualitatively in. In Figure \ref{fig:visualfeatures}c, we quantify the impact of matching keypoints on tracking error. As shown, the error is consistent as long as the number of features are well above 500 and it suddenly spikes up when the number goes below 300 consistently for a long period of time. Note, if the matching keypoints goes below 100 for longer periods, the tracking completely fails. We leverage this metric as a certainty measure to guide our hybrid fusion. Additionally, we also find several other useful certainty metrics such as the depth of the these matching features, outliers and inliers, the reprojection error computed while reprojecting the features on to real world etc that can be used to drive the fusion.

\subsection{Sensor Fusion through Cross-Modal Attention}
% cross-modal attention background and how it is applied in \system to predict the absolute location estimate
In this section we describe our hybrid fusion approach to estimate the absolute location by leveraging RF and VO algorithmic tracking solutions presented in \S\ref{}. As discussed in \S\ref{}, \system  adopts a learning-based approach to fuse the RF and VO tracking. 

\subsubsection{Challenges of fusing active passive tracking} \system's goal is to fuse the multi-modal RF and VO tracking to obtain accurate and robust absolute tracking. There are two key challenges associated to achieve this goal. First, \system should efficiently adapt the fusion to weight sensor appropriately when the the sensors face favourable and unfavourable environmental conditions. The complementary nature of RF and VO should drive the fusion, for example, by weighting RF more than VO under dim-lit and feature less environmental conditions and similarly, weight VO more when there are a lot of NLOS anchors. Second, \system should estimate an absolute location from the active RF that gives absolute location, while the VO tracking is relative. Directly combining the absolute and relative tracking from RF and VO can lead to inefficient fusion because the relative tracking does not have the ability to recover quickly when faced with intermittent unfavourable conditions. In the following, \system addresses these two challenges. 

\subsubsection{Adaptive fusion using cross-model attention} To exploit the complementary nature of the sensors, we adopt \textit{Attention} mechanism, a commonly used technique for weighting the features to adapt the multi-modal-driven learning solutions. There are a variety of attention models in the learning literature, fore example, self attention~\cite{} and cross-model attention~\cite{} etc. The self attention weights the features of an individual sensor to self adapt and eliminate the influence of outliers. This is analogous to traditional self-filtering methods such as KF and PF described in \S\ref{}. The cross-attention model, however, weights each sensor with respect to one another. \system directly adopts the cross attention model without using self attention because the features engineering described in \S\ref{} has already in a way captures this through the correlations of features with the tracking error. Next, we provide the details of cross-model  attention.

The cross-model attention technique has been heavily used in machine learning multi-modal tasks~\cite{}. The cross attention is used to extract the inter-sensor correlations and re-weight the sensors with respect to each other. Essentially, two probability maps or masks are learned using the RF and VO features before fusing the features directly; one mask for RF and another for VO. Given the features of RF and VO as $A_r$ and $A_v$, the cross attention masks can be computed as below:

\begin{equation}
    A_{rv} = \sigma[(W^Q_{rv}z_v)^T W^\psi_{rv}z_v], 
    A_{vr} = \sigma[(W^Q_{vr}z_r)^T W^\psi_{vr}z_r]
\end{equation}

where, W are the learnable weight parameters, and $\sigma$ is nonlinear activation function. After the masks are learned, each mask is applied to respective sensor and then the masked features are merged together to fuse both the sensors and estimate the location. The fused features can be formally represented as:

\begin{equation}
    A = [A_{rv} \oplus z_v; A_{vr} \oplus z_r]
\end{equation}

\subsubsection{Absolute location estimate} As discussed in \S\ref{}, the key challenge with the relative tracking its inability to recover quickly when it loses tracking under unfavourable conditions, because of its decision based on previous positions. Isolating this limitation relative tracking and predicting the absolute location can make the tracking more resilient and quickly recover even if the VO-tracking faces unfavourable conditions frequently. \system achieves this by leveraging the estimates in translational ($r$) and rotational displacements ($\theta$) from the VO-tracking described in \S\ref{} to guide the fusion, instead of final relative position estimates.

\smallskip
\noindent \textbf{\system's end-to-end fusion and location estimation:} Figure \ref{fig:rovarfusion} shows the \system's end-to-end hybrid fusion. On the VO path, the stereo frames at two consecutive time intervals ($V_t, V_{t-1}$) are passed to the SLAM algorithm to estimate the polar coordinates ($r, \theta$) which are passed along with the extracted certainty metrics presented in \S\ref{} such as matching keypoints and additional metrics to the fusion model. On the RF path, the anchor selection model filters out anchors with poor ranging using the link quality ($L_i$) and ranges ($R_i$). The filtered ranges and their fixed locations are fed to the multi-lateration get the absolute location estimates (after filtering the anchors as described in \S\ref{}). The location estimates given by the algorithm are passed along with the ranges and received signal power estimates to fusion model. See Figure \ref{}. These features first passed through two convolutional layers to extract the correlations among the individual features and certainty metrics before applying the attention masks. The features are then merged together and passed though an RNN layer to capture the temporal correlations and estimate the absolute location. 

\subsection{Contrasting with Pure ML-driven Fusion} \label{label:bbdesign}
% talk about the pure data-driven (black-box) approach to contrast the difference in \system's approach

\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/bb-system.png}
      \caption{Blackbox Fusion.}
     \label{fig:bbdesign}
\end{figure}

In this section, we present a blackbox approach, a general learning framework for multi-modal fusion followed by recent literature~\cite{} and contrast it with \system. 

\subsubsection{Feature extraction} Most of the state-of-the-art learning-driven methods fuse the multi-modal information by directly feeding the raw input data from each sensor to a deep network and extract the features through learning. Recent solutions that follow this approach include milliEgo~\cite{} to combine mmWave and IMU, DeepTIO~\cite{} to thermal and IMU, VINET~\cite{} to combine visual and IMU data. We adopt a similar method to fuse RF and Visual data.

Figure \ref{fig:bbdesign} shows the end-to-end pure learning-based approach for fusion. For RF, input the ranges ($R_i$) as well as the link quality ($L_i$) metrics as described in \S\ref{} to an RF sub-network for feature extraction. We use two ConV1D layers to extract the latent correlations across the features followed by the three Dense layers, each block including standard Batchnorm and Dropout blocks to improve generalization. Similarly for VO, the stereo frames at two consecutive time intervals are passed to a VO sub-network to extract the features that implicitly compute the correspondences between the two images. In particular, we adopt a FlowNet~\cite{} module to estimate the optical flow between the the images for feature correspondence. The FlowNet module consists of 9 convolutional layers followed by a LeakyReLu activation function. The features extracted from this module are compact in size reducing the dimensions and capturing the temporal dependencies through time-distributed layers. 

\subsubsection{Attending the features and location estimate} Once the features are extracted from each sensor, we follow a two-stage attention mechanism proposed in \S\ref{}. This two-stage attention is proven to perform better than a mixed single-stage attention. The two-stage attention involves i) self attention, ii) cross-modal attention. The self attention is similar to self-filtering process to remove weak features before combining with other sensor features. Given, $z_v$ as the visual, $z_r$ as the RF features extracted the individual sub-networks, we learn the self attention mask/probability map based through learnable parameters as follows:

\begin{equation}
    A_{vm} = \sigma[(W^Q_v z_v)^T W^\psi_v z_v], A_{rm} = \sigma[(W^Q_r z_r)^T W^\psi_r z_r]
\end{equation}

where, the $W$ are the learnable parameters that transform the extracted features into embedding spaces $Q$ and $\psi$ respectively. The original features can be attended using the obtained masks as below:

\begin{equation}
    A_v = A_{vm} \oplus z_v, A_r = A_{rm} \oplus z_r
\end{equation}

After the features are self-attended, we follow a cross-attention and fusion pipeline similar to \system (presented in \S\ref{}).

\subsubsection{\system versus Blacbox} \system differs from the above blackbox design in three important directions--- i) algorithm-assisted generalization, ii) much of the feature extraction burden in the blackbox fusion model is driven by the algorithm, so the fusion model can optimize more on the fusion rather than extracting features, iii) \system does not require a complex network like blackbox solution to extract features and therefore can reduce the model complexity significantly. As a result, \system fusion network is lightweight and takes significantly less time for inference/predicting compared to blacbox methods.


==> design1.tex <==
\subsection{Overview of \system}
The block diagram in Fig~\ref{} shows the end-to-end architecture of \system. 
\system incorporates dual-layer diversity by (a) employing an algorithm-driven approach in the first stage to engineer features from individual RF (UWB ranges) and visual (camera frames) sensor inputs; (b) followed by a data-driven (machine learning, ML) approach for effective fusion of these complementary sensor features through a cross-attention mechanism in the second stage;	
% and (b) at another level, fuses and leverages the complementary nature of active (RF) and passive (visual) tracking sensors, 
to deliver robust and  accurate, multi-agent tracking. 

Its algorithmic component, namely multi-lateration for UWB and ORB-SLAM3 for camera inputs, allows for embedding the physical and geometrical nature of the localization problem by providing the absolute (RF) and relative (visual) position estimates directly as features. These estimates, along with other (robustness-related) features that capture sensor-specific and environmental artifacts (RF channel quality, camera inter-frame keypoints, etc.), together form a complete set of features that can also determine the certainty of the individual sensor estimates. 
This is then made possible by its ML component, which first employs a CNN encoder to extract dependencies within the individual sensor features to capture the certainty of their respective location estimates. This is followed by a cross-attention mechanism along with a 2-layer LSTM network (to capture temporal dependencies), to effectively fuse these disparate (absolute and relative) location-related features and predict the final absolute location estimate of the device with a high accuracy even under challenging environmental conditions. 

Leveraging the initial location estimates from algorithms as features, frees the ML module from the heavy-lifting needed to  capture the physical and geometrical embedding inherent to localization, allowing it to focus solely on sensor fusion, and results in two key benefits: (i) robustness and generalizability:  delivering accurate tracking even in unseen challenging environmental conditions, and (ii) real-time tracking: significantly reduces the compute-intensive nature of the end-to-end processing pipeline to enable real-time operation on resource-constrained platforms. We now discuss these two stages in detail. 

%The system consists
%of two main modules: (i) An RF module which takes the UWB ranges and received power as input, and
%(ii) A VO module which takes the raw camera images as input. The RF and the VO modules house
%multilateration and the ORB-SLAM3 algorithmic units, respectively, and a CNN encoder as shown.
%The feature output from the two modules are fed into a cross-attention fusion model. The fused
%sensor features are next sent into a Long Short-Term Memory (LSTM) module - a 2 layer RNN, which
%finally outputs the absolute location estimates. Below, we discuss each component of \system in detail.
%
%%\subsection{Overview of \system}
%\% Dual-layered fusion approach that (a) at one level, employs an algorithm-driven approach for feature engineering and a data-driven approach for fusion of the sensor features through cross-modal attention, and (b) at another level, fuses and leverages the complementary nature of active (RF) and passive (visual) tracking sensors, to deliver robust and  accurate, multi-agent tracking. Algorithmic approach allows for embedding of the physical and geometrical nature of the localization problem by providing the absolute (RF) and relative (visual) location estimates from the respective sensors as features. These estimates, along with other features specific to the sensors (RF channel quality, camera inter-frame keypoints, etc.) that in turn determine the certainty of these estimates, together form a robust set of features that drive the data-driven fusion of these sensors to predict the final absolute location estimate of the device with a high accuracy even under challenging environment conditions. Leveraging the initial location estimates from algorithms as features, alleviates the need for the data-driven fusion module to do the heavy-lifting in capturing the physical-geometrical embedding inherent to the sensors, thereby resulting in two key benefits: (i) scalability and generalizability:  delivering accurate tracking even in unseen challenging environmental conditions, and (ii) real-time tracking: significantly reduces the compute-intensive nature of the end-to-end processing pipeline to enable real-time operation. 
%
% \begin{figure}[t]
% \centering
%         \subfloat[P2P Ranging]{%
%       \includegraphics[width=0.35\linewidth]{figs/ranging-a.png} 
%      }
%         \subfloat[TWR Protocol Message Exchange]{%
%       \includegraphics[width=0.65\linewidth]{figs/ranging-b.png}  
%      }
%     % \subfloat[Trilateration]{%
%     %   \includegraphics[width=0.4\linewidth]{figs/trilateration.png}  
%     %  }
%       \caption{IEEE 802.15.4 TWR ranging protocol to measure the range between two nodes.}
%      \label{fig:extreme}
% \end{figure}

\subsection{Algorithm-driven Feature Engineering:}
The goal of this stage is to generate features that capture not only location estimates delivered by the respective sensor algorithms, but also the certainty of those estimates as impacted by sensor and environmental artifacts. 

\subsubsection{RF Module:}

\textbf{(1) Determining absolute location estimate:}
In the case of UWB, the device employs time of flight (ToF) to measure the range (i.e., distance) $R_i$ to a known anchor $i$.
Such range estimations to multiple anchors (atleast 3) or fewer number of anchors (if angular information, AoA is available) along with the location of the anchors, is sufficient for the multi-lateration algorithm to solve for the absolute location estimate of the device.  If there are $n$ anchors deployed, each with a fixed position ($x_i$, $y_i$) with $i=1..n$, the absolute 2D location of the device ($x, y$) can be estimated by minimizing the error $f_i = R_i - \sqrt{(x_i-x)^2+(y_i-y)^2}$ across the anchors. Several optimization solutions are available~\cite{} to solve the multi-lateration problem, of which \system adopts a least-squares based approach.

\begin{figure}[!h]
\centering
    \subfloat[Error vs. received power.]{%
    \includegraphics[width=0.5\linewidth]{figs/losvsnloserror.pdf}\label{fig:errorvlosnlos}
    }
    \subfloat[Best case error]{%
      \includegraphics[width=0.5\linewidth]{figs/besterror.pdf} \label{fig:besterror}
     }
    \caption{Localization error under LOS and NLOS scenarios.}
\end{figure} 


%\textbf{(2) Improving estimate by addressing NLoS impact:}
\textbf{(2) Extracting features to capture NLoS impact:}
There are two components that impact the localization accuracy: (i) multi-lateration optimization error, and (ii) environmental conditions (multipath, NLoS) that manifest as inaccurate range estimates. While the former can be estimated as a direct output of the optimization solution, the latter is challenging to address.
Recall from \S\ref{label:background} that the range estimates to NLOS anchors have a high variance, which can have a large impact on localization accuracy.  
%in range estimates event at short distances. Such inaccurate range estimates will influence the optimization to minimize its range error, and estimate a sub-optimal location. For example, 
\newline\noindent{\em Impact of NLoS:} 
We consider an indoor deployment of five anchors (testbed details in Sec~\ref{}), while the device to be located moves in a trajectory, exposing both LoS and NLoS paths to various anchors. To capture the maximum performance impact, Figure \ref{fig:errorvlosnlos} categorizes scenarios, indicating that the median error is as low as 0.2m when the device has access to all LoS anchors, compared to 1m when they are all NLoS anchors with a maximum error of 3m. For a more practical setting, we redeploy the anchors such that the device sees a mix of LoS and NLoS anchors in its trajectory. While all the anchors are used in localization in the {\em Mixed} case, only the best set of 3 anchors (out of 5), potentially LoS ones if available, are chosen for localization (by comparing with the ground truth location) in the {\em Best} case.  The 90-th percentile error shows a gain of over 0.5m between the two schemes, with the {\em Mixed} case being over a meter in error. While this suggests that filtering out NLoS anchors can bring down the error significantly, selecting the best anchors is nontrivial without knowledge of the ground truth environmental conditions, a challenge we address next.
%shows the impact of various combinations of anchors in LoS and NLoS on localization. 
%The median error is 0.2m and 1m when all anchors are under LoS and NLoS respectively. The max error for NLoS case is as high as 3m. This shows that noisy anchors with poor range estimates can result in huge localization errors.  




%The RF module of \system consists of an algorithmic component (achor selection and a multilateration solver) 
%and a CNN encoder. The input is a 2-D vector () that contains the UWB ranges to various anchjors and the
%corresponding received power (measured in dBm), measured during the UWB's two-way-ranging. While the UWB ranges 
%is used by the multilateration solver to determine the device location, the received power has a dual intent (i)First,   
%as an input to an SVM model that selects a subset of the anchor ranges that are most likely from LoS anchors (and hence accurate),
%aiding the multilateration optimizer to determine the device location more precisely, and (ii) As an input to
%the CNN encoder to determine the certainty of the location determined by the multilateration solver.
%
%\emph{UWB multilateration localization:}
%
%Accuracy of the multilateration localization depends on the accuracy of the UWB's Time-of-Flight 
%based two-way-ranging. In the presence of NLoS anchors, the ranging is erroneous. 

%\emph{CNN Feature extraction:}




%\emph{ORB-SLAM3:}

%\emph{VO CNN encoder:}


%The first stage of \system's dual-layer fusion is feature engineering from 
%individual tracking algorithms. 
%In the following, we provide the details of the feature extraction from RF and VO tracking algorithms.
%
%\subsubsection{RF Path} %selection of range estimates, algorithm details, composition of features 
%As mentioned before, we use UWB for RF tracking modality. UWB nodes use time of flight (ToF) to measure the range (i.e., distance) between two nodes by multiplying the signal's ToF with speed of light. At each time instance, the collected ranges and the respective fixed positions of the anchors (as <$location_i$, $range_i$> tuples) are fed to the multilateration algorithm and and solve for \textit{\underline{absolute location}} estimate. To estimate a 2D location, three non-collinear anchors are sufficient while more anchors may improve the estimate further. Assuming there are $n$ anchors deployed in the environment, each with fixed position ($x_i$, $y_i$) with $i=1..n$, and original location of the tag as ($x, y$), the location can be estimated by minimizing the error $f_i = R_i - \sqrt{(x_i-x)^2+(y_i-y)^2}$, where $R_i$ is the range between tag and anchor $i$. Ideally, we want the $f_i$ to be zero. Therefore, by setting the error equation to zero, we can solve for an optimal ($\mathcal{X}$, $\mathcal{Y}$) that gives overall minimum error for all anchors. 
%
%%There are a variety of optimization solutions available in the literature~\cite{}. We adopt a simple least square error optimization with geometric constraints in order to force the solutions to be in the intersection areas of all multilateration circles.
%
%\smallskip
%\noindent \textbf{Challenges of UWB Localization:} A key problem with the above direct optimization is the localization accuracy is influenced by the environmental conditions. Recall from \S\ref{label:background}, the range estimates under LOS and NLOS differ significantly, with NLOS anchors having high variance in range estimates event at short distances. Such inaccurate range estimates will influence the optimization to minimize its range error, and estimate a sub-optimal location. For example, Figure \ref{fig:errorvlosnlos} shows the impact of various combinations of anchors in LoS and NLoS on localization. The median error is 0.2m and 1m when all anchors are under LoS and NLoS respectively. The max error for NLoS case is as high as 3m. This shows that noisy anchors with poor range estimates can result in huge localization errors.  


%To ascertain this finding, we study a more practical scenario by deploying the anchors in a mixed LoS and NLoS combination. We compute the error with all the anchors (Mixed), and also under a best case. The best case error is computing by populating all possible combinations of anchors out of deployed 5 anchors having at least 3 (i.e., $5 \choose 3$=10) and selecting a best combination (approx all LoS) for each point measurement that gives minimum error when compared against the groundtruth trajectory. Figure \ref{fig:besterror} shows the difference in error with the mixed set of anchors versus best selected anchors. The median difference between both cases XXcm while the max error under best case is well under a meter. While this suggests that filtering out NLoS anchors brings down the error significantly, selecting the best anchors is nontrivial without knowing the ground truth trajectory in advance, a challenge we address next.

%One way to identify these noisy anchors is by as by \textit{learning} to select the best anchors by training the model with ranges from all the anchors offline using the available groundtruth. However, this will lead to generalization issues ....

%\noindent \textit{Selecting best anchors:} 


%The localization error mainly results from two sources--- i) from the accuracy of range estimates (recall from \S\ref{}), ii) from the algorithmic optimization when the circles of ranges of anchors do not overlap at a single location. While the algorithmic error can be obtained directly after the minimization, 

\noindent{\em Feature selection:} 
Determining the accuracy of location estimates requires an understanding of the fundamental wireless signal characteristics affecting range estimation in NLoS. As seen in Figure \ref{} in \S\ref{}, the range estimates are significantly poor under NLOS scenarios even at short distances. We investigate several link related metrics (e.g., first path power, amplitude, impulse power etc) to characterize this behavior, and find that amongst all metrics, received signal power exhibits a highly discriminative  behavior with respect to range estimates. The received signal power can be estimated using the below equation.

\begin{equation}
    P_{rx} = 10 \times \log_{10}\left({\frac{C \times 2^{17}}{N^2}}\right) - A \hspace{0.1cm}dBm
\end{equation}

where, $C$ is the Channel Impulse Response Power, $N$ is a preamble accumulation count~\cite{}, $A$ is a constant that is determined with the pulse repetition frequency~\cite{}. The constants involved are specific to Decawave's UWB chip and firmware employed for range estimation (found in~\cite{}).
Figure \ref{fig:rangevsrxp} shows the impact of range versus power under LoS and NLoS conditions for three different anchors and averaged over several device locations. As the range from the anchor increases, the received power under NLOS goes below -95dBm even within 15m, while it remains above -90dBm even after 30m for LoS. Further, this is consistent across multiple anchors. Figure \ref{fig:errorvsrxp} also shows that the received power has a strong negative correlation with localization error, with a corresponding Pearson correlation coefficient of -0.63. Thus, received power to an anchor ($P_i$) along with its range ($R_i$) can serve as an effective discriminative feature, capturing the impact of NLoS on the accuracy of its range and eventually location estimate, although with a nonlinear relationship.
%This gives us an insight in understanding the accuracy of ranging under both scenarios, although, with a nonlinear relationship. 


\textbf{(3) Leveraging RF features to address NLoS:} 
The extracted feature $\{P,R\}$, serves two purposes in \system: (i) to filter out accurate range estimates used for localization when $>3$ anchors are available, and (ii) indirectly capture the certainty (variance) of the location estimate for subsequent fusion.
% \textbf{(3) Composing feature to capture location certainty:} 

\noindent{\em (i) Anchor selection:} As the problem space involves selecting anchors from a small set (we deploy a maximum of 7 anchors in our system), \system leverages simple but explainable ML models (e.g., SVM and Logistic regression) to classify the best anchors. To this end, we derive a separate anchor classification dataset from our collected data to train a classifier that selects the best $K$ anchors for localization. We fit a model with the ranges from all anchors along with their corresponding received powers as input, and the best anchor set (providing min. error compared to ground-truth) as the output binary vector. The multi-output classification using classifier chains~\cite{}  exploits the correlation among the anchors rather than independently selecting each anchor.
%We create this dataset with best anchors offline by localizing with all possible combinations of anchors and selecting a combination that gives the minimum error when compared to the groundtruth. 
%We fit a multi-output classification model to predict the best anchor binary vector using classifier chains~\cite{} to exploit the correlation among the anchors rather than independently selecting each anchor. 
We fit three models--- SVM, Logistic Regression, and a RandomForests classifier and perform a grid search on each of them to tune the best parameters. After the grid search, we select a best performing model (SVM in our case) and its optimal parameters from the search. Figure \ref{fig:anchorselection} shows the prediction performance in terms of mean accuracy, when predicting a subset of anchors. As shown, the model performance is highly accurate with the accuracy increasing as expected when more anchors are available for selection. Note that the model only helps filter the inputs, while the multi-lateration algorithm is still responsible for estimating the location estimate.  

\begin{figure}[!h]
\centering
\begin{minipage}{.47\linewidth}
\centering
  \includegraphics[width=\linewidth]{figs/anchor-selection.pdf}
  \caption{Selecting different no of anchors out of 7.}
\end{minipage}\hspace{0.3cm}%
\begin{minipage}{.47\linewidth}
  \includegraphics[width=\linewidth]{figs/anchor-selection2.pdf}
  \caption{Selecting 3 out of different no of anchors.}
\end{minipage}
\label{fig:anchorselection}
\end{figure}

%\noindent {\em Predicting best anchors improves accuracy but not sufficient for fusion:} 
\noindent {\em (ii) Feature composition:} While anchor selection filters NLoS anchors to improve the location estimate, a device often might not have access to 3 LoS anchors.
As seen in Fig.~\ref{},  the maximum localization error is still over 1m even after selecting the best set of anchors. 
%practical deployments might not often allow room for 3 LoS anchorsmigthe multi-lateration algorithm . However, the localization error is still as high as 1m (see Figure \ref{}) even after the selecting the best anchors. Ideally, if the anchors are deployed in such a way that we can always predict at least 3 LoS anchors out of all the anchors, the location estimate from the multi-lateration algorithm is sufficiently accurate (see \ref{fig:errorvlosnlos}). However, guaranteeing LoS anchors throughout the users' trajectory is not practical. Consequently, 
Thus, employing the absolute location estimates alone can misguide the fusion framework to adapt inefficiently to different RF conditions.
Hence, \system leverages 
%the additional feature of received power for each anchor to capture the environment-dependent impact on the certainty of the range and consequently the location estimate. \system composes the absolute location 
% To counter this challenge, we need to incorporate additional features to fusion framework along with the absolute location estimate. These features should be  environment-dependent to adapt the fusion to different environmental conditions and provide a certainty measure in the location estimates. We explore a variety of certainty metrics that quantify the impact of RF environmental conditions and leverage these metrics along with the location estimates from the algorithm for the fusion.
 %We leverage these ranges and 
 the additional feature of received powers together with the ranges as a form of certainty measure (in modeling our anchors as LoS and NLoS) and combines these certainty features with the absolute location estimates from the multi-lateration algorithm as a composed RF input to our fusion framework. Formally, the input from the RF path to \system's module is given as $<\mathcal{X} \oplus R_i | P_i>, <\mathcal{Y} \oplus R_i | P_i>$, where $\oplus$ is the concatenation operation of the location estimates with the device's range and received power to each anchor.



%The localization error mainly results from two sources--- i) from the accuracy of range estimates (recall from \S\ref{}), ii) from the algorithmic optimization when the circles of ranges of anchors do not overlap at a single location. While the algorithmic error can be obtained directly after the minimization, determining the accuracy of range estimates require the understanding of fundamental signal characteristics. As shown in the Figure \ref{} in \S\ref{}, the range estimates are significantly poor under NLOS scenario compared to LOS event at shorter distances. We investigate several link related metrics (e.g., first path power, amplitude, impulse power etc) to identify this behaviour, and find that the received signal power shows complementary behaviour for range estimates. The received signal power can be estimated using the below equation.
%
%\begin{equation}
%    P_{rx} = 10 \times \log_{10}\left({\frac{C \times 2^{17}}{N^2}}\right) - A \hspace{0.1cm}dBm
%\end{equation}
%
%where, $C$ is the Channel Impulse Response Power, $N$ is a preamble accumulation count~\cite{}, $A$ is a constant that is determined with the pulse repetition frequency~\cite{}. Figure \ref{fig:rangevsrxp} shows the impact of range versus power under LoS and NLoS conditions for one anchor. The figure shows that as we move away from the anchor, the received power under NLOS goes below -95dBm within 15m whereas the power remains above -90dBm even after 30m. Furthermore, Figure \ref{fig:errorvsrxp} shows that the received power has a strong negative correlation with the localization error having a Pearson correlation coefficient of -0.63. This gives us an insight in understanding the accuracy of ranging under both scenarios, although, with a nonlinear relationship. 

 %We leverage these ranges and received power estimates together as a form of certainty measures in modeling our anchors as LoS and NLoS and combine these certainty features with the absolute location estimates from the multi-lateration algorithm as a composed RF input to our fusion framework. Formally put, the input from the RF path to our fusion is given as $<\mathcal{X} \oplus R_i | P_i, <\mathcal{Y} \oplus R_i | P_i>$, where $\oplus$ is the concatenation operation of the location estimates with the device's range and received power to each anchor.

\begin{figure}[t]
\centering
    \subfloat[Range vs. received power.]{%
      \includegraphics[width=0.5\linewidth]{figs/range_vs_rx_power.png} \label{fig:rangevsrxp}
     }
    \subfloat[Received power vs. Error]{%
      \includegraphics[width=0.5\linewidth]{figs/overall_correlation.pdf} \label{fig:errorvsrxp}
     }
     \caption{Received power vs. ranging and localization error.}
\end{figure} 

\subsubsection{VO Module:}
\textbf{(1) Determining relative position estimate:}
Most visual SLAM solutions comprise of  three key components--- i) Tracking, ii) Local Mapping, and iii) Loop closing~\cite{}. The Tracking module, which is our focus, uses a stream of stereo frames to incrementally (relatively) localize the camera/device on a frame-by-frame basis. This is accomplished by extracting unique features from the images and establishing matching keypoint correspondences between frames. Typical features can be SIFT, SURF, ORB or corners~\cite{}. \system employs ORBSLAM3, where ORB features that are invariant to scale, rotation, translation properties, are used. 
%These features are invariant to scale, rotation, translation properties, for e.g., a corner in one image can be larger and oriented in a slightly different direction compared to the same feature in another image. 
At a given time instance ($t$), these features are extracted from two or more stereo frames ($V^s_t$), reprojected on to real world to estimate the depth of each feature, which  then allows for estimating the scale of tracking. %Once the features are extracted from each stereo frame, 
Final features are counted by matching the features across all the stereo images. These matched features are used to find correspondences with a previous reference frame(s) ($V^s_{t-1}$) and create a set of matching keypoints, which are then used to %. Based on the correspondences in features between the two frames, it 
calculate the relative distance and heading (labeled frame-to-frame alignment) estimates between the two frames. %reference keyframe and the current frame, and 
These are converted to relative displacement (${\Delta x}_v,{\Delta y}_v$) to compute the current position ($x_v,y_v$). 

\textbf{(2) Improving estimate by tracking translation \& heading:}
Being a relative tracking approach, even temporary environmental artifacts (limited visual features, dynamic scenes, etc.) that degrade just a few displacement estimates, result in the continuous accumulation of errors over time. 
%Hence, when the resulting drifted $(x,y)$ position from VO is provided as input, not much benefit can be derived from fusing its estimates with those of RF's. 
%To eliminate the drift issue faced by the passive VO approache during the fusion leading to two challenges.  
Hence, when we combine VO's relative position estimate directly with UWB's absolute location estimate, the resulting fused location estimate is also impacted by the long-term drift of VO's estimates. 
%Second, these relative estimates in itself are erroneous even when there is no drift, for example, short-term changes in environmental conditions can result in inaccurate short-term relative estimates and the tracking error can be up to 1m even under best visual feature rich conditions. To compensate for such inaccurate estimates, we need additional certainty metrics to provide the confidence in tracking. We address these challenges next.

\system address this challenge by using the relative displacement in translation ($r_v$) and the heading ($\theta_v$) directly rather than using the final relative estimates of position, to drive the fusion module. Hence, even when odometry faces displacement errors temporarily, the resulting error propagation is only in displacement (heading continues tracking the absolute trajectory direction), which is transient and does not propagate. % after recovery, while the direction of trajectory is still captured by the heading. 
Further, even this transient error propagation can be completely eliminated, when its relative estimates ($r_v, \theta_v$)  are fused together with UWB's absolute location estimates ($x_u,y_u$), to result in accurate tracking.
% and these polar coordinates ($(r, \theta)$), the drift can practically vanish and result in robust tracking. To address the second challenge, we compose additional features similar to RF path, as described below.



%\subsubsection{Visual Path} % algorithm details, composition of features
%Most of the visual SLAM solutions have mainly three components--- i) Tracking, ii) Local Mapping, iii) Loop closing~\cite{}. The Tracking module uses a stream of stereo frames to incrementally localize the camera on a frame-by-frame basis. This is accomplished by extracting unique features from the images and establishing matching keypoint correspondences between frames. Typical features can be SIFT, SURF, ORB or corners~\cite{}. In ORBSLAM3, ORB features are used. These features are defined in such a way that they are invariant to scale, rotation, translation properties i.e., for example, a corner in one image can be larger and slightly oriented in a different direction compared to the same feature in another image. At a given time instance ($t$), these features are extracted from two or more stereo frames ($V^s_t$) and are reprojected on to a real world to estimate the depth of each feature, which is used to estimate the scale of the tracking. Once the features are extracted from each stereo frame, final features are counted by matching the features across all the stereo images. The tracking module then uses these matched features to find correspondences with a previous reference image ($V^s_{t-1}$) and create a set of matching keypoints. Based on the correspondences in features between the two frames, it calculates the relative estimates in terms of the distance ($v_x$) and the heading ($v_y$) (labeled frame-to-frame alignment) between the reference keyframe and the current frame, and computes the final position.
%
%The other two components are related to building a map environment and thus their details are not needed for our work. 

%\noindent \textbf{Challenges of directly using the relative position in fusion:} One of our goals is to eliminate the drift issues faced by the passive odometry approaches during the fusion leading to two challenges. First, when we combine these relative position estimates directly with the RF absolute location estimate, the end result from the fusion is also influenced by the long-term drift of relative estimates. Second, these relative estimates in itself are erroneous even when there is no drift, for example, short-term changes in environmental conditions can result in inaccurate short-term relative estimates and the tracking error can be up to 1m even under best visual feature rich conditions. To compensate for such inaccurate estimates, we need additional certainty metrics to provide the confidence in tracking. We address these challenges next.
%
%\system address the first challenge by using the relative displacement in translation ($r$) and the heading ($\theta$) rather than using the final relative estimates to drive the fusion. By using the translational displacement and the heading, if when odometry loses tracking, the error propagation in displacement is transient while the direction of trajectory is captured by the heading. Together with the RF absolute estimates and these polar coordinates ($(r, \theta)$), the drift can practically vanish and result in robust tracking. To address the second challenge, we compose additional features similar to RF path, as described below.
%
\begin{figure}[t]
\centering
    \subfloat[Well-lit (568 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-well-lit.pdf} 
     }
    \subfloat[Dim-lit (252 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-dim-lit.pdf}  
     }
     
    \subfloat[Matches vs. Error]{%
      \includegraphics[width=\linewidth]{figs/matches-vs-error.pdf}  
     }
      \caption{VO matching keypoints (markers in green color) vs. error under different environmental conditions.}
     \label{fig:visualfeatures}
\end{figure}

\begin{figure*}[t]
\centering
      \includegraphics[width=0.9\linewidth]{figs/rovar-fusion.pdf}
      \caption{\system Hybrid Fusion.}
     \label{fig:rovarfusion}
\end{figure*} 

\smallskip
\noindent \textbf{(3) Composing features to capture estimate certainty:}
Note that the relative estimates can themselves be erroneous even in the absence of any error drift.
Short-term environmental artifacts (e.g. dynamic occlusion of lighting) can result in inaccurate estimates with up to 1m error (see Fig. ~ref{}) even in best visually feature-rich environments. 
To compensate for such inaccurate estimates, \system  employs  additional features to capture the certainty of the tracking algorithm's estimate . %We address these challenges next

Recall that, the features extracted from the images determine the SLAM algorithm's tracking accuracy and  robustness. 
We dissected ORB-SLAM3's tracking component to understand the suitability of its features in capturing certainty of its estimates. 
% extracted several features that are directly related to the tracking performance. For example, 
A straightforward feature is the number of ORB features that are matched by the algorithm across all stereo frames. 
%Fundamentally, the SLAM algorithm relies on the matching features across all the stereo images. 
However, these cannot be directly used, as there can be spurious matches and outliers. The latter can be determined based on their estimated depth and  removed before feeding them to the tracking algorithm. After filtering the outliers, the final matching keypoints are the ones most relevant for tracking. We study the effect of matching keypoints on tracking performance under different environmental conditions and find that the tracking error is directly influenced by them. Figure \ref{fig:visualfeatures} shows the number of matching keypoints under well-lit (568) and dim-lit (252) conditions, whose corresponding tracking error is shown in Figure \ref{fig:visualfeatures}c.
%, we quantify the impact of matching keypoints on tracking error. As shown, 
The error is consistent with keypoints as long as they are well above 500 and spikes, when the keypoints drop below 300 consistently for a long period of time. If the  keypoints go below 100 for longer periods, the tracking completely fails. While we have also explored other additional features such as depth of matching features, outliers and inliers, reprojection error, and their  combinations, we find the matching keypoints ($M$) to best capture the certainty of the estimates delivered by the algorithm.
Hence, \system combines this certainty-capturing feature $M$ with the relative location estimates $(r,\theta)$ from ORB-SLAM3 as a composed VO input to our fusion framework. Formally, the input from the VO path to \system's module is given as $<r \oplus M>, <{\theta} \oplus M>$, where $\oplus$ is the concatenation operation.
% of the location estimates with the device's range and received power to each anchor.

% We leverage this metric as a certainty measure to guide our hybrid fusion. Additionally, we also find several other useful certainty metrics such as the depth of the these matching features, outliers and inliers, the reprojection error computed while reprojecting the features on to real world etc that can be used to drive the fusion.

\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/att-example.pdf}
      \caption{Attention mask for BB vs. RoVAR.}
     \label{fig:attexample}
\end{figure}

\subsection{Sensor Fusion through Cross-Attention}
\system uses a cross-attention (or inter-modality attention) module to complementarily fuse the feature vectors output
by the RF and VO CNN encoders (see Fig~\ref{}). The cross-attention calibrates the individual weights (i.e., importance) of the two
feature vectors based on their respective uncertainties. Intuitively, this
would mean the model would rely more on the RF location estimates when
VO encounters unfavourable environments (e.g., dim-light), and similarly, rely more on VO location estimates
in the presence of NLoS anchors.

\subsubsection{Masking attention weights:}
Why masking is necessary and how the actual masks are calculated?





\subsubsection{Why cross-attention works?}
Cross-attention works because we observe data is complementary. Point out to the graph arlier in the paper. Based on that
if we plot the attention masks, we see that the weights are indeed complementary.


\subsubsection{LSTM - Learning from the fused features:}
Output is absolute location co-ordinates.

% cross-modal attention background and how it is applied in \system to predict the absolute location estimate
%In this section we describe our hybrid fusion approach to estimate the absolute location by leveraging RF and VO algorithmic tracking solutions presented in \S\ref{}. As discussed in \S\ref{}, \system  adopts a learning-based approach to fuse the RF and VO tracking. 
%
%\subsubsection{Challenges of fusing active passive tracking} \system's goal is to fuse the multi-modal RF and VO tracking to obtain accurate and robust absolute tracking. There are two key challenges associated to achieve this goal. First, \system should efficiently adapt the fusion to weight sensor appropriately when the the sensors face favourable and unfavourable environmental conditions. The complementary nature of RF and VO should drive the fusion, for example, by weighting RF more than VO under dim-lit and feature less environmental conditions and similarly, weight VO more when there are a lot of NLOS anchors. Second, \system should estimate an absolute location from the active RF that gives absolute location, while the VO tracking is relative. Directly combining the absolute and relative tracking from RF and VO can lead to inefficient fusion because the relative tracking does not have the ability to recover quickly when faced with intermittent unfavourable conditions. In the following, \system addresses these two challenges. 
%
%\subsubsection{Adaptive fusion using cross-model attention} To exploit the complementary nature of the sensors, we adopt \textit{Attention} mechanism, a commonly used technique for weighting the features to adapt the multi-modal-driven learning solutions. There are a variety of attention models in the learning literature, fore example, self attention~\cite{} and cross-model attention~\cite{} etc. The self attention weights the features of an individual sensor to self adapt and eliminate the influence of outliers. This is analogous to traditional self-filtering methods such as KF and PF described in \S\ref{}. The cross-attention model, however, weights each sensor with respect to one another. \system directly adopts the cross attention model without using self attention because the features engineering described in \S\ref{} has already in a way captures this through the correlations of features with the tracking error. Next, we provide the details of cross-model  attention.
%
%The cross-model attention technique has been heavily used in machine learning multi-modal tasks~\cite{}. The cross attention is used to extract the inter-sensor correlations and re-weight the sensors with respect to each other. Essentially, two probability maps or masks are learned using the RF and VO features before fusing the features directly; one mask for RF and another for VO. Given the features of RF and VO as $A_r$ and $A_v$, the cross attention masks can be computed as below:
%
%\begin{equation}
%    A_{rv} = \sigma[(W^Q_{rv}z_v)^T W^\psi_{rv}z_v], 
%    A_{vr} = \sigma[(W^Q_{vr}z_r)^T W^\psi_{vr}z_r]
%\end{equation}
% 
%where, W are the learnable weight parameters, and $\sigma$ is nonlinear activation function. After the masks are learned, each mask is applied to respective sensor and then the masked features are merged together to fuse both the sensors and estimate the location. The fused features can be formally represented as:
%
%\begin{equation}
%    A = [A_{rv} \oplus z_v; A_{vr} \oplus z_r]
%\end{equation}

%\subsubsection{Absolute location estimate} As discussed in \S\ref{}, the key challenge with the relative tracking its inability to recover quickly when it loses tracking under unfavourable conditions, because of its decision based on previous positions. Isolating this limitation relative tracking and predicting the absolute location can make the tracking more resilient and quickly recover even if the VO-tracking faces unfavourable conditions frequently. \system achieves this by leveraging the estimates in translational ($r$) and rotational displacements ($\theta$) from the VO-tracking described in \S\ref{} to guide the fusion, instead of final relative position estimates.
%
%\smallskip
%\noindent \textbf{\system's end-to-end fusion and location estimation:} Figure \ref{fig:rovarfusion} shows the \system's end-to-end hybrid fusion. On the VO path, the stereo frames at two consecutive time intervals ($V_t, V_{t-1}$) are passed to the SLAM algorithm to estimate the polar coordinates ($r, \theta$) which are passed along with the extracted certainty metrics presented in \S\ref{} such as matching keypoints and additional metrics to the fusion model. On the RF path, the anchor selection model filters out anchors with poor ranging using the link quality ($L_i$) and ranges ($R_i$). The filtered ranges and their fixed locations are fed to the multi-lateration get the absolute location estimates (after filtering the anchors as described in \S\ref{}). The location estimates given by the algorithm are passed along with the ranges and received signal power estimates to fusion model. See Figure \ref{}. These features first passed through two convolutional layers to extract the correlations among the individual features and certainty metrics before applying the attention masks. The features are then merged together and passed though an RNN layer to capture the temporal correlations and estimate the absolute location. 
%
\subsection{Contrasting with Pure ML-driven Fusion} \label{label:bbdesign}
% talk about the pure data-driven (black-box) approach to contrast the difference in \system's approach

\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/bb-system.png}
      \caption{Blackbox Fusion.}
     \label{fig:bbdesign}
\end{figure}

In this section, we present a blackbox approach, a general learning framework for multi-modal fusion followed by recent literature~\cite{} and contrast it with \system. 

\subsubsection{Feature extraction} Most of the state-of-the-art learning-driven methods fuse the multi-modal information by directly feeding the raw input data from each sensor to a deep network and extract the features through learning. Recent solutions that follow this approach include milliEgo~\cite{} to combine mmWave and IMU, DeepTIO~\cite{} to thermal and IMU, VINET~\cite{} to combine visual and IMU data. We adopt a similar method to fuse RF and Visual data.

Figure \ref{fig:bbdesign} shows the end-to-end pure learning-based approach for fusion. For RF, input the ranges ($R_i$) as well as the link quality ($L_i$) metrics as described in \S\ref{} to an RF sub-network for feature extraction. We use two ConV1D layers to extract the latent correlations across the features followed by the three Dense layers, each block including standard Batchnorm and Dropout blocks to improve generalization. Similarly for VO, the stereo frames at two consecutive time intervals are passed to a VO sub-network to extract the features that implicitly compute the correspondences between the two images. In particular, we adopt a FlowNet~\cite{} module to estimate the optical flow between the the images for feature correspondence. The FlowNet module consists of 9 convolutional layers followed by a LeakyReLu activation function. The features extracted from this module are compact in size reducing the dimensions and capturing the temporal dependencies through time-distributed layers. 

\subsubsection{Attending the features and location estimate} Once the features are extracted from each sensor, we follow a two-stage attention mechanism proposed in \S\ref{}. This two-stage attention is proven to perform better than a mixed single-stage attention. The two-stage attention involves i) self attention, ii) cross-modal attention. The self attention is similar to self-filtering process to remove weak features before combining with other sensor features. Given, $z_v$ as the visual, $z_r$ as the RF features extracted the individual sub-networks, we learn the self attention mask/probability map based through learnable parameters as follows:

\begin{equation}
    A_{vm} = \sigma[(W^Q_v z_v)^T W^\psi_v z_v], A_{rm} = \sigma[(W^Q_r z_r)^T W^\psi_r z_r]
\end{equation}

where, the $W$ are the learnable parameters that transform the extracted features into embedding spaces $Q$ and $\psi$ respectively. The original features can be attended using the obtained masks as below:

\begin{equation}
    A_v = A_{vm} \oplus z_v, A_r = A_{rm} \oplus z_r
\end{equation}

After the features are self-attended, we follow a cross-attention and fusion pipeline similar to \system (presented in \S\ref{}).

\subsubsection{\system versus Blacbox} \system differs from the above blackbox design in three important directions--- i) algorithm-assisted generalization, ii) much of the feature extraction burden in the blackbox fusion model is driven by the algorithm, so the fusion model can optimize more on the fusion rather than extracting features, iii) \system does not require a complex network like blackbox solution to extract features and therefore can reduce the model complexity significantly. As a result, \system fusion network is lightweight and takes significantly less time for inference/predicting compared to blacbox methods.


==> design2.tex <==
\subsection{Overview of \system}
The block diagram in Fig~\ref{fig:rovarfusion} shows the end-to-end architecture of \system. 
\system incorporates dual-layer diversity by (a) employing an algorithm-driven approach in the first stage to engineer features from individual RF (UWB ranges) and visual (camera frames) sensor inputs; (b) followed by a data-driven (machine learning, ML) approach for effective fusion of these complementary sensor features through a cross-attention mechanism in the second stage;	
% and (b) at another level, fuses and leverages the complementary nature of active (RF) and passive (visual) tracking sensors, 
to deliver robust and  accurate, multi-agent tracking. 

Its algorithmic component, namely multi-lateration for UWB and ORB-SLAM3 for camera inputs, allows for embedding the physical and geometrical nature of the localization problem by providing the absolute (RF) and relative (visual) position estimates directly as features. These estimates, along with other (robustness-related) features that capture sensor-specific and environmental artifacts (RF channel quality, camera inter-frame keypoints, etc.), together form a complete set of features that can also determine the certainty of the individual sensor estimates. 
This is then made possible by its ML component, which first employs a CNN encoder to extract dependencies within the individual sensor features to capture the certainty of their respective location estimates. This is followed by a cross-attention mechanism along with a 2-layer LSTM network (to capture temporal dependencies), to effectively fuse these disparate (absolute and relative) location-related features and predict the final absolute location estimate of the device with a high accuracy even under challenging environmental conditions. Estimating a device's {\em absolute} location estimate, allows \system to easily scale to multi-agent collaborative applications, where all agents are tracked within a common frame of reference. 

Leveraging the initial location estimates from algorithms as features, frees the ML module from the heavy-lifting needed to  capture the physical and geometrical embedding inherent to localization, allowing it to focus solely on sensor fusion, and results in two key benefits: (i) robustness and generalizability:  delivering accurate tracking even in unseen challenging environmental conditions, and (ii) real-time tracking: significantly reduces the compute-intensive nature of the end-to-end processing pipeline to enable real-time operation on resource-constrained platforms. We now discuss these two stages in detail from the perspective of a single agent. 

%The system consists
%of two main modules: (i) An RF module which takes the UWB ranges and received power as input, and
%(ii) A VO module which takes the raw camera images as input. The RF and the VO modules house
%multilateration and the ORB-SLAM3 algorithmic units, respectively, and a CNN encoder as shown.
%The feature output from the two modules are fed into a cross-attention fusion model. The fused
%sensor features are next sent into a Long Short-Term Memory (LSTM) module - a 2 layer RNN, which
%finally outputs the absolute location estimates. Below, we discuss each component of \system in detail.
%
%%\subsection{Overview of \system}
%\% Dual-layered fusion approach that (a) at one level, employs an algorithm-driven approach for feature engineering and a data-driven approach for fusion of the sensor features through cross-modal attention, and (b) at another level, fuses and leverages the complementary nature of active (RF) and passive (visual) tracking sensors, to deliver robust and  accurate, multi-agent tracking. Algorithmic approach allows for embedding of the physical and geometrical nature of the localization problem by providing the absolute (RF) and relative (visual) location estimates from the respective sensors as features. These estimates, along with other features specific to the sensors (RF channel quality, camera inter-frame keypoints, etc.) that in turn determine the certainty of these estimates, together form a robust set of features that drive the data-driven fusion of these sensors to predict the final absolute location estimate of the device with a high accuracy even under challenging environment conditions. Leveraging the initial location estimates from algorithms as features, alleviates the need for the data-driven fusion module to do the heavy-lifting in capturing the physical-geometrical embedding inherent to the sensors, thereby resulting in two key benefits: (i) scalability and generalizability:  delivering accurate tracking even in unseen challenging environmental conditions, and (ii) real-time tracking: significantly reduces the compute-intensive nature of the end-to-end processing pipeline to enable real-time operation. 
%
% \begin{figure}[t]
% \centering
%         \subfloat[P2P Ranging]{%
%       \includegraphics[width=0.35\linewidth]{figs/ranging-a.png} 
%      }
%         \subfloat[TWR Protocol Message Exchange]{%
%       \includegraphics[width=0.65\linewidth]{figs/ranging-b.png}  
%      }
%     % \subfloat[Trilateration]{%
%     %   \includegraphics[width=0.4\linewidth]{figs/trilateration.png}  
%     %  }
%       \caption{IEEE 802.15.4 TWR ranging protocol to measure the range between two nodes.}
%      \label{fig:extreme}
% \end{figure}

\subsection{Algorithm-driven Feature Engineering:}
The goal of this stage is to generate features that capture not only location estimates delivered by the respective sensor algorithms, but also the certainty of those estimates as impacted by sensor and environmental artifacts. 

\subsubsection{RF Module:} \label{sec:rfmodule}

\textbf{(1) Determining absolute location estimate:}
In the case of UWB, the device employs time of flight (ToF) to measure the range (i.e., distance) $R_i$ to a known anchor $i$.
Such range estimations to multiple anchors (atleast 3) or fewer number of anchors (if angular information, AoA is available) along with the location of the anchors, is sufficient for the multi-lateration algorithm to solve for the absolute location estimate of the device.  If there are $n$ anchors deployed, each with a fixed position ($x_i$, $y_i$) with $i=1..n$, the absolute 2D location of the device ($x, y$) can be estimated by minimizing the error $f_i = R_i - \sqrt{(x_i-x)^2+(y_i-y)^2}$ across the anchors. Several optimization solutions are available~\cite{jayashree2006accuracy, cheung2006constrained, hua2014geometrical} to solve the multi-lateration problem, of which \system adopts a least-squares based approach.

\begin{figure}[!h]
\centering
\vspace{-0.2cm}
    \subfloat[Error vs. received power.]{%
    \includegraphics[width=0.5\linewidth]{figs/losvsnloserror.pdf}\label{fig:errorvlosnlos}
    }
    \subfloat[Best case error]{%
      \includegraphics[width=0.5\linewidth]{figs/besterror.pdf} \label{fig:besterror}
     }
    \caption{Localization error under LOS and NLOS scenarios.}
    \vspace{-0.2cm}
\end{figure} 


%\textbf{(2) Improving estimate by addressing NLoS impact:}
\textbf{(2) Extracting features to capture NLoS impact:}
There are two components that impact the localization accuracy: (i) multi-lateration optimization error, and (ii) environmental conditions (multipath, NLoS) that manifest as inaccurate range estimates. While the former can be estimated as a direct output of the optimization solution, the latter is challenging to address.
Recall from \S\ref{sec:background} that the range estimates to NLOS anchors have a high variance, which can have a large impact on localization accuracy.  
%in range estimates event at short distances. Such inaccurate range estimates will influence the optimization to minimize its range error, and estimate a sub-optimal location. For example, 
\newline\noindent{\em \underline{Impact of NLoS:}} 
We consider an indoor deployment of five anchors (testbed details in Sec~\ref{IMPL}), while the device to be located moves in a trajectory, exposing both LoS and NLoS paths to various anchors. To capture the maximum performance impact, Figure \ref{fig:errorvlosnlos} categorizes scenarios, indicating that the median error is as low as 0.2m when the device has access to all LoS anchors, compared to 1m when they are all NLoS anchors with a maximum error of 3m. For a more practical setting, we redeploy the anchors such that the device sees a mix of LoS and NLoS anchors in its trajectory. While all the anchors are used in localization in the {\em Mixed} case, only the best set of 3 anchors (out of 5), potentially LoS ones if available, are chosen for localization (by comparing with the ground truth location) in the {\em Best} case.  The 90-th percentile error shows a gain of over 0.5m between the two schemes, with the {\em Mixed} case being over a meter in error. While this suggests that filtering out NLoS anchors can bring down the error significantly, selecting the best anchors is nontrivial without knowledge of the ground truth environmental conditions, a challenge we address next.
%shows the impact of various combinations of anchors in LoS and NLoS on localization. 
%The median error is 0.2m and 1m when all anchors are under LoS and NLoS respectively. The max error for NLoS case is as high as 3m. This shows that noisy anchors with poor range estimates can result in huge localization errors.  




%The RF module of \system consists of an algorithmic component (achor selection and a multilateration solver) 
%and a CNN encoder. The input is a 2-D vector () that contains the UWB ranges to various anchjors and the
%corresponding received power (measured in dBm), measured during the UWB's two-way-ranging. While the UWB ranges 
%is used by the multilateration solver to determine the device location, the received power has a dual intent (i)First,   
%as an input to an SVM model that selects a subset of the anchor ranges that are most likely from LoS anchors (and hence accurate),
%aiding the multilateration optimizer to determine the device location more precisely, and (ii) As an input to
%the CNN encoder to determine the certainty of the location determined by the multilateration solver.
%
%\emph{UWB multilateration localization:}
%
%Accuracy of the multilateration localization depends on the accuracy of the UWB's Time-of-Flight 
%based two-way-ranging. In the presence of NLoS anchors, the ranging is erroneous. 

%\emph{CNN Feature extraction:}




%\emph{ORB-SLAM3:}

%\emph{VO CNN encoder:}


%The first stage of \system's dual-layer fusion is feature engineering from 
%individual tracking algorithms. 
%In the following, we provide the details of the feature extraction from RF and VO tracking algorithms.
%
%\subsubsection{RF Path} %selection of range estimates, algorithm details, composition of features 
%As mentioned before, we use UWB for RF tracking modality. UWB nodes use time of flight (ToF) to measure the range (i.e., distance) between two nodes by multiplying the signal's ToF with speed of light. At each time instance, the collected ranges and the respective fixed positions of the anchors (as <$location_i$, $range_i$> tuples) are fed to the multilateration algorithm and and solve for \textit{\underline{absolute location}} estimate. To estimate a 2D location, three non-collinear anchors are sufficient while more anchors may improve the estimate further. Assuming there are $n$ anchors deployed in the environment, each with fixed position ($x_i$, $y_i$) with $i=1..n$, and original location of the tag as ($x, y$), the location can be estimated by minimizing the error $f_i = R_i - \sqrt{(x_i-x)^2+(y_i-y)^2}$, where $R_i$ is the range between tag and anchor $i$. Ideally, we want the $f_i$ to be zero. Therefore, by setting the error equation to zero, we can solve for an optimal ($\mathcal{X}$, $\mathcal{Y}$) that gives overall minimum error for all anchors. 
%
%%There are a variety of optimization solutions available in the literature~\cite{}. We adopt a simple least square error optimization with geometric constraints in order to force the solutions to be in the intersection areas of all multilateration circles.
%
%\smallskip
%\noindent \textbf{Challenges of UWB Localization:} A key problem with the above direct optimization is the localization accuracy is influenced by the environmental conditions. Recall from \S\ref{label:background}, the range estimates under LOS and NLOS differ significantly, with NLOS anchors having high variance in range estimates event at short distances. Such inaccurate range estimates will influence the optimization to minimize its range error, and estimate a sub-optimal location. For example, Figure \ref{fig:errorvlosnlos} shows the impact of various combinations of anchors in LoS and NLoS on localization. The median error is 0.2m and 1m when all anchors are under LoS and NLoS respectively. The max error for NLoS case is as high as 3m. This shows that noisy anchors with poor range estimates can result in huge localization errors.  


%To ascertain this finding, we study a more practical scenario by deploying the anchors in a mixed LoS and NLoS combination. We compute the error with all the anchors (Mixed), and also under a best case. The best case error is computing by populating all possible combinations of anchors out of deployed 5 anchors having at least 3 (i.e., $5 \choose 3$=10) and selecting a best combination (approx all LoS) for each point measurement that gives minimum error when compared against the groundtruth trajectory. Figure \ref{fig:besterror} shows the difference in error with the mixed set of anchors versus best selected anchors. The median difference between both cases XXcm while the max error under best case is well under a meter. While this suggests that filtering out NLoS anchors brings down the error significantly, selecting the best anchors is nontrivial without knowing the ground truth trajectory in advance, a challenge we address next.

%One way to identify these noisy anchors is by as by \textit{learning} to select the best anchors by training the model with ranges from all the anchors offline using the available groundtruth. However, this will lead to generalization issues ....

%\noindent \textit{Selecting best anchors:} 


%The localization error mainly results from two sources--- i) from the accuracy of range estimates (recall from \S\ref{}), ii) from the algorithmic optimization when the circles of ranges of anchors do not overlap at a single location. While the algorithmic error can be obtained directly after the minimization, 

\noindent{\em \underline{Feature selection:}} 
Determining the accuracy of location estimates requires an understanding of the fundamental wireless signal characteristics affecting range estimation in NLoS. As seen in Figure \ref{fig:nlosvsranging} in \S\ref{MOTIV}, the range estimates are significantly poor under NLOS scenarios even at short distances. We investigate several link related metrics (e.g., first path power, amplitude, impulse power etc) to characterize this behavior, and find that amongst all metrics, received signal power exhibits a highly discriminative  behavior with respect to range estimates. The received signal power can be estimated using the below equation.
\begin{equation}
    P_{rx} = 10 \times \log_{10}\left({\frac{C \times 2^{17}}{N^2}}\right) - A \hspace{0.1cm}dBm
\end{equation}
where, $C$ is the Channel Impulse Response Power, $N$ is a preamble accumulation count used to normalize the
amplitude of channel
impulse responses~\cite{gururaj2017real}, $A$ is a constant that is determined with the pulse repetition 
frequency. These constants are specific to Decawave's UWB chip and firmware employed for range estimation (found in~\cite{dw1000}).
Fig.~\ref{fig:rangevsrxp} shows the impact of range versus power under LoS and NLoS conditions for three 
different anchors and averaged over several device locations. As the range from the anchor increases, 
the received power under NLOS goes below -95dBm even within 15m, while it remains above -90dBm even 
after 30m for LoS. Further, this is consistent across multiple anchors. Fig.~\ref{fig:errorvsrxp} 
also shows that the received power has a strong negative correlation with localization error, 
with a corresponding Pearson correlation coefficient of -0.63. Thus, received power to an anchor ($P_i$) 
along with its range ($R_i$) can serve as an effective discriminative feature, capturing the impact 
of NLoS on the accuracy of its range and eventually location estimate, although with a nonlinear relationship.
%This gives us an insight in understanding the accuracy of ranging under both scenarios, although, with a nonlinear relationship. 

\begin{figure}[t]
\centering
\begin{minipage}{.47\linewidth}
\centering
  \includegraphics[width=\linewidth]{figs/anchor-selection.pdf}
  \vspace{-0.5cm}
  \caption{Selecting different no of anchors out of 7.}
  \label{fig:anchorselection1}
\end{minipage}\hspace{0.3cm}%
\begin{minipage}{.47\linewidth}
  \includegraphics[width=\linewidth]{figs/anchor-selection2.pdf}
  \vspace{-0.5cm}
  \caption{Selecting 3 out of different no of anchors.}
  \label{fig:anchorselection2}
\end{minipage}
\vspace{-0.2cm}
\end{figure}
\begin{figure}[t]
\centering
\vspace{-0.2cm}
    \subfloat[Range vs. received power.]{%
      \includegraphics[width=0.5\linewidth]{figs/range_vs_rx_power.png} \label{fig:rangevsrxp}
     }
    \subfloat[Received power vs. Error]{%
      \includegraphics[width=0.5\linewidth]{figs/overall_correlation.pdf} \label{fig:errorvsrxp}
     }
     \vspace{-0.4cm}
     \caption{Received power vs. ranging and localization error.}
\vspace{-0.2cm}
\end{figure} 

\textbf{(3) Leveraging RF features to address NLoS:} 
The extracted feature $\{P,R\}$, serves two purposes in \system: (i) to filter out accurate range estimates used for localization when $>3$ anchors are available, and (ii) indirectly capture the certainty (variance) of the location estimate for subsequent fusion.
% \textbf{(3) Composing feature to capture location certainty:} 

\noindent{\em (i) \underline{Anchor selection:}} As the problem space involves selecting anchors from a small set (we deploy a maximum of 7 anchors in our system), \system leverages simple but explainable ML models (e.g., SVM and Logistic regression) to classify the best anchors. To this end, we derive a separate anchor classification dataset from our collected data to train a classifier that selects the best $K$ anchors for localization. We fit a model with the ranges from all anchors along with their corresponding received powers as input, and the best anchor set (providing min. error compared to ground-truth) as the output binary vector. The multi-output classification using classifier chains~\cite{read2015scalable}  exploits the correlation among the anchors rather than independently selecting each anchor.
%We create this dataset with best anchors offline by localizing with all possible combinations of anchors and selecting a combination that gives the minimum error when compared to the groundtruth. 
%We fit a multi-output classification model to predict the best anchor binary vector using classifier chains~\cite{} to exploit the correlation among the anchors rather than independently selecting each anchor. 
We fit three models--- SVM, Logistic Regression, and a RandomForests classifier and perform a grid search on each of them to tune the best parameters. After the grid search, we select a best performing model (SVM in our case) and its optimal parameters from the search. Figure \ref{fig:anchorselection1} and \ref{fig:anchorselection2} shows the prediction performance in terms of mean accuracy, when predicting a subset of anchors. As shown, the model performance is highly accurate with the accuracy increasing as expected when more anchors are available for selection. Note that the model only helps filter the inputs ($K=3$ in \system), while the multi-lateration algorithm is still responsible for estimating the location estimate.  

\begin{figure}[t]
\centering
     \vspace{-0.2cm}
    \subfloat[Well-lit (568 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-well-lit.pdf} 
     }
    \subfloat[Dim-lit (252 matches)]{%
      \includegraphics[width=0.48\linewidth]{figs/vo-matches-dim-lit.pdf}  
     }
     
     \vspace{-0.2cm}
    \subfloat[Matches vs. Error]{%
      \includegraphics[width=0.9\linewidth]{figs/matches-vs-error.pdf}  
     } 
     \vspace{-0.4cm}
      \caption{VO matching keypoints (markers in green color) vs. error under different environmental conditions.}
     \label{fig:visualfeatures}
\vspace{-0.2cm}
\end{figure}

\begin{figure*}[t]
\centering
\vspace{-0.2cm}
      \includegraphics[width=0.9\linewidth]{figs/rovar-fusion.pdf}
\vspace{-0.4cm}
      \caption{\system Hybrid Fusion.}
     \label{fig:rovarfusion}
\vspace{-0.2cm}
\end{figure*} 


%\noindent {\em Predicting best anchors improves accuracy but not sufficient for fusion:} 
\noindent {\em (ii) \underline{Feature composition:}} While anchor selection filters NLoS anchors to improve the location estimate, a device often might not have access to 3 LoS anchors.
As seen in Fig.~\ref{fig:errorvlosnlos},  the maximum localization error is still over 1m even after selecting the best set of anchors. 
%practical deployments might not often allow room for 3 LoS anchorsmigthe multi-lateration algorithm . However, the localization error is still as high as 1m (see Figure \ref{}) even after the selecting the best anchors. Ideally, if the anchors are deployed in such a way that we can always predict at least 3 LoS anchors out of all the anchors, the location estimate from the multi-lateration algorithm is sufficiently accurate (see \ref{fig:errorvlosnlos}). However, guaranteeing LoS anchors throughout the users' trajectory is not practical. Consequently, 
Thus, employing the absolute location estimates alone can misguide the fusion framework to adapt inefficiently to different RF conditions.
Hence, \system leverages 
%the additional feature of received power for each anchor to capture the environment-dependent impact on the certainty of the range and consequently the location estimate. \system composes the absolute location 
% To counter this challenge, we need to incorporate additional features to fusion framework along with the absolute location estimate. These features should be  environment-dependent to adapt the fusion to different environmental conditions and provide a certainty measure in the location estimates. We explore a variety of certainty metrics that quantify the impact of RF environmental conditions and leverage these metrics along with the location estimates from the algorithm for the fusion.
 %We leverage these ranges and 
 the additional feature of received powers together with the ranges as a form of certainty measure (in modeling our anchors as LoS and NLoS) and combines these certainty features with the absolute location estimates from the multi-lateration algorithm as a composed RF input to our fusion framework. Formally, the input from the RF path to \system's module is given as $F_r$ = $<{X_u} \oplus P_i | R_i>, <{Y_u} \oplus P_i | R_i>$, $i\in[1,K]$, where $\oplus$ is the concatenation operation of the location estimates with the device's range and received power to each anchor.

%The localization error mainly results from two sources--- i) from the accuracy of range estimates (recall from \S\ref{}), ii) from the algorithmic optimization when the circles of ranges of anchors do not overlap at a single location. While the algorithmic error can be obtained directly after the minimization, determining the accuracy of range estimates require the understanding of fundamental signal characteristics. As shown in the Figure \ref{} in \S\ref{}, the range estimates are significantly poor under NLOS scenario compared to LOS event at shorter distances. We investigate several link related metrics (e.g., first path power, amplitude, impulse power etc) to identify this behaviour, and find that the received signal power shows complementary behaviour for range estimates. The received signal power can be estimated using the below equation.
%
%\begin{equation}
%    P_{rx} = 10 \times \log_{10}\left({\frac{C \times 2^{17}}{N^2}}\right) - A \hspace{0.1cm}dBm
%\end{equation}
%
%where, $C$ is the Channel Impulse Response Power, $N$ is a preamble accumulation count~\cite{}, $A$ is a constant that is determined with the pulse repetition frequency~\cite{}. Figure \ref{fig:rangevsrxp} shows the impact of range versus power under LoS and NLoS conditions for one anchor. The figure shows that as we move away from the anchor, the received power under NLOS goes below -95dBm within 15m whereas the power remains above -90dBm even after 30m. Furthermore, Figure \ref{fig:errorvsrxp} shows that the received power has a strong negative correlation with the localization error having a Pearson correlation coefficient of -0.63. This gives us an insight in understanding the accuracy of ranging under both scenarios, although, with a nonlinear relationship. 

 %We leverage these ranges and received power estimates together as a form of certainty measures in modeling our anchors as LoS and NLoS and combine these certainty features with the absolute location estimates from the multi-lateration algorithm as a composed RF input to our fusion framework. Formally put, the input from the RF path to our fusion is given as $<\mathcal{X} \oplus R_i | P_i, <\mathcal{Y} \oplus R_i | P_i>$, where $\oplus$ is the concatenation operation of the location estimates with the device's range and received power to each anchor.

\subsubsection{VO Module:} \label{sec:vomodule}
\textbf{(1) Determining relative position estimate:}
Most vSLAM solutions comprise of  three key components--- i) Tracking, ii) Local Mapping, and iii) Loop 
closing~\cite{campos2021orb, mur2017orb, labbe2014online}. The Tracking module, which is our focus, 
uses a stream of stereo frames to incrementally (relatively) localize the camera/device on a frame-by-frame basis, 
by extracting unique features from the images and establishing matching keypoint correspondences between frames. 
Typical features can be SIFT, SURF, ORB or corners~\cite{rublee2011orb}. \system employs ORBSLAM3, where ORB features 
that are invariant to scale, rotation, translation properties, are used. 
%These features are invariant to scale, rotation, translation properties, for e.g., a corner in one image can be larger and oriented in a slightly different direction compared to the same feature in another image. 
At a given time instance ($t$), these features are extracted from two or more stereo frames ($V^s_t$), reprojected onto the real world to estimate the depth of each feature, which  then allows for estimating the scale of tracking. %Once the features are extracted from each stereo frame, 
Final features are counted by matching the features across all the stereo images. These matched features are used to find correspondences with a previous reference frame(s) ($V^s_{t-1}$) and create a set of matching keypoints, which are then used to %. Based on the correspondences in features between the two frames, it 
calculate the relative distance and heading (labeled frame-to-frame alignment) estimates between the two frames. %reference keyframe and the current frame, and 
These are converted to relative displacement (${\Delta x}_v,{\Delta y}_v$) to compute the current position ($x_v,y_v$). 

\textbf{(2) Improving estimate by tracking translation \& heading:}
Being a relative tracking approach, even temporary environmental artifacts (limited visual features, dynamic scenes, etc.) that degrade just a few displacement estimates, result in the continuous accumulation of errors over time. 
%Hence, when the resulting drifted $(x,y)$ position from VO is provided as input, not much benefit can be derived from fusing its estimates with those of RF's. 
%To eliminate the drift issue faced by the passive VO approache during the fusion leading to two challenges.  
Hence, when we combine VO's relative position estimate directly with UWB's absolute location estimate, the resulting fused location estimate is also impacted by the long-term drift of VO's estimates. 
%Second, these relative estimates in itself are erroneous even when there is no drift, for example, short-term changes in environmental conditions can result in inaccurate short-term relative estimates and the tracking error can be up to 1m even under best visual feature rich conditions. To compensate for such inaccurate estimates, we need additional certainty metrics to provide the confidence in tracking. We address these challenges next.

\system address this challenge by using the relative displacement in translation ($r_v$) and the heading ($\theta_v$) directly rather than using the final relative estimates of position, to drive the fusion module. Hence, even when odometry faces displacement errors temporarily, the resulting error propagation is only in displacement (heading continues tracking the absolute trajectory direction), which is transient and does not propagate. % after recovery, while the direction of trajectory is still captured by the heading. 
Further, even this transient error propagation is completely eliminated, when its relative estimates ($r_v, \theta_v$)  are fused together with UWB's absolute location estimates ($x_u,y_u$), to result in accurate tracking.
% and these polar coordinates ($(r, \theta)$), the drift can practically vanish and result in robust tracking. To address the second challenge, we compose additional features similar to RF path, as described below.



%\subsubsection{Visual Path} % algorithm details, composition of features
%Most of the visual SLAM solutions have mainly three components--- i) Tracking, ii) Local Mapping, iii) Loop closing~\cite{}. The Tracking module uses a stream of stereo frames to incrementally localize the camera on a frame-by-frame basis. This is accomplished by extracting unique features from the images and establishing matching keypoint correspondences between frames. Typical features can be SIFT, SURF, ORB or corners~\cite{}. In ORBSLAM3, ORB features are used. These features are defined in such a way that they are invariant to scale, rotation, translation properties i.e., for example, a corner in one image can be larger and slightly oriented in a different direction compared to the same feature in another image. At a given time instance ($t$), these features are extracted from two or more stereo frames ($V^s_t$) and are reprojected on to a real world to estimate the depth of each feature, which is used to estimate the scale of the tracking. Once the features are extracted from each stereo frame, final features are counted by matching the features across all the stereo images. The tracking module then uses these matched features to find correspondences with a previous reference image ($V^s_{t-1}$) and create a set of matching keypoints. Based on the correspondences in features between the two frames, it calculates the relative estimates in terms of the distance ($v_x$) and the heading ($v_y$) (labeled frame-to-frame alignment) between the reference keyframe and the current frame, and computes the final position.
%
%The other two components are related to building a map environment and thus their details are not needed for our work. 

%\noindent \textbf{Challenges of directly using the relative position in fusion:} One of our goals is to eliminate the drift issues faced by the passive odometry approaches during the fusion leading to two challenges. First, when we combine these relative position estimates directly with the RF absolute location estimate, the end result from the fusion is also influenced by the long-term drift of relative estimates. Second, these relative estimates in itself are erroneous even when there is no drift, for example, short-term changes in environmental conditions can result in inaccurate short-term relative estimates and the tracking error can be up to 1m even under best visual feature rich conditions. To compensate for such inaccurate estimates, we need additional certainty metrics to provide the confidence in tracking. We address these challenges next.
%
%\system address the first challenge by using the relative displacement in translation ($r$) and the heading ($\theta$) rather than using the final relative estimates to drive the fusion. By using the translational displacement and the heading, if when odometry loses tracking, the error propagation in displacement is transient while the direction of trajectory is captured by the heading. Together with the RF absolute estimates and these polar coordinates ($(r, \theta)$), the drift can practically vanish and result in robust tracking. To address the second challenge, we compose additional features similar to RF path, as described below.
%

\smallskip
\noindent \textbf{(3) Composing features to capture estimate certainty:}
Note that the relative estimates can themselves be erroneous even in the absence of any error drift.
Short-term environmental artifacts (e.g. dynamic occlusion of lighting) can result in inaccurate estimates with up to 1m error (see Fig. ~\ref{fig:comprehensive-seen}) even in best visually feature-rich environments. 
To compensate for such inaccurate estimates, \system  employs  additional features to capture the certainty of the tracking algorithm's estimate . %We address these challenges next

Recall that, the features extracted from the images determine the SLAM algorithm's tracking accuracy and  robustness. 
We dissected ORB-SLAM3's tracking component to understand the suitability of its features in capturing certainty of its estimates. 
% extracted several features that are directly related to the tracking performance. For example, 
A straightforward feature is the number of ORB features that are matched by the algorithm across all stereo frames. 
%Fundamentally, the SLAM algorithm relies on the matching features across all the stereo images. 
However, these cannot be directly used, as there can be spurious matches and outliers. The latter can be determined based on their estimated depth and  removed before feeding them to the tracking algorithm. After filtering the outliers, the final matching keypoints are the ones most relevant for tracking. We study the effect of matching keypoints on tracking performance under different environmental conditions and find that the tracking error is directly influenced by them. Figure \ref{fig:visualfeatures} shows the number of matching keypoints under well-lit (568) and dim-lit (252) conditions, whose corresponding tracking error is shown in Figure \ref{fig:visualfeatures}c.
%, we quantify the impact of matching keypoints on tracking error. As shown, 
The error is consistent with keypoints as long as they are well above 500 and spikes, when the keypoints drop below 300 consistently for a long period of time. If the  keypoints go below 100 for longer periods, the tracking completely fails. While we have also explored other additional features such as depth of matching features, outliers and inliers, reprojection error, and their  combinations, we find the matching keypoints ($M$) to best capture the certainty of the estimates delivered by the algorithm.
Hence, \system combines this certainty-capturing feature $M$ with the relative location estimates $(r,\theta)$ from ORB-SLAM3 as a composed VO input to our fusion framework. Formally, the input from the VO path to \system's module is given as $F_v$ = $<r \oplus M>, <{\theta} \oplus M>$, where $\oplus$ is the concatenation operation.
% of the location estimates with the device's range and received power to each anchor.

% We leverage this metric as a certainty measure to guide our hybrid fusion. Additionally, we also find several other useful certainty metrics such as the depth of the these matching features, outliers and inliers, the reprojection error computed while reprojecting the features on to real world etc that can be used to drive the fusion.

\subsection{Sensor Fusion through Cross-Attention}
 \system first prepares the composed features from individual sensors by passing them through a simple CNN network.
 This allows the location and its certainty-related features to be embedded into a more representative feature (capturing both estimate and its certainty) that can enable effective fusion. 
 
 \system then adopts an \textit{Attention} mechanism for fusion, a commonly used learning technique~\cite{vaswani2017attention, wang2018non}, for adaptively weighting the features of the sensors, so as to leverage their complementary nature. %self attention~\cite{} and cross-model attention~\cite{} etc. The
 While self attention~\cite{lee2019self} weights the features of an individual sensor to self-adapt and eliminate the influence of outliers (analogous to traditional filtering methods such as KF and PF, \S\ref{MOTIV}), cross-attention~\cite{lu2020milliego}, focuses on weighting each sensor with respect to one another to extract inter-sensor correlations and leverage their complementary nature. Intuitively, the model would weight the RF estimates (with higher certainty) more when VO encounters unfavorable environments (e.g., dim-light; lower certainty of VO estimate), and the VO estimates more when RF estimates suffer from NLoS anchors.
\system directly adopts cross-attention since the features engineered by its algorithms already capture self-attention (incorporating features that correlate with tracking error). 
 
%The cross-model attention technique has been heavily used in machine learning multi-modal tasks~\cite{}. The cross attention is used to extract the inter-sensor correlations and re-weight the sensors with respect to each other. Essentially, 
Two cross-attention (probability) masks ($A_{rv}$, $A_{vr}$) are {\em jointly} learned using the RF 
and VO features ($F_r$, $F_v$) respectively. %; one mask for RF and another for VO. 
%Given the features of RF and VO as $z_r$ and $z_v$, the cross attention masks can be computed as below:
\begin{equation}
    A_{rv} = Sigmoid((W'_{rv}F_v)^T W''_{rv}F_v), 
    A_{vr} = Sigmoid((W'_{vr}F_r)^T W''_{vr}F_r)
\end{equation}
where, $W'$ and $W''$ are the weights learned during the training, which transform the extracted features into a lower dimension version of original inputs from RF and VO, that extracts the underlying 
global topology of data. On a high level, the equation captures meaningful features through local convolutions
and long term dependencies through embedding spaces, jointly adapting the masks by capturing cross-correlations
between the two sensors. After the masks are learned, each mask is applied to its respective sensor feature 
(element-wise, $\odot$) and then the masked features are merged (concatenated, $\oplus$) together to provide the fused feature.
% to fuse both the sensors and estimate the location. The fused features can be formally represented as:
\begin{equation}
    A = [A_{rv} \odot F_v] \oplus [A_{vr} \odot F_r]
\end{equation}
Finally, the output from cross-attention, which is a single dimension flattened array,  is  
forwarded to an LSTM network - a 2 layer RNN (with 64 hidden units per layer) to model the temporal 
dependency of the fused features, followed by 
%The output of the LSTM is next fed into 
2 Fully Connected (FC) layers that finally outputs the predicted absolute location.
The LSTM's ability to access its outputs from prior time instants (i.e., prior absolute
location estimates), enables it to effectively predict {\em absolute} location estimate
while relying on the {\em relative} location estimate from VO (when RF features have large uncertainty), 
thereby eliminating (resetting) potential VO drifts.
% based on the relative location estimates from VO alone, whenever RF features have large uncertainties.

\begin{figure}[t]
\centering
      \includegraphics[width=0.9\linewidth]{figs/att-example.pdf}
\vspace{-0.4cm}
      \caption{Attention mask for BB vs. \system. BB's attention is comparable to \system in trained environemnt (orange region) while failing to attend well in unseen places (light blue region shown cases for both VO and RF).}
     \label{fig:attexample}
\vspace{-0.4cm}
\end{figure}

 
%\system uses a cross-attention (or inter-modality attention) module to complementarily fuse the feature vectors output
%by the RF and VO CNN extractors (see Fig~\ref{}). Below, we discuss the process of attention calibration and the significance
%of it in the fusion process.
%\subsubsection{Attention Weights:}
%The cross-attention calibrates the individual weights (i.e., importance) of the RF and the VO
%feature vectors based on their respective uncertainties derived from the CNN extractor. Higher the uncertainty, lower
%the individual weight. Intuitively, this would mean the model would 
%rely more on the RF location estimates when VO encounters unfavourable environments (e.g., dim-light), 
%and similarly, reliance on VO location estimates would be higher than RF estimates in the presence of NLoS anchors. 
%
%\subsubsection{Masking attention weights:}
%To ensure that the two (heterogeneous) weighted feature vectors of RF and VO are compatible for fusion, it is important to
%mask the attended weights. We follow the methodology in~\cite{} to derive the cross-attention masks. Accordingly, we use a 
%sigmoid function to normalize the attended weights of the two feature vectors. The derived attention masks are used to
%multiply element-wise to each feature before concatinating the two attended features.
%
%
%\subsubsection{LSTM - Learning from the fused features:}
%The output from the cross-attention is a single dimension flattened array, which is  
%forwarded into an LSTM - a 2 layer RNN (with 64 hidden units per layer) to model the temporal 
%dependency of the fused features. 
%The output of the LSTM is next fed into 
%2 Fully Connected (FC) layers that finally outputs the predicted absolute location.
%The LSTM due to its ability to train on its own outputs (i.e., prior absolute
%location estimtes), can effectively produce absolute location estimates based on the
%relative location estimates from VO alone, when RF features have large uncertainties.

\subsubsection{Effectiveness of Cross-Attention:}
%role in sensor works because we observe data is complementary. Recall the trajectory we discussed earlier (\S\ref{MOTIV}, Fig.~\ref{})
Fig. \ref{fig:attexample} shows \system's attended weights for RF and VO feature vectors. As the device suffers dim-light conditions, \system
increases RF feature attention from .6 to 1, while decreasing that of the VO's features from .9 to .5, 
and in NLoS, RF features are weighted low (decreased from 1 to 0.1), while VO's weights increase from 0.5 to 0.85.
Given the independent and complementary nature of the RF and VO sensors as well as their environmental artifacts, 
it is clear that \system's cross-attention plays a valuable role in effective sensor fusion.

\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/bb-system.png}
      \vspace{-0.8cm}
      \caption{Blackbox Fusion.}
     \label{fig:bbdesign}
\vspace{-0.4cm}
\end{figure}

\subsection{\system vs. Pure ML-driven Fusion} 
\label{sec:bbdesign}
At this point, it is natural to wonder -  {\emph{"How and why is \system better than
prior machine learning based fusion solutions?"}} 
%-- And, answer we shall! 
Prior works (milliEgo~\cite{lu2020milliego} for mmWave+IMU, DeepTIO~\cite{saputra2020deeptio} for thermal+IMU, VINET~\cite{clark2017vinet} for camera+IMU, etc.) have employed 
raw sensor data to directly train a (BlackBox -- BB) ML model, compared to \system's hybrid approach, where ML is largely leveraged for fusion alone. 
%algorithm + machine learning strategy. 
Hence, prior proposed models tend to be more complex (e.g., additional attention layers), requiring
higher computational resources (e.g., more convolution and RNN layers). Further still, having to 
extract the challenging problem structure inherent to {\em absolute localization}, they are 
unable to generalize and deliver robust performance in unseen environments (see \S\ref{EVAL}).  %And still, could potentially succumb to the lack of diversity in the training
%dataset, resulting in underperformance in unseen environments (see \S\ref{EVAL}). 
For an objective comparison, we also implement a pure ML-driven counterpart solution to \system (called BlackBox, BB), 
by instrumenting the network architecture similar to those used in~\cite{lu2020milliego} for our 
UWB and stereo-camera inputs, as shown in Fig.~\ref{fig:bbdesign}. The key differences in 
BB are that, it has an extensive feature extraction network for each of the UWB and camera 
sensor streams, and consequently also employs a self-attention module. The role of self-attention 
is to enable a form of filtering of the weak input features, while emphasizing those that contribute 
to an accurate output prediction. The operation is similar to cross-attention, but instead attending 
on the sensor's own features.  The self-attention masks are given by,
\begin{equation}
    A_{v} = Sigmoid((W'_v F_v)^T W''_v F_v), A_{r} = Sigmoid((W'_r F_r)^T W''_r F_r)
\end{equation}
and the self-attended features as,
\begin{equation}
    A_v' = A_{v} \odot F_v, A_r' = A_{r} \odot F_r
\end{equation}
After the features are self-attended, it follows a cross-attention and fusion pipeline similar to that in \system.
 
%the entire model pipeline proposed in~\cite{}(see Fig.~\ref{}) for fusing our UWB and ORB-SLAM3 data. While the actual performance of the BB model
%on our dataset is deferred to \S\ref{EVAL}, we take this opportunity to show the difference in the complexity of the BB (and other similar) 
%model to \system. 

While \system's detailed performance comparison with BB is deferred to \S\ref{EVAL}, we highlight two of its key advantages:
i) much of its feature extraction burden is driven by efficient algorithms, allowing its ML-component 
to focus solely on fusion, enabling it to generalize and accurately track absolute 
location (and hence across multiple agents) even in unseen environments (see Fig.~\ref{fig:attexample}), 
and ii) lack of a complex feature extraction network reduces its model complexity 
significantly, making it light-weight and deployable on resource-constrained platforms, 
while incurring significantly less time for inference/prediction than is needed for real-time 
operation. In our testbed (described in \S\ref{IMPL}), we show that \system has only 1.2 M 
parameters while BB requires 70 M, when translated into raw data (after model compression), 
\system's size is 62$\times$ smaller than BB, directly leading to a 5 fold decrease in inference 
latency (see \S\ref{sec:syseff}). 


%In this section, we present a blackbox approach, a general learning framework for multi-modal fusion followed by recent literature~\cite{} and contrast it with \system. 

%\subsubsection{Feature extraction} Most of the state-of-the-art learning-driven methods fuse the multi-modal information by directly feeding the raw input data from each sensor to a deep network and extract the features through learning. Recent solutions that follow this approach include milliEgo~\cite{} to combine mmWave and IMU, DeepTIO~\cite{} to thermal and IMU, VINET~\cite{} to combine visual and IMU data. We adopt a similar method to fuse RF and Visual data.
%
%Figure \ref{fig:bbdesign} shows the end-to-end pure learning-based approach for fusion. For RF, input the ranges ($R_i$) as well as the link quality ($L_i$) metrics as described in \S\ref{} to an RF sub-network for feature extraction. We use two ConV1D layers to extract the latent correlations across the features followed by the three Dense layers, each block including standard Batchnorm and Dropout blocks to improve generalization. Similarly for VO, the stereo frames at two consecutive time intervals are passed to a VO sub-network to extract the features that implicitly compute the correspondences between the two images. In particular, we adopt a FlowNet~\cite{} module to estimate the optical flow between the the images for feature correspondence. The FlowNet module consists of 9 convolutional layers followed by a LeakyReLu activation function. The features extracted from this module are compact in size reducing the dimensions and capturing the temporal dependencies through time-distributed layers. 
%
%\subsubsection{Attending the features and location estimate} Once the features are extracted from each sensor, we follow a two-stage attention mechanism proposed in \S\ref{}. This two-stage attention is proven to perform better than a mixed single-stage attention. The two-stage attention involves i) self attention, ii) cross-modal attention. The self attention is similar to self-filtering process to remove weak features before combining with other sensor features. Given, $z_v$ as the visual, $z_r$ as the RF features extracted the individual sub-networks, we learn the self attention mask/probability map based through learnable parameters as follows:
%
%\begin{equation}
%    A_{vm} = \sigma[(W^Q_v z_v)^T W^\psi_v z_v], A_{rm} = \sigma[(W^Q_r z_r)^T W^\psi_r z_r]
%\end{equation}
%
%where, the $W$ are the learnable parameters that transform the extracted features into embedding spaces $Q$ and $\psi$ respectively. The original features can be attended using the obtained masks as below:
%
%\begin{equation}
%    A_v = A_{vm} \oplus z_v, A_r = A_{rm} \oplus z_r
%\end{equation}
%
%After the features are self-attended, we follow a cross-attention and fusion pipeline similar to \system (presented in \S\ref{}).
%
%\subsubsection{\system versus Blacbox} \system differs from the above blackbox design in three important directions--- i) algorithm-assisted generalization, ii) much of the feature extraction burden in the blackbox fusion model is driven by the algorithm, so the fusion model can optimize more on the fusion rather than extracting features, iii) \system does not require a complex network like blackbox solution to extract features and therefore can reduce the model complexity significantly. As a result, \system fusion network is lightweight and takes significantly less time for inference/predicting compared to blacbox methods.




% cross-modal attention background and how it is applied in \system to predict the absolute location estimate
%In this section we describe our hybrid fusion approach to estimate the absolute location by leveraging RF and VO algorithmic tracking solutions presented in \S\ref{}. As discussed in \S\ref{}, \system  adopts a learning-based approach to fuse the RF and VO tracking. 
%
%\subsubsection{Challenges of fusing active passive tracking} \system's goal is to fuse the multi-modal RF and VO tracking to obtain accurate and robust absolute tracking. There are two key challenges associated to achieve this goal. First, \system should efficiently adapt the fusion to weight sensor appropriately when the the sensors face favourable and unfavourable environmental conditions. The complementary nature of RF and VO should drive the fusion, for example, by weighting RF more than VO under dim-lit and feature less environmental conditions and similarly, weight VO more when there are a lot of NLOS anchors. Second, \system should estimate an absolute location from the active RF that gives absolute location, while the VO tracking is relative. Directly combining the absolute and relative tracking from RF and VO can lead to inefficient fusion because the relative tracking does not have the ability to recover quickly when faced with intermittent unfavourable conditions. In the following, \system addresses these two challenges. 
%
%\subsubsection{Adaptive fusion using cross-model attention} To exploit the complementary nature of the sensors, we adopt \textit{Attention} mechanism, a commonly used technique for weighting the features to adapt the multi-modal-driven learning solutions. There are a variety of attention models in the learning literature, fore example, self attention~\cite{} and cross-model attention~\cite{} etc. The self attention weights the features of an individual sensor to self adapt and eliminate the influence of outliers. This is analogous to traditional self-filtering methods such as KF and PF described in \S\ref{}. The cross-attention model, however, weights each sensor with respect to one another. \system directly adopts the cross attention model without using self attention because the features engineering described in \S\ref{} has already in a way captures this through the correlations of features with the tracking error. Next, we provide the details of cross-model  attention.
%
%The cross-model attention technique has been heavily used in machine learning multi-modal tasks~\cite{}. The cross attention is used to extract the inter-sensor correlations and re-weight the sensors with respect to each other. Essentially, two probability maps or masks are learned using the RF and VO features before fusing the features directly; one mask for RF and another for VO. Given the features of RF and VO as $A_r$ and $A_v$, the cross attention masks can be computed as below:
%
%\begin{equation}
%    A_{rv} = \sigma[(W^Q_{rv}z_v)^T W^\psi_{rv}z_v], 
%    A_{vr} = \sigma[(W^Q_{vr}z_r)^T W^\psi_{vr}z_r]
%\end{equation}
% 
%where, W are the learnable weight parameters, and $\sigma$ is nonlinear activation function. After the masks are learned, each mask is applied to respective sensor and then the masked features are merged together to fuse both the sensors and estimate the location. The fused features can be formally represented as:
%
%\begin{equation}
%    A = [A_{rv} \oplus z_v; A_{vr} \oplus z_r]
%\end{equation}

%\subsubsection{Absolute location estimate} As discussed in \S\ref{}, the key challenge with the relative tracking its inability to recover quickly when it loses tracking under unfavourable conditions, because of its decision based on previous positions. Isolating this limitation relative tracking and predicting the absolute location can make the tracking more resilient and quickly recover even if the VO-tracking faces unfavourable conditions frequently. \system achieves this by leveraging the estimates in translational ($r$) and rotational displacements ($\theta$) from the VO-tracking described in \S\ref{} to guide the fusion, instead of final relative position estimates.
%
%\smallskip
%\noindent \textbf{\system's end-to-end fusion and location estimation:} Figure \ref{fig:rovarfusion} shows the \system's end-to-end hybrid fusion. On the VO path, the stereo frames at two consecutive time intervals ($V_t, V_{t-1}$) are passed to the SLAM algorithm to estimate the polar coordinates ($r, \theta$) which are passed along with the extracted certainty metrics presented in \S\ref{} such as matching keypoints and additional metrics to the fusion model. On the RF path, the anchor selection model filters out anchors with poor ranging using the link quality ($L_i$) and ranges ($R_i$). The filtered ranges and their fixed locations are fed to the multi-lateration get the absolute location estimates (after filtering the anchors as described in \S\ref{}). The location estimates given by the algorithm are passed along with the ranges and received signal power estimates to fusion model. See Figure \ref{}. These features first passed through two convolutional layers to extract the correlations among the individual features and certainty metrics before applying the attention masks. The features are then merged together and passed though an RNN layer to capture the temporal correlations and estimate the absolute location. 
%
%\subsection{Contrasting with Pure ML-driven Fusion} \label{label:bbdesign}
% talk about the pure data-driven (black-box) approach to contrast the difference in \system's approach




==> discussion.tex <==
% discussion
\noindent\textbf{(1) Reducing RF Deployment Overhead:} 
%While \system's UWB component leverages 3 anchors for absolute device localization, 
The infrastructure assistance (anchors) for RF localization is becoming common-place. 
WiFi APs (e.g. Google Nest products) already support ranging mechanisms (FTM~\cite{ibrahim2018verification}) similar to UWB, albeit with a maximum of 160 MHz bandwidth.
While \system is equally applicable to leveraging WiFi-based absolute localization, we believe UWB is likely to become part of our APs as well in future (already available in Apple and Samsung smartphones~\cite{appleu1chip, sammobileuwbchip}). Further, one can also reduce the dependence on 3 anchors (either for UWB or WiFi) by leveraging just a single multi-radio (antenna) anchor that provides both angle (AoA) and range information (e.g. NXP UWB chips~\cite{nxpsinglechip}) to directly localize a device. This single reference anchor could be built as part of an access point, application  (e.g. game) controller, just a smart device in the environment to track multiple agents simultaneously.     
%our future deployments will readily support 
%\% Single Multi-radio anchor can reduce the dependence on  multiple anchors to just a single anchor.
 
\noindent\textbf{(2) From Position to Pose:}
While ORB-SLAM3 can already deliver relative pose estimation, \system's UWB-localization currently supports only position.
Employing a multi-radio (two synced radios)  design on the device (e.g. one on either side of a headset), can allow the device on the agent to also determine its orientation from RF AoAs. Similar to fusion of position from RF and visual sensors, one can also fuse orientations from the two sensors, to yield absolute pose of the agent.  This is part of our next step. 

\noindent\textbf{(3) Addition of Inertial Sensors:}
\system's objective has been to bring dual-layer diversity to sensor fusion and hence focused on two key sensors, cameras and RF (UWB) for the start.  
One can extend \system to a third popular sensor, namely inertial (IMU) sensors, for which there exists a rich body of sensor fusion work~\cite{lu2020milliego, clark2017vinet, venkatnarayan2019enhancing}.
\system would employ a third algorithmic branch for IMU-based feature extraction (position and other relevant features). The key adaptation needed to \system's framework would be to consider cross-sensor attention between every pair of the three sensors (cameras, UWB and IMU), before fusing them to bring further robustness and accuracy to multi-agent tracking. 


==> evaluation.tex <==
% evaluation

\begin{figure*}[t]
\centering
    \subfloat[Well-lit, Walking Trajectory]{%
      \includegraphics[width=0.245\linewidth]{figs/bestcase-shape1-trajectory.png} 
     }
    \subfloat[Well-lit, Walking Trajectory Error]{%
      \includegraphics[width=0.245\linewidth]{figs/bestcase-shape1-error.png} 
     }
    \subfloat[Well-lit, Walking Curve Trajectory]{
      \includegraphics[width=0.245\linewidth]{figs/bestcase-shape3-trajectory.png}  
     }
    \subfloat[Well-lit, Walking Curve Error]{
      \includegraphics[width=0.245\linewidth]{figs/bestcase-shape3-error.png}  
     }
    
    \subfloat[Dim-lit, Walking Curve Trajectory]{
      \includegraphics[width=0.245\linewidth]{figs/shape2-dimlit-trajectory.png}  
     }
    \subfloat[Dim-lit, Walking Curve Error]{
      \includegraphics[width=0.245\linewidth]{figs/shape2-dimlit-error.png}  
     }
    
    \subfloat[Well-lit, Running Trajectory]{%
      \includegraphics[width=0.245\linewidth]{figs/shape1-running-trajectory.png} 
     }
    \subfloat[Well-lit, Running Trajectory Error]{%
      \includegraphics[width=0.245\linewidth]{figs/shape1-running-error.png} 
     }
    \subfloat[Well-lit, Running Trajectory]{
      \includegraphics[width=0.245\linewidth]{figs/shape3-running-trajectory.png}  
     }
    \subfloat[Well-lit, Running Trajectory Error]{
      \includegraphics[width=0.245\linewidth]{figs/shape3-running-error.png}  
     }
      \caption{Comparing \system's tracking performance with exiting methods. Top rows a-c: walking, Bottom rows d-f: running.}
     \label{fig:comprehensive}
\end{figure*}

We experimentally evaluate \system under a diverse set of environmental conditions and performance metrics, with a goal towards answering the following questions:

\begin{itemize}[leftmargin=5mm]
    \item How does \system perform compared to the state-of-the-art approaches in terms of tracking accuracy? 
    \item Does \system generalize to new environmental conditions? 
    \item How does \system perform under multi-user scenarios in terms of relative tracking error?
    \item How robust \system is under highly unfavourable conditions such as dim-lighting, random motions, and NLOS scenarios? How quickly \system can recover compared to prior work?
    \item What is the end-to-end latency and system efficiency of \system?
\end{itemize}

\subsection{Experimental Methodology} \label{label:expmethodology}
\noindent \textbf{Evaluation metrics:} We evaluate the \system's tracking performance using Absolute Trajectory Error (ATE), a commonly adopted metric to compare the tracking error relative to ground truth. ATE is computed as the euclidean distance of the estimated and ground truth trajectories after associating the estimated trajectory with ground truth and provides a holistic long term tracking performance. We report ATE performance in terms mean, standard deviation (std), max error. We also  evaluate the relative error among the users' trajectories by computing the difference between the ground truth distance and the users' distance (see \ref{label:multiusr-eval}).

\smallskip
\noindent \textbf{Baselines:} We compare \system with a suite of methods that include both conventional algorithmic as well as learning methods:

\begin{itemize}[leftmargin=5mm]
    \item \textbf{RF:} We report the localization results of RF-based approach alone. This is an algorithmic solution as described in \S\ref{}.
    \item \textbf{VO:} We also compare the VO solution alone using ORBSLAM3 method described in \S\ref{}.
    \item \textbf{EKF:} This is a conventional method of multi-modal data with relaxed Gaussian assumptions of Kalman filter approach~\cite{}. This class of solutions mainly work well for linear system models and suffer from the linearization of nonlinear models. There are other solutions such as UKF~\cite{} and Particle filter~\cite{}, but are computationally heavy and require significant convergence time. Therefore, we consider EKF approach taken by recent works such as~\cite{}, in the  context of combining WiFi+IMU~\cite{} and IMU+UWB~\cite{}.
    \item \textbf{BB}: A blackbox-driven multi-modal fusion method that is described in \S\ref{label:bbdesign}. This method takes the raw data from individual sensors and extracts features through neural layers. The final pose is obtained by attending and fusing the learned features. A recent method called milliEgo~\cite{} follows this design in a different context of combining IMU and mmWave data.
    \item \textbf{VINET:} A state-of-the-art visual-inertial tracking solution based on blackbox learning approach~\cite{}. 
\end{itemize}

\subsection{\system Vs. Existing Methods}
We start comparing \system's performance with the existing methods under best case environmental conditions for both RF and VO. Figure \ref{fig:comprehensive} shows a comprehensive comparison of \system's tracking performance with the suite of algorithms described in \S\ref{label:expmethodolog}. The results spread across three different shapes of trajectories and two types motion (walking and running).

\smallskip
\noindent \textbf{Effect of trajectory shapes and environments:} Figure \ref{fig:comprehensive}a-c shows the impact of different shapes on tracking performance while walking along these trajectories. We deliberately consider different shapes as users in practice follow random paths, especially in open environments. Figure shows that, \system achieves the lowest error out all the existing methods with an average ATE of XXm. More importantly, the maximum of ATE of \system is well under 60cm across all three trajectories. The state-of-the-art fusion solutions such as BB and EKF does perform better than the individual algorithmic solutions, however, their error is still more than \system. 

The Figure also shows that there is a slight change the tracking performance across the trajectories. For example, even though the rectangle and S-shaped curve trajectories are in the same indoor open space, the rectangle trajectory has slightly more error. This is because of the small drift accumulated at the sharp turns (we will show impact of such abrupt turns in \S\ref{label:extremeconditions}). Similarly, the error in case of the semi-construction space trajectory is more (by XXm) than the indoor open space area. There are two reasons behind--- i) the RF anchors are placed in a wider space (40mx30m area) in the latter case while the former case is smaller space (20mx20m), and therefore there is more ranging error because of the coverage and occasional NLOS conditions due to pillars in the construction area, ii) the VO tracking is weaker here because of the glass wall with outdoor environment having less features than the indoor spaces.   

\smallskip
\noindent \textbf{Effect of motion:} We study the \system's performance under different users' motions--- walking and running. As users follow different speeds while moving around, studying the impact of motion is important. Figure \ref{fig:comprehensive}d-e shows the impact of running on the same trajectories mentioned above. Again, \system is the best performing solution among all with an average ATE of XXm and a maximum ATE of YYm. The average ATE under running scenario is slightly more than the walking scenario. We find that this increase is mostly due to VO-tracking being sensitive to motion. In our experiments, we find that the matching keypoints are significantly less (by XX\%) in the running case compared to walking case. The RF tracking is less affected compared to VO because there is no change in anchors' LOS conditions.

\begin{figure}[t]
\centering
        \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/att-eval-trajectory.png} 
     }

    \subfloat[]{%
      \includegraphics[width=\linewidth]{figs/att-eval-error.png} 
     }
      \caption{Dissecting the attention mask for RF and VO (e.g., NLOS for RF and Dim-lit for VO).}
     \label{fig:attention}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[Unseen Place1 Trajectory]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-place1-trajectory.png} 
     }
        \subfloat[Unseen Place1 Error]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-place1-error.png}  
     }
     
    \subfloat[Unseen Place2 Trajectory]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-place2-trajectory.png} 
     }
        \subfloat[Unseen Place2 Error]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-place2-error.png}  
     }
    \label{fig:unseen}
\end{figure}

% \begin{figure}[t]
% \centering
%     \subfloat[Unseen Place3 walking]{%
%       \includegraphics[width=0.8\linewidth]{figs/home-well-lit-walking.pdf} 
%      }
     
%     \subfloat[Unseen Place3 Running]{%
%       \includegraphics[width=0.8\linewidth]{figs/home-well-lit-running.pdf} 
%      }
%       \caption{Home environment.}
%      \label{fig:place-home}
% \end{figure}

% \subsection{Robustness to Extreme Conditions} \label{label:extremeconditions}
Next, we study the resiliency of \system compared to other solutions when the sensors face unfavourable conditions for a short period of times. We deconstruct the effect of VO and RF by creating scenarios such that one faces regular environmental conditions while the other faces quick extreme conditions and evaluate how quickly \system is able to recover. We experiment with two types of experiments--- i) we create a scenario such that each sensor continues to track (albeit with drifted and larger errors) for the entire duration of the trajectory (e.g., acceptable dim lighting for VO and NLOS anchors for RF), ii) we create a scenario where one sensor complete loses track and hence \system relies completely on one sensor (e.g., total dark rooms for VO and out of coverage for RF).

In summary, \system substantially outperforms all the competing methods with an average ATE of XXm and  a maximum ATE under well under 1m.

\subsection{Generalizability in Unseen Environments}
As described in \S\ref{label:bbdesign}, a classical limitation of learning through deep networks is hard to achieve generalizability. \system avoids this problem of generalization through algorithmic assistance. We show this by evaluating \system in two unseen environments and compare with the pure learning approaches along with the conventional methods. These two unseen places have different floor plan with different wall color and follow across corridors in an office environment, where as the training consists of large open spaces, semi-construction environment and small office room.

Figure \ref{fig:unseen} shows the tracking performance across two different unseen trajectories. Despite the unseen environment, Figure shows that \system's trajectory is consistent with the ground truth trajectory and its performance similar to seen environments with a mean ATE of XXm and max ATE of YYm being consistent with the ATE from the seen environments. The main reason behind this impressive generalization is that \system's fusion is guided by algorithm intelligence through confidence features from tracking algorithms. However, BB fails to be consistent with the ground truth trajectory and results in large ATE across the entire trajectories with a mean ATE of XXm and max ATE of YYm. The primary reason behind this failure is that BB's fusion is guided by the learned high level features extracted through convolutions that are hard to capture the unseen features. Whereas in case of \system, the environmental conditions are abstracted through algorithm, and hence the generalization. 

\subsection{Tracking Across Multiple Users} \label{label:multiusr-eval}

Most of the tracking-based applications (e.g., first responders~\cite{}, medical training~\cite{}, Education~\cite{}, etc) involve multiple users interacting with each other. In order to have a seamless experience, these applications require accurate tracking of users relative to each other along with self-tracking. We study \system's tracking performance as we more users into the system and compare the with the state-of-the-art methods. To this end, we show two application use cases: one where 'relative' tracking sensitive and another 'additive' tracking sensitive application by reporting two error metrics--- i) relative error, ii) additive error. The relative error the difference in the estimated distance and the ground truth distance between two users. The additive error is a combined error of two users tracking relative to their ground truth. For more than two users, we compute the average of all users' tracking relative to all the other users.

Figure \ref{fig:multi-user} shows the tracking performance of \system for 2 and 3 users and compared with BB. In both relative and additive case, \system outperforms the individual algorithms as well as BB. The benefits are as we more users and significantly better under additive scenario. In case of relative, we observe that RF-tracking is more consistent compared to VO because the latter is more sensitive where start and end as its drift accumulates towards the end of the trajectory.

\begin{figure}[t]
\centering
    \subfloat[2 Users (Seen)]{%
      \includegraphics[width=0.5\linewidth]{figs/relative-error-2-users.png} 
     }
    \subfloat[3 Users (Seen)]{%
      \includegraphics[width=0.5\linewidth]{figs/relative-error-3-users.png}  
     }
     
    \subfloat[2 Users (Seen)]{%
      \includegraphics[width=0.5\linewidth]{figs/additive-error-2-users.png} 
     }
    \subfloat[3 Users (Seen)]{%
      \includegraphics[width=0.5\linewidth]{figs/additive-error-3-users.png}  
     }
    
    \subfloat[2 Users (Unseen)]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-relative-error-2users.png} 
     }
    \subfloat[3 Users (Unseen)]{%
      \includegraphics[width=0.5\linewidth]{figs/unseen-relative-error-3users.png}  
     }
      \caption{Relative and additive error multiple users.}
     \label{fig:multi-user}
\end{figure}

\subsection{Real-time Operation}

We evaluate the real-time capability of \system and show that it outperforms the existing methods in terms of its system efficiency. We report latency results on two platforms: 1) Desktop-grade machine with a configuration described in \S\ref{label:prototype}, 2) Jetson TX2, a mobile-grade device. Table \ref{tab:syseff} compares the latency of \system with the algorithmic RF and VO solutions, and the blackbox model. 

The table shows that \system fusion is highly light-weight and takes under 6ms even on the mobile platform. However, as an end-to-end system \system constitutes the algorithmic latency as well of our hybrid algorithm-assisted learning approach. The RF localization is also light-weight and takes under 3ms, whereas the VO (ORBSLAM3) is highly compute expensive. Together, \system's end-to-end latency comes down to XXms on Desktop and YYms on the mobile platform, translating to XX Fps and YY Fps respectively. However, there is an extensive prior work in reducing the latency of VO solutions~\cite{} that significantly bring down the VO latency and therefore \system can be easily deployed in practice. Nevertheless, the end-to-end \system system is significantly faster than state-of-the-art blackbox solution by almost 3$\times$ on the Desktop. Moreover, the blackbox model cannot even be run on the mobile platform because of its high model complexity. As shown in the table, the model size of blackbox solution is 68$\times$ more compared to \system. This is because \system works on the algorithm-given features, whereas the blackbox solution needs additional neural network layers to extract features before the fusion.

\begin{table}[t]
  \centering
     \caption{System efficiency and run-time analysis of ROVAR comparing with other methods.}
  \scalebox{0.89}{
  \begin{tabular}{|l|c|c|c|c|}
  %\hline 
  \hline
      \textbf{ } & \textbf{RF} & \textbf{VO} & \textbf{BB-Fusion} & \textbf{\system-Fusion} \\
    \hline
    %\hline
    Desktop-latency (ms)  & 1.80           & 43.67     & 126.91    & 2.61  \\ \hline
    Jetson TX2-latency (ms)  & 3.20          & 61.67  & - & 5.34\\ \hline
    Model size (MB) & -  &  - & 341.15 & 5.05 \\ \hline %\hline
  \end{tabular}
    }
  \label{tab:syseff}
\end{table}


==> evaluation1.tex <==
\begin{figure}
\includegraphics[width=1\linewidth]{figs/legend.png}
  \vspace{-0.4cm}
\centering
    \subfloat[Walking, Office - 1]{%
      \includegraphics[width=0.5\linewidth]{figs/evaluations/seen/well-lit-walking-curve-trajectory} 
     }
    \subfloat[Running, Office - 2]{
      \includegraphics[width=0.5\linewidth]{figs/evaluations/seen/dim-lit-running-rectangle-trajectory}  
     }
%  \vspace{-0.1cm}
  \caption{\system Vs. Baselines trajectory in trained environment -- Favorable condition (left), Practical condition (right).}
\label{fig:trajectory-seen}
\vspace{-0.9cm}
\end{figure}
\begin{figure}
%\includegraphics[width=1\linewidth]{figs/legend.png}
\centering
    \subfloat[Walking, Home]{%
      \includegraphics[width=0.5\linewidth]{figs/evaluations/unseen/home-dim-lit-walking-trajectory} 
     }
    \subfloat[Running, Office - 3]{
      \includegraphics[width=0.5\linewidth]{figs/evaluations/unseen/unseen-place2-dim-lit-walking-trajectory}  
     }
  \vspace{-0.3cm}
  \caption{\system Vs. Baselines trajectory in Unseen environment in Practical conditions.}
\label{fig:trajectory-unseen}
\vspace{-0.4cm}
\end{figure}

\begin{figure*}
\includegraphics[width=0.8\linewidth]{figs/legend.png}
\centering
    \subfloat[Walking, Office - 1]{
      \includegraphics[width=0.245\linewidth]{figs/evaluations/seen/well-lit-walking-curve-cdf}  
     }
    \subfloat[Running, Office - 2]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/seen/well-lit-running-rectangle-cdf} 
     }
    \subfloat[Walking, Office - 1]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/seen/dim-lit-running-rectangle-cdf} 
     }
    \subfloat[Running, Office - 2]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/seen/dim-lit-walking-curve-cdf} 
     }
     \vspace{-0.2cm}
     \caption{CDFs \system Vs. Baselines in Trained environment. Favorable conditions (a,b), Practical conditions (c,d).}
     \label{fig:comprehensive-seen}
     \vspace{-0.3cm}
\end{figure*}
\begin{figure*}[t]
%\includegraphics[width=0.8\linewidth]{figs/legend.png}
\centering
    \subfloat[Walking, Home]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/unseen/home-well-lit-walking-cdf} 
     }
    \subfloat[Walking, Office - 3]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/unseen/unseen-place1-well-lit-walking-cdf} 
     }
    \subfloat[Walking, Home]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/unseen/home-dim-lit-walking-cdf} 
     }
    \subfloat[Walking, Office - 3]{%
      \includegraphics[width=0.245\linewidth]{figs/evaluations/unseen/unseen-place1-dim-lit-walking-cdf} 
     }
      \vspace{-0.1in}
      \caption{\system Vs. Baselines in Unseen environments. Favorable conditions(a,b), Practical conditions(c,d).}
     \label{fig:comprehensive-unseen}
%      \vspace{-0.2in}
\end{figure*}
\begin{figure*}
\vspace{-0.2in}
%\includegraphics[width=0.8\linewidth]{figs/legend.png}
\centering
%    \subfloat[Relative-distance, Office, Unseen, 3 Unsers]{%
%      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/unseen-relative-error-3-users-place1.pdf} 
%     }
%    \subfloat[Relative-angle, Office, Unseen, 3 Users]{%
%      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/relative-angle-error-3-users-place1.pdf} 
%     }
    \subfloat[Trained, Office, 2 Users]{%
      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/seen-relative-translation-error-2-users.pdf} 
     }
    \subfloat[Unseen (Home), 3 Users]{
      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/unseen-relative-error-3-users-place3.pdf}  
     }
    \subfloat[Trained, Office, 2 Users]{%
      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/seen-relative-angle-error-2-users.pdf} 
     }
    \subfloat[Unseen (Home), 3 Users]{%
      \includegraphics[width=0.25\linewidth]{figs/evaluations/multi-user/relative-angle-error-3-users-place3.pdf} 
     }
     \vspace{-0.1in}
     \caption{\system performance for multi-users. Relative distance error (a,b) and Relative angular error (c,d)}
     \label{fig:multi-user}
\end{figure*}

%We evaluate performance of \system under diverse environmental conditions, with a goal of answering the following questions:\\
%- How does \system perform compared to the state-of-the-art approaches in terms of tracking accuracy? \\
%- Does \system generalize to new environmental conditions?\\ 
%- How does \system perform under multi-user scenarios in terms of relative tracking error?\\
%- How robust \system is under highly unfavourable conditions such as dim-lighting, random motions, 
%and NLOS scenarios? How quickly can \system recover compared to prior work?\\
%- What is \system's end-to-end latency and its system efficiency?\\

%\begin{itemize}[leftmargin=5mm]
%    \item How does \system perform compared to the state-of-the-art approaches in terms of tracking accuracy? 
%    \item Does \system generalize to new environmental conditions? 
%    \item How does \system perform under multi-user scenarios in terms of relative tracking error?
%    \item How robust \system is under highly unfavourable conditions such as dim-lighting, random motions, and NLOS scenarios? How quickly \system can recover compared to prior work?
%    \item What is the end-to-end latency and system efficiency of \system?
%\end{itemize}

\subsection{Experimental Methodology} 
\label{label:expmethodology}
We extensively evaluate \system for the case of single and (collaborative) multi-user tracking scenarios, under diverse (trained and unseen) environmental 
conditions, for two different human-motions (running and walking), to demonstrate \system's robustness and efficacy 
vis-a-vis other state-of-the-art solutions (described below). Our evaluation testbeds are located in home and office 
environments with each testbed having varying texture (rich and poor) and lighting conditions (good and dim). 
In each testbed, we ensure there is a healthy mix of LoS and NLoS UWB anchors, to mimic real-world deployments. \\
%Finally, we evaluate \system for different types of human-motions (e.g., walking, running etc). \\
\noindent \textbf{Evaluation metrics:} We use the Absolute Trajectory Error (ATE)~\cite{sturm2012benchmark} - 
a commonly used metric for VO evaluations to quantify the performance of \system. ATE is calculated as the  
Euclidean distance between corresponding points on the estimated and the GT 
trajectories that are time-aligned. \\ %We report mean-ATE values.\\
%We report ATE performance in terms mean, 
%standard deviation (std), max error. We also  evaluate the relative error among the users' trajectories by computing 
%the difference between the ground truth distance and the users' distance (see \ref{label:multiusr-eval}).
%\smallskip
\noindent \textbf{Baselines:} We compare \system with the following suite of baseline solutions that include both conventional algorithms
and ML based solutions.
%\begin{itemize}[leftmargin=5mm]
\textbf{RF}  is the multilateration-based RF localization solution described in \S\ref{sec:background}.
\textbf{VO} is the ORB-SLAM3 VO tracking solution described in \S\ref{sec:background}.
\textbf{EKF} is the Extended Kalman-filter (EKF), an algorithmic solution commonly used for multi-sensor data fusion. We found
other flavors of Kalman-filter like UKF~\cite{wan2000unscented} and Bayesian filters (e.g., particle filter) to have similar
performance. In the interest of space, we show results only for EKF.
%Kalman filter approach~\cite{}. This class of solutions mainly work well for linear system models 
%and suffer from the linearization of nonlinear models. There are other solutions such as UKF~\cite{} 
%and Particle filter~\cite{}, but are computationally heavy and require significant convergence time. 
%Therefore, we consider EKF approach taken by recent works such as~\cite{}, in the  context of combining WiFi+IMU~\cite{} and IMU+UWB~\cite{}.
\textbf{BB} is the (Black Box) ML based fusion approach described in \S\ref{sec:bbdesign}. 
%This method takes the raw data from individual sensors and extracts features through neural layers. 
%The final pose is obtained by attending and fusing the learned features. 
%A recent method called milliEgo~\cite{} follows this design in a different context of combining IMU and mmWave data.
\textbf{VINET} is a state-of-the-art ML based visual-inertial tracking solution~\cite{clark2017vinet}. 
%\end{itemize}

%\begin{table}[t]
%\centering
%\caption{Aggregate results.}
%\label{label:skype-devices}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%    \multicolumn{1}{|c|}{Users} & Metric   & \multicolumn{1}{c|} {RF} & {VO} & {EKF} & {BB} & {VINET} & \system \\ \hline
%\multirow{3}{*}{1}   & Mean  & 0.42  & 0.38 & 0.36  & 0.48 & 0.59 & 0.17  \\ \cline{2-8} 
%                     & Std   & 0.24  & 0.36 & 0.29  & 0.45 & 0.55 & 0.12 \\ \cline{2-8} 
%                     & Max   & 1.32  & 1.82 & 1.28  & 2.67 & 2.87 & 0.89  \\ \hline
%\multirow{3}{*}{2}   & Mean  & 0.48  & 0.56 & 0.51  & 0.58 & 0.64 & 0.20 \\ \cline{2-8} 
%                     & Std   & 0.27  & 0.41 & 0.31  & 0.51 & 0.53 & 0.13     \\ \cline{2-8} 
%                     & Max   & 1.66  & 2.12 & 1.98  & 2.34 & 1.34 & 1.02     \\ \hline
%\multirow{3}{*}{3}   & Mean  & 0.61  & 0.74 & 0.62  & 0.72 & 0.89 & 0.28     \\ \cline{2-8} 
%                     & Std   & 0.41  & 0.58 & 0.43  & 0.63 & 0.73 & 0.18  \\ \cline{2-8} 
%                     & Max   & 2.14  & 2.38 & 2.21  & 2.72 & 2.97 & 1.32 \\ \hline
%\end{tabular}
%\end{table}

\subsection{Performance in Trained Environments}
We begin evaluating (testing) performance %of \system and baseline solutions 
in environments that were used for training the 
ML models. Due to space-constraints we show results from only a subset of the 
trajectories used in our evaluation. 
Interested readers can find the rest of the results in~\cite{tech-report}.
%good for both RF (only LoS anchors) and VO (bright light and abundant features), and gradually start
%start degrading the conditions, with NLoS anchors for RF and moving VO conditions (NLoS anchors and poor features and lighting) 
%and evaluate the ability of \system to adapt to the changing conditions effectively while the 
%baseline solutions suffer.
%conditions for both RF (no NLoS anchors) and VO (good light and abundant image features). Figure ~\ref{fig:comprehensive} 
%shows a comprehensive comparison 
%of \system's tracking performance with the suite of algorithms described in \S\ref{label:expmethodolog}. 
%The results spread across three different shapes of trajectories and two types motion (walking and running).

%\subsubsection{Trained environment:}
%Trained environment includes testbeds which were used to train \system and other machine-learning based baseline solutions.\\
\textbf{Favorable conditions:} 
We first evaluate in environments with rich texture, good lighting (good for visual tracking) and LoS RF anchors (good for RF tracking). 
Fig.~\ref{fig:trajectory-seen} shows the Ground Truth (GT) and the estimated 
trajectories of all the solutions, when a user is walking and running. The 
CDF graphs in Fig.\ref{fig:comprehensive-seen}a-b show the ATE (Absolute Trajectory Error) information for each solution.
While the algorithmic solutions (RF and VO) are agnostic to environmental conditions, the 
trained environments allow us to capture BB and VINET's performance in their most favorable scenarios. 
As expected, BB and ViNET provide a median error of 23cm, 24cm (office-1 and office-2) and 
28cm, 27cm (office-1, and office-2), respectively (walking and running case), and perform better than 
the individual algorithms, RF (median ATE 42cm \& 35cm in office-1 and office-2), VO (median error 32cm \& 29cm), as well as their fused version, 
EKF (median error 41cm in office-1). This is because VO, despite its inherent 
error-correction mechanism, suffers during  trajectory-turns where
the number of ORB feature matches are relatively lower than when walking in straight lines, leading 
to accumulation of error; 
while RF delivers a coarser accuracy compared to visual tracking 
even in the best case. The EKF fusion % aims to minimize individual algorithmic errors, but 
is still vulnerable to the individual sensor errors and artifacts, while ML solution are able 
to mitigate algorithmic uncertainties using data-driven models. 
\system's dual-layer diversity provides a significantly better performance (median error 17cm) 
over both algorithmic and data driven solutions,
resulting in 46\% and 66\% higher median-accuracy even compared to BB and VINET, respectively. 

\textbf{Practical conditions:}
Next, we evaluate \system in the same environments, but by introducing dim lighting conditions 
(in a room that is part of the trajectory - Fig.~\ref{fig:trajectory-seen}), and moving 
a subset of RF anchors into NLoS. Results are shown in Fig.~\ref{fig:comprehensive-seen}c-d.
% shows the GT and estimated 
%trajectories and the ATE CDFs for all the solutions  when user is walking and running.
We see that RF and VO algorithms suffer due to NLoS anchors and dim lighting, respectively, with
VO (median error 40cm) performing worst, especially when user is running (see~\ref{fig:trajectory-seen}b - 
VO deviations are clearly visible). VINET which relies mainly on the VO performance
seem to suffer too due to VO's degradation. BB performs
better (median error 25cm, 28cm) than the algorithmic ones (including EKF - median error 35cm), owing to its model (which leverages RF and visual raw data)
capturing environmental artifacts and their impact on fusion in the trained scenarios.  
%due to their data-driven training and also the evaluation is in the
%same environment as the training. Furthermore, 
Finally, \system which benefits from its RF anchor selection module to increase the accuracy in RF tracking, combined with its dual-diversity fusion,
performs best with median error 17cm, and a gain of 29\% and 64\% in accuracy over BB and VINET respectively. 
%algorithms. Accuracy of \system is 29\% and 64\% higher 
%than BB and VINET, respectively. 

\subsection{Robustness in Unseen Environments}
In order to test \system's ability to generalize to untrained environments, we evaluate its performance
in completely unseen input distributions (new places). % that are unseen, and unused during training. 
We deploy two separate testbeds - one in an
office environment and one in a home environment - for this purpose.
Results for a third testbed can be found in ~\cite{tech-report}.
%and use them to test \system's performance.
%Untrained environment includes testbeds that are unseen by \system and other machine-learning based baseline solutions. The
%goal is to test the generalization of \system. In this segment, we use three new testbeds - two in an office building
%and the third is at a house.

\textbf{Favorable conditions:} 
As before, we begin our experiments with favorable conditions for RF and visual tracking ,i.e., ensure that the 
visual scenery has rich texture, good 
lighting and the RF anchors are all in LoS. 
%Graphs in Fig~\ref{fig:comprehensive-unseen}a-c
%show the trajectories and the ATE CDFs for \system and other baseline algorithms.
Graphs in Fig~\ref{fig:comprehensive-unseen}a-b show that while RF, VO and EKF algorithms' performance
are similar to the trained environments due to their environmental-agnostic nature, 
BB and VINET solutions' performance deteriorates significantly with median ATE for both the 
solutions $>$ 50 cm (>125\% degradation compared to trained environments), with the top 10\% of points having errors $>$1m. 
Clearly, BB and VINET are unable to generalize and perform robustly in untrained environments. % with the amount of data used in their training.
On the other hand, \system 
%\emph{with the same training} 
has a median error of only {$\approx$20cm, 15cm in Home and Office - 4} (similar to its performance in trained environments) and
a maximum error that is $<$ 0.75cm ($\approx$ 230\% increase in median-accuracy). 
{\em \system's strategy of 
leveraging RF and VO algorithms for extracting tracking features, allows its sensor fusion
to perform robustly even in untrained environments with high accuracy.}

\textbf{Practical conditions:}
Untrained environments with practical conditions (for RF and VO) are perhaps the most challenging. 
The trajectories estimated by \system, BB and  EKF are shown in Fig.~\ref{fig:trajectory-unseen}, and
the CDFs of the error graph is shown in Fig.~\ref{fig:comprehensive-unseen}c-d.
Similar to earlier results for practical, trained environments, RF, VO and EKF algorithms suffer 
with median errors of {e.g., 42cm, 48cm, 34cm in home env.}, respectively. BB and VINET tend to 
suffer the most with median error $>$50cm and max. error $>$1.2m (large trajectory deviations clearly visible in 
Fig.~\ref{fig:trajectory-unseen}).
BB and VINET's inability to generalize to unknown environments, combined with the practical environmental artifacts,
makes their performance deteriorate significantly.
\system's performance with a median error of only 18cm (office-3) and 23cm (Home), 
shows that {\em its hybrid fusion strategy really delivers in practical environments, 
to provide more than 2$\times$ and 3$\times$ better accuracy} than BB, VINET respectively.

\subsection{Scalability across Multiple Agents}
%Collaborative tracking (e.g. AR/VR) applications are becoming increasingly popular. With that 
Keeping collaborating  (e.g. AR/VR) applications in mind, we evaluate \system's ability
to track multiple agents (users) with respect to each other. We have upto three users moving simultaneously along the same trajectory,
but in different directions. To capture the tracking accuracy across multiple users simultaneously, we calculate the mean error in the relative positions for every pair of users. For every user-pair, this in turn, is captured jointly by the error in their relative distance and angle compared to ground truth. 
%for each 
%user with respect to all other users.
%Note that, %in a 2D plane when it comes to multi-user scenarios, 
%the error in relative position is given by both distance and angle.
In the interest of space, we show the results (Fig.~\ref{fig:multi-user}) for only two environments (trained office and unseen home environment) in 
practical conditions. % (NLoS RF anchors and dim-light), 
%when 3 users are walking. 
For results of other scenarios, users can take a look at~\cite{tech-report}.
%The graphs in Fig.~\ref{fig:multi-user} shows the CDFs of mean error in relative distance and relative angles, calculated at each data-point across 
%all the users. 
{\em \system, with its ability to absolutely localize every user (with help of anchors), and 
leverage dual-layer diversity, performs best with 30cm, 35cm relative-distance, 2.5$^{\circ}$, 3$^{\circ}$
relative-angular errors in trained and unseen environments, respectively. With gains increasing for more users,  it can scale to collaborative 
applications easily even in unseen environments.} This is a
1.2$\times$ (distance) and 1.6$\times$ (angle) improvement over BB and VINET respectively. 
RF, VO and EKF perform better than BB and VINET owing to better robustness, but still underperform \system
by 36\%, 41\% and 35\% respectively, with respect to relative-distance error. 

\subsection{Low Training Requirements}
In addition to bringing robustness to new environments, {\em the reduced burden on \system's fusion module,
enables it to operate at a significantly reduced training cost compared to pure ML-driven solutions.} 
Fig.~\ref{fig:trainingdata} shows \system's performance as an increasing function of training data size (out of entire dataset available to BB).
\system is able to reduce the training size requirements by over 60\%, while still delivering a comparable performance. 

\begin{figure}
\centering
      \vspace{-0.1cm}
      \includegraphics[width=0.95\linewidth]{figs/trainingdataresult.pdf}
      \vspace{-0.4cm}
      \caption{Training data size vs. tracking performances.}
     \label{fig:trainingdata}
\vspace{-0.4cm}
\end{figure} 

\subsection{Low Latency and Memory Requirements} \label{sec:syseff}
We evaluate the end-to-end running time %latency 
and memory requirements of \system (in table~\ref{tab:syseff}) to highlight its readiness 
for real-time operation on resource-constrained platforms. We use the following two platforms 
to measure the running time and latency for \system, BB 
and VINET. 1) A desktop machine with Ubuntu 18.04 OS 
%({\color{red}CPU speed and No. of CPU/GPU}) and
2) A Jetson TX2~\cite{jetsontx2}, a mobile-grade device. 
%({\color{red}CPU speed and No. of CPU/GPU}). 

The total running time of \system is significantly lower than BB %and VINET 
on desktop machines. On the Jetson Tx2, we were unable to run BB %and VINET
(as they require more neural network layers compared to \system, to extract features from raw 
images with 848x800 resolution) owing to their need for
a larger processing-capacity. Furthermore, since \system's latency is largely contributed by 
its component VO algorithm (compared to its fusion module), 
we believe that adopting solutions from ~\cite{ben2020edge} can drastically reduce VO's processing time, 
and hence \system's latency further, making it very attractive for real-time operation on resource-constrained mobile platforms.

\begin{table}[t]
  \centering
     \caption{Runtime and Memory utilization - ROVAR Vs. Baseline solutions ($^*$downsampled and measured for 480p resolution due to memory constraints).}
  \vspace{-0.3cm}
  \scalebox{0.89}{
  \begin{tabular}{|l|c|c|c|c|c|}
  %\hline 
  \hline
      \textbf{ } & \textbf{RF} & \textbf{VO} & \textbf{BB} & \textbf{\system} & \textbf{\system} \\
       &   &   &   & \textbf{Fusion} & \textbf{Overall} \\
    \hline
    %\hline
    Desktop (ms)  & 1.80 & 43.67     & 126.91    & 2.61  & 48.08 \\ \hline
    Jetson TX2 (ms)  & 3.20 & 61.67  & 348$^*$ & 5.34 & 70.31\\ \hline
    Model/Binary size & 13KB  &  100KB & 341.15MB & 5.05MB & 5.28MB \\ \hline %\hline
  \end{tabular}
    }
  \label{tab:syseff}
  \vspace{-0.6cm}
\end{table}


%The table shows that \system is indeed light-weight, that can easily run in real-time.

%\smallskip
%\noindent \textbf{Effect of trajectory shapes and environments:} Figure \ref{fig:comprehensive}a-c shows 
%the impact of different shapes on tracking performance while walking along these trajectories. 
%We deliberately consider different shapes as users in practice follow random paths, especially in open 
%environments. Figure shows that, \system achieves the lowest error out all the existing methods with 
%an average ATE of {\color{red}XXm}. More importantly, the max ATE of \system is well under 60cm across all three 
%trajectories. The state-of-the-art fusion solutions such as BB and EKF does perform better than the 
%individual algorithmic solutions, however, their error is still more than \system. 
%
%The Figure also shows that there is a slight change the tracking performance across the trajectories. 
%For example, even though the rectangle and S-shaped curve trajectories are in the same indoor open space, 
%the rectangle trajectory has slightly more error. This is because of the small drift accumulated at the 
%sharp turns (we will show impact of such abrupt turns in \S\ref{label:extremeconditions}). Similarly, 
%the error in case of the semi-construction space trajectory is more (by XXm) than the indoor open space 
%area. There are two reasons behind--- i) the RF anchors are placed in a wider space (40mx30m area) in the 
%latter case while the former case is smaller space (20mx20m), and therefore there is more ranging error 
%because of the coverage and occasional NLOS conditions due to pillars in the construction area, ii) 
%the VO tracking is weaker here because of the glass wall with outdoor environment having less features 
%than the indoor spaces.   
%
%\smallskip
%\noindent \textbf{Effect of motion:} We study the \system's performance under different users' motions--- walking and running. As users follow different speeds while moving around, studying the impact of motion is important. Figure \ref{fig:comprehensive}d-e shows the impact of running on the same trajectories mentioned above. Again, \system is the best performing solution among all with an average ATE of XXm and a maximum ATE of YYm. The average ATE under running scenario is slightly more than the walking scenario. We find that this increase is mostly due to VO-tracking being sensitive to motion. In our experiments, we find that the matching keypoints are significantly less (by XX\%) in the running case compared to walking case. The RF tracking is less affected compared to VO because there is no change in anchors' LOS conditions.

% \begin{figure}[t]
% \centering
%         \subfloat[]{%
%       \includegraphics[width=\linewidth]{figs/att-eval-trajectory.png} 
%      }

%     \subfloat[]{%
%       \includegraphics[width=\linewidth]{figs/att-eval-error.png} 
%      }
%       \caption{Dissecting the attention mask for RF and VO (e.g., NLOS for RF and Dim-lit for VO).}
%      \label{fig:attention}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \subfloat[Unseen Place1 Trajectory]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-place1-trajectory.png} 
%      }
%         \subfloat[Unseen Place1 Error]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-place1-error.png}  
%      }
     
%     \subfloat[Unseen Place2 Trajectory]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-place2-trajectory.png} 
%      }
%         \subfloat[Unseen Place2 Error]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-place2-error.png}  
%      }
%     \label{fig:unseen}
% \end{figure}

%  \begin{figure}[t]
%  \centering
%      \subfloat[Unseen Place3 walking]{%
%       \includegraphics[width=0.8\linewidth]{figs/home-well-lit-walking.pdf} 
%       }
    
%      \subfloat[Unseen Place3 Running]{%
%       \includegraphics[width=0.8\linewidth]{figs/home-well-lit-running.pdf} 
%       }
%       \caption{Home environment.}
%       \label{fig:place-home}
%  \end{figure}

% \subsection{Robustness to Extreme Conditions} \label{label:extremeconditions}
%Next, we study the resiliency of \system compared to other solutions when the sensors face unfavourable conditions for a short period of times. We deconstruct the effect of VO and RF by creating scenarios such that one faces regular environmental conditions while the other faces quick extreme conditions and evaluate how quickly \system is able to recover. We experiment with two types of experiments--- i) we create a scenario such that each sensor continues to track (albeit with drifted and larger errors) for the entire duration of the trajectory (e.g., acceptable dim lighting for VO and NLOS anchors for RF), ii) we create a scenario where one sensor complete loses track and hence \system relies completely on one sensor (e.g., total dark rooms for VO and out of coverage for RF).
%
%In summary, \system substantially outperforms all the competing methods with an average ATE of XXm and  a maximum ATE under well under 1m.
%
%\subsection{Generalizability in Unseen Environments}
%As described in \S\ref{label:bbdesign}, a classical limitation of learning through deep networks is hard to achieve generalizability. \system avoids this problem of generalization through algorithmic assistance. We show this by evaluating \system in two unseen environments and compare with the pure learning approaches along with the conventional methods. These two unseen places have different floor plan with different wall color and follow across corridors in an office environment, where as the training consists of large open spaces, semi-construction environment and small office room.
%
%Figure \ref{fig:unseen} shows the tracking performance across two different unseen trajectories. Despite the unseen environment, Figure shows that \system's trajectory is consistent with the ground truth trajectory and its performance similar to seen environments with a mean ATE of XXm and max ATE of YYm being consistent with the ATE from the seen environments. The main reason behind this impressive generalization is that \system's fusion is guided by algorithm intelligence through confidence features from tracking algorithms. However, BB fails to be consistent with the ground truth trajectory and results in large ATE across the entire trajectories with a mean ATE of XXm and max ATE of YYm. The primary reason behind this failure is that BB's fusion is guided by the learned high level features extracted through convolutions that are hard to capture the unseen features. Whereas in case of \system, the environmental conditions are abstracted through algorithm, and hence the generalization. 
%
%\subsection{Tracking Across Multiple Users} \label{label:multiusr-eval}
%
%Most of the tracking-based applications (e.g., first responders~\cite{}, medical training~\cite{}, Education~\cite{}, etc) involve multiple users interacting with each other. In order to have a seamless experience, these applications require accurate tracking of users relative to each other along with self-tracking. We study \system's tracking performance as we more users into the system and compare the with the state-of-the-art methods. To this end, we show two application use cases: one where 'relative' tracking sensitive and another 'additive' tracking sensitive application by reporting two error metrics--- i) relative error, ii) additive error. The relative error the difference in the estimated distance and the ground truth distance between two users. The additive error is a combined error of two users tracking relative to their ground truth. For more than two users, we compute the average of all users' tracking relative to all the other users.
%
%Figure \ref{fig:multi-user} shows the tracking performance of \system for 2 and 3 users and compared with BB. In both relative and additive case, \system outperforms the individual algorithms as well as BB. The benefits are as we more users and significantly better under additive scenario. In case of relative, we observe that RF-tracking is more consistent compared to VO because the latter is more sensitive where start and end as its drift accumulates towards the end of the trajectory.

% \begin{figure}[t]
% \centering
%     \subfloat[2 Users (Seen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/relative-error-2-users.png} 
%      }
%     \subfloat[3 Users (Seen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/relative-error-3-users.png}  
%      }
     
%     \subfloat[2 Users (Seen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/additive-error-2-users.png} 
%      }
%     \subfloat[3 Users (Seen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/additive-error-3-users.png}  
%      }
    
%     \subfloat[2 Users (Unseen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-relative-error-2users.png} 
%      }
%     \subfloat[3 Users (Unseen)]{%
%       \includegraphics[width=0.5\linewidth]{figs/unseen-relative-error-3users.png}  
%      }
%       \caption{Relative and additive error multiple users.}
%      \label{fig:multi-user}
% \end{figure}

%\subsection{Real-time Operation}
%
%We evaluate the real-time capability of \system and show that it outperforms the existing methods in terms of its system efficiency. We report latency results on two platforms: 1) Desktop-grade machine with a configuration described in \S\ref{label:prototype}, 2) Jetson TX2, a mobile-grade device. Table \ref{tab:syseff} compares the latency of \system with the algorithmic RF and VO solutions, and the blackbox model. 
%
%The table shows that \system fusion is highly light-weight and takes under 6ms even on the mobile platform. However, as an end-to-end system \system constitutes the algorithmic latency as well of our hybrid algorithm-assisted learning approach. The RF localization is also light-weight and takes under 3ms, whereas the VO (ORBSLAM3) is highly compute expensive. Together, \system's end-to-end latency comes down to XXms on Desktop and YYms on the mobile platform, translating to XX Fps and YY Fps respectively. 
%However, there is an extensive prior work in reducing the latency of VO solutions~\cite{} that significantly bring down the VO latency and therefore \system can be easily deployed in practice. Nevertheless, the end-to-end \system system is significantly faster than state-of-the-art blackbox solution by almost 3$\times$ on the Desktop. Moreover, the blackbox model cannot even be run on the mobile platform because of its high model complexity. As shown in the table, the model size of blackbox solution is 68$\times$ more compared to \system. This is because \system works on the algorithm-given features, whereas the blackbox solution needs additional neural network layers to extract features before the fusion.


==> implementation.tex <==
% implementation

In this section, we describe the details of various hardware and software components of \system system  prototype.

\subsection{\system Prototype} \label{label:prototype}

\noindent \textbf{UWB Module:} We use a set of Decawave EVK1000 UWB chips as anchors and tags to collect the two-way ranges. We modify its firmware to collect the received signal power along with the ranges. The two-way ranging is realized on the in-built micro-controller on the EVK board. We run the ranging protocol in 6GHz frequency band. We connect these boards to Raspberri Pis and collect the ranges and the signal quality data through a serial port. Each round of ranging takes about 80ms to collect ranges from all anchors. With additional TX and RX threading delays, we obtain the ranges at the rate of 10Hz. Once ranges are collect, we feed the ranges to a off-the-shelf multilateration algorithm for localization.

\smallskip
\noindent \textbf{ORBSLAM3 Module:} For visual tracking, we use ORBSLAM3 at state-of-the-art SLAM algorithm~\cite{}. We use Intel RealSense tracking camera (T265) to capture the video while moving around the tracks. The T265 has two Fisheye lens wide angle cameras with a resolution of 848x800 pixel resolution. The T265 also houses an IMU. We collect both the visual and IMU data together using the ROS platform as ROS bags and directly feed them to the ORBSLAM3 algorithm for the tracking.

\smallskip
\noindent \textbf{\system Model Training:} We use Pytorch, a commonly used deep learning platform to train our hybrid fusion algorithm. We split the data into train (70\%), validation (10\%), test (20\%) sets, and train our model using the standard train and validation procedure. Before feeding the data to the network, we normalize the input data by subtracting the mean over the dataset. We use Adam optimizer with L2 norm as the loss function during the training. As we show later, our model very lightweight and therefore takes less than an hour for training on a Desktop-grade Nvidia 1070 GPU.

To select a subset of the anchors, we adopt simple ML models such as SVM, Logistic regression, and an MLP. We experiment with each of these using a grid search to tune the hyper-parameters. We use Logistic regression in our system as it shows slightly better performance compared to other models both in terms of accuracy and the inference latency (see \S\ref{}).

\subsection{Experimental Setup} \label{label:setup}

\noindent \textbf{Groundtruth Deployment:} Much of the prior work uses expensive tracking systems such as VICON or bulky Lidar sensors to obtain mm-scale tracking and compare the tracking solutions relative to these. Costs up to 10s of thousands of dollars. Moreover, these are hard to scale across larger distances and different environments, difficult to carry around in hand. Where are cheaper sensors such Kinnect and lightweight Lidar sensors similar in terms of accuracy but are susceptible to environmental conditions because of the limited depth sensing capabilities. Therefore lack of a high precision and reliable groundtruth system poses a nontrivial challenge in order for us to compare and validate \system's performance in practice. 

\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/implementation.png}
      \caption{Testbed for data collection: a) Groundtruth system consisting of RFID tracks deployed at a gap of every 10cm, b) Sensors (RF, VO, IMU) attached to a Rig that is carried by the users while moving along the track.}
     \label{fig:implementation}
\end{figure} 

To this end, we design a new groundtruth system for 2D-tracking using an RFID deployment that is low-cost, highly accurate, and more scalable than the expensive groundtruth solutions as shown in Figure \ref{fig:implementation}. We deploy fixed RFID tags on the ground one every 10cm, along dedicated trajectories (see the top portion of the figure). An RFID reader is used to read the Ids of these tags when moving around the fixed trajectories. We manually mark the location of each tag and construct the groundtruth trajectories by mapping the Ids from the reader their corresponding locations noted manually. We control the reader's transmit power as well as the antenna orientation to limit the reading range to about 10cm. Using an RPi, we read the timestamped Ids and the signal power of the tags at a rate of 10Hz. To make the groundtruth more accurate, we select Ids with high signal strength whenever there are more tags selected for a given timestamp.

\smallskip
\noindent \textbf{Data Collection:} We attach the sensors and the RFID reader to a long thin stick to collect the data as shown in Figure \ref{fig:implementation}. The RFID reader is attached at the bottom of the stick and the stick carried around the trajectories such that the reader is within ~10cm distance of the tags. To avoid offset issues, we attach both UWB tag and the T265 stereo camera along same vertical axis on the stick. The UWB and RFID tag are connected to RPi that is also attached to the stick, to collect the data from respective sensors. The camera sensor is connected to a laptop via a USB cable to capture the camera data. Rpi and the laptop are clock synced using a locally hosted NTP system so that the timestamps of all sensors are in sync.

\smallskip
\noindent \textbf{Testbed and Trajectories:} We lay out a wide variety of trajectories across different locations and different shapes to test our model rigorously. The dataset consists of hallways, office rooms, cubicles, corridors, conference rooms, and including a semi-outdoor construction space. In total, we deploy XXm long groundtruth trajectories and collect data under several environmental conditions across these locations. Specifically, we collect data under the following favourable as well as unfavourable conditions for the RF and VO tracking: i) LOS and NLOS anchors, ii) bright and dim lighting conditions, iii) walking, running and with random motions. In total, our dataset consists of XX traces consisting of YY measurement points. Finally, to validate the robustness of \system, we collect data in two completely unseen environments. 

==> implementation2.tex <==
%\subsubsection{\system - The system:}
{\bf \system - The system:}
We implement a hand held prototype of \system,
containing the following three modules: (a) Decawave EVK1000~\cite{dw1000evk} 
UWB radios for RF-based localization (\S\ref{sec:rfmodule}),
(b) Intel Realsense T265 stereo camera~\cite{intelrealsenset265}
connected to a Jetson Nano~\cite{}
for realtime VO tracking (\S\ref{sec:vomodule}) and 
(c) A ThingMagic M6E-Nano RFID reader~\cite{rfidreader} for Ground Truth (GT) measurements. 
The RFID reader and the UWB radio are connected to a
RaspberryPi-4 (RPi) %single board
computer via the RPi's serial and Ethernet ports, respectively. A Dell laptop running Ubuntu 18.04 OS is connected
to the Intel camera via an ethernet cable for recording the camera images. 
All the devices are time-synced using a local NTP server running on the
laptop. The picture in Fig.~\ref{fig:implementation} shows %a volunteer holding 
the \system prototype %(stick held vertically) 
of the entire setup. As seen in the picture, the camera, UWB and the RFID 
reader are all on the same vertical plane, ensuring that the location determined 
by each sensor are on the same X-Y plane.

%\subsubsection{Testbeds:} 
{\bf Testbeds:} 
We use several testbeds with varying scenery and lighting conditions 
for data collection and testing. The testbeds are setup across multiple floors of an indoor office and a home,
in locations that include: large carpeted rooms with artificial lights, semi-constructed cemented-area surrounded 
by glass walls, narrow and wide office corridors surrounded by numerous obstacles (either cubicles or offices) 
and finally in conference rooms leading out to narrow corridors.  Except one, all the testbeds 
allow for us to control the lighting conditions through light dimmers, while one testbed has only natural sunlight.
We use a subset of testbeds (trained environments) for data collection, while the rest are kept completely unseen 
for testing the generalizability of \system.
%In total, we have collected data from {\color{red}YY} different traces for training the \system models. We ensure 
%the datasets are diverse to avoid the case of over-fitting the \system models. 
Fig~\ref{fig:implementation} shows subset of testbeds deployed in office and home environments with different RFID tracks
for ground truth. \\
%\subsubsection{Data collection:} We ensure 
{\bf Data collection for Model training:} We ensure 
the datasets are diverse to avoid over-fitting the \system models.
Each testbed has 2-to-3 different trajectories that contain
simple straight lines to more complex curvy-trajectories. For each trajectory, we 
collect data in: (i) bright and dim lighting conditions, and (ii) when user is walking and
running. The UWB anchors %along different trajectories, 
are often occluded due to physical structures and hence the UWB data contain both LoS and NLoS ranges.
In total, we have collected data from 72 different traces, amounting to a total distance of 4800 meters, for training the \system models. \\
%\subsubsection{Ground Truth:}
\begin{figure}
\centering
      \includegraphics[width=0.9\linewidth]{figs/implementation.png}
      \vspace{-0.5cm}
      \caption{Testbed: RFID tracks for GT and \system prototype}
     \label{fig:implementation}
\vspace{-0.4cm}
\end{figure} 
{\bf Ground Truth:}
%\label{sec:gt}
We use RFID tags, placed continuously at every 10cm intervals along 
the user's walking path for ground truth data. While other modalities like Lidars are conducive for single-user ground-truth,
the physically deployed RFIDs provide absolute ground-truth, allowing for evaluation of multiple-agent tracking. 
We physically measure each RFID tag's X-Y location. As the user walks along
the predefined trajectories holding the \system prototype in the vertical position 
(see Fig.~\ref{fig:implementation}), the RPi which is connected to the RFID reader (with the antenna 
at the bottom of the stick) records a time-stamped EPC and
RSSI information of the RFID tag directly below it. The Tx power of the RFID reader is set to a minimum
so that the RFID antenna reads the RFID tag only when it is a couple of inches directly
above it (any additional tag that is rarely read is filtered using RSSI information). 
Further, the velocity of the device, derived from a short sliding window of tag reads (say, 20 tags), allows 
for accurate interpolation of location within the 10cm granularity.
%processing the RSSI information allows us to filter out erroneous tags, if and when more than one tag is read. 
We record the ground truth information at 50Hz.\\
%\subsubsection{UWB localization:}
{\bf UWB localization:}
%\label{sec:uwb}
We use 7 static anchors placed at known 
locations in each testbed (e.g., refer Fig~\ref{fig:implementation}).
The RPi connected to the client UWB radio on the \system prototype initiates
the two-way ranging protocol~\cite{dalce2014experimental} sequentially with each UWB anchor. 
\system implements an optimized ranging protocol, described in~\cite{dw1000evk}, to reduce
the total packet exchanges required for ranging with each anchor. Range estimates are
recorded with timestamps at 15Hz speed.
We use the geometry constrained least-squares multi-lateration 
algorithm~\cite{hua2014geometrical} to calculate the client UWB's 2D location.\\
%\subsubsection{ORB-SLAM3 VO:} 
{\bf ORB-SLAM3 VO:} 
We record the camera images from the Intel realsense T265 cameras~\cite{intelrealsenset265}
as the user moves around. The T265 has stereo cameras with fisheye lens and records images at
848x800 pixel resolution. The recorded camera images is time-synced with the
UWB and ground truth data. We use the open-source ORB-SLAM3 ROS implementation~\cite{campos2021orb}.
The camera images are fed to the ORB-SLAM3 algorithm as ROS bags and record the resulting 
VO output. While we do record the IMU information from the T265 camera, we have not yet integrated them in 
\system's models. We discuss more on integrating IMU into \system in \S\ref{DISC}.\\
%\subsubsection{Network training:}
{\bf Network training:}
We use 70\% of our dataset for model-training,
10\% for validation and 20\% for evaluation. We ensure that our
dataset is diverse to avoid the case of over-fitting. We use Pytorch~\cite{paszke2019pytorch}, an
open source machine-learning (ML) library to implement the \system models.
Before feeding the data to the network, we normalize the input data by subtracting 
the mean over the dataset. We use Adam optimizer with L2 norm as the loss function 
during the training. \system's  model is lightweight and takes less than an hour 
for training on a Desktop-grade Nvidia-1070 GPU.


%\subsection{\system Prototype} \label{label:prototype}
%\noindent \textbf{UWB Module:} We use a set of Decawave EVK1000 UWB chips as anchors and tags to collect the two-way ranges. We modify its firmware to collect the received signal power along with the ranges. The two-way ranging is realized on the in-built micro-controller on the EVK board. We run the ranging protocol in 6GHz frequency band. We connect these boards to Raspberri Pis and collect the ranges and the signal quality data through a serial port. Each round of ranging takes about 80ms to collect ranges from all anchors. With additional TX and RX threading delays, we obtain the ranges at the rate of 10Hz. Once ranges are collect, we feed the ranges to a off-the-shelf multilateration algorithm for localization.
%\smallskip
%\noindent \textbf{ORBSLAM3 Module:} For visual tracking, we use ORBSLAM3 at state-of-the-art SLAM algorithm~\cite{}. We use Intel RealSense tracking camera (T265) to capture the video while moving around the tracks. The T265 has two Fisheye lens wide angle cameras with a resolution of 848x800 pixel resolution. The T265 also houses an IMU. We collect both the visual and IMU data together using the ROS platform as ROS bags and directly feed them to the ORBSLAM3 algorithm for the tracking.

%\subsection{\system dataset:}The dataset is 
%split with 70\% of it used for model-training, 10\% for validation and the rest 20\% for evaluation. We ensure that the
%dataset is divided such that the training, validation and evaluation dataset is diverse and help us evaluate our model
%more thoroughly. We use Pytorch~\cite{} to train \system's algorithm. 

%To select a subset of the anchors, we adopt simple ML models such as SVM, Logistic regression, 
%and an MLP. We experiment with each of these using a grid search to tune the 
%hyper-parameters. We use Logistic regression in our system as it shows slightly 
%better performance compared to other models both in terms of accuracy and the 
%inference latency (see \S\ref{}).


%\subsection{Experimental Setup} \label{label:setup}

%\noindent \textbf{Groundtruth Deployment:} Much of the prior work uses expensive tracking systems such as VICON or bulky Lidar sensors to obtain mm-scale tracking and compare the tracking solutions relative to these. Costs up to 10s of thousands of dollars. Moreover, these are hard to scale across larger distances and different environments, difficult to carry around in hand. Where are cheaper sensors such Kinnect and lightweight Lidar sensors similar in terms of accuracy but are susceptible to environmental conditions because of the limited depth sensing capabilities. Therefore lack of a high precision and reliable groundtruth system poses a nontrivial challenge in order for us to compare and validate \system's performance in practice. 


%To this end, we design a new groundtruth system for 2D-tracking using an RFID deployment that is low-cost, highly accurate, and more scalable than the expensive groundtruth solutions as shown in Figure \ref{fig:implementation}. We deploy fixed RFID tags on the ground one every 10cm, along dedicated trajectories (see the top portion of the figure). An RFID reader is used to read the Ids of these tags when moving around the fixed trajectories. We manually mark the location of each tag and construct the groundtruth trajectories by mapping the Ids from the reader their corresponding locations noted manually. We control the reader's transmit power as well as the antenna orientation to limit the reading range to about 10cm. Using an RPi, we read the timestamped Ids and the signal power of the tags at a rate of 10Hz. To make the groundtruth more accurate, we select Ids with high signal strength whenever there are more tags selected for a given timestamp.


%\smallskip
%\noindent \textbf{Data Collection:} We attach the sensors and the RFID reader to a long thin stick to collect the data as shown in Figure \ref{fig:implementation}. The RFID reader is attached at the bottom of the stick and the stick carried around the trajectories such that the reader is within ~10cm distance of the tags. To avoid offset issues, we attach both UWB tag and the T265 stereo camera along same vertical axis on the stick. The UWB and RFID tag are connected to RPi that is also attached to the stick, to collect the data from respective sensors. The camera sensor is connected to a laptop via a USB cable to capture the camera data. Rpi and the laptop are clock synced using a locally hosted NTP system so that the timestamps of all sensors are in sync.
%
%\smallskip
%\noindent \textbf{Testbed and Trajectories:} We lay out a wide variety of trajectories across different locations and different shapes to test our model rigorously. The dataset consists of hallways, office rooms, cubicles, corridors, conference rooms, and including a semi-outdoor construction space. In total, we deploy XXm long groundtruth trajectories and collect data under several environmental conditions across these locations. Specifically, we collect data under the following favourable as well as unfavourable conditions for the RF and VO tracking: 


==> intro.tex <==
%intro
% Needs of growing services
	Industrial and enterprise automation, fueled by the pandemic, has contributed to a rapid
  growth in interactive and immersive applications such as augmented (AR) and virtual reality (VR)~\cite{jung2018augmented, munoz2020augmented} that are available not only on dedicated devices (e.g. headsets) but potentially even our smartphones. 
  These applications go beyond gaming to unlock significant value for various tasks like industrial training, collaborative robotics, remote 
  operation, etc.~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual} in the broader Industry 4.0 ecosystem.
 % are not just targeted at gaming, but are well-poised to deliver significant value 
  %in several other verticals in industry 4.0 ranging from logistics and supply chain to hospitality and
  %healthcare, for various tasks relating to industrial training, collaborative robotics, remote 
  %operation, etc.~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual}.  
  A key primitive central to delivering these applications is the ability 
  to provide accurate, cost-effective and robust tracking  of multiple agents (humans and robots) 
  involved in every-day, challenging environments. 

%current solutions and technical gaps in meeting needs
	{\bf Technical gaps in current solutions.}  The growing availability of visual (cameras), inertial (IMUs), and RF (WiFi, BLE, UWB) sensors on our everyday devices provides a rich substrate for effective tracking. Existing tracking solutions fall into two categories: passive and active (infrastructure-assisted) tracking. Passive tracking solutions~\cite{campos2021orb, bloesch2015robust, zhang2014loam, solin2018inertial} are largely odometry-based, a popular variant of which is visual inertial odometry (VIO) that combines and fuses cameras (stereo or mono) and inertial sensors. While this approach is cost-effective and can track to within few tens of cm accuracy  under favorable visual conditions, they are significantly vulnerable (1m+ error), when facing everyday environmental conditions like dim-light, texture-less surfaces, etc.~\cite{feigl2020localization, saputra2018visual}. Further, their inherent notion of {\em relative} tracking prevents them from robustly recovering from such unfavorable events, while also  limiting them from catering to multi-agent tracking within a global frame of reference. On the other hand, active tracking approaches~\cite{ni2017accurate, palacios2017jade, ibrahim2018verification, ruiz2017comparing} that involve the planned deployment of one or more anchors to locate agents, easily enable multi-agent tracking through {\em absolute} localization that eliminates error accumulation. However, notwithstanding the associated deployment overhead, they face a tradeoff in operational range and accuracy -- while high-resolution ( cm-level) tracking technologies (e.g. IR~\cite{kumar2014improving, jung2004ubitrack}, mmWave~\cite{zeng2016human, palacios2018communication}, acoustic~\cite{lollmann2018locata, fallon2011acoustic}) are restricted in range to LoS and room-level tracking, low-resolution (meter-level) tracking technologies (e.g. WiFi~\cite{venkatnarayan2020leveraging, ibrahim2018verification}, BLE~\cite{chen2017locating}) can handle NLoS and longer operational range but at the expense of reduced tracking accuracies.
  
\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/ravar-applications.png}
      \vspace{-0.6cm}
      \caption{Proposed system and its applications.}
     \label{fig:systemaandapplications}
\vspace{-0.5cm}
\end{figure} 
  
% case for a hybrid approach, that fuses active and passive tracking to enable robust, multi-agent tracking, and the challenges in making it happen
	{\bf Need for Dual-layer Diversity.} We advocate the need for a hybrid approach, that can effectively bring together the complementary benefits of active (absolute, multi-agent) and passive (relative, high resolution) tracking to enable {\em scalable and accurate multi-agent} tracking\footnote{We consider 2D position tracking in this work to focus more on the fusion methodology. We discuss in Section~\ref{DISC} how our approach can be extended to include orientation and hence pose in the future.}. While this forms the first layer that leverages  diversity in the sensor tracking {\em modalities}, this is not sufficient. Note that conventional, {\em algorithmic} sensor-fusion approaches (e.g. RF-IMU fusion~\cite{venkatnarayan2019enhancing, venkatnarayan2019measuring}) that offer this first layer of diversity are robust to operate in various environments in the wild, but are unable to effectively sift out the environmental artifacts as well as the erroneous artifacts of individual sensors and provide effective fusion that can deliver high accuracies sustainably. On the other hand, while the recent {\em data-driven}  approaches (e.g. visual-IMU~\cite{clark2017vinet}, mmwave-IMU~\cite{lu2020milliego} fusion) show promise for much better fusion, they have thus far targeted passive tracking with a black-box learning approach, leaving the problem of robust (generalizable to unseen environments) and scalable (multi-agent) tracking open. Hence, the fundamental challenge in realizing our vision for a robust, accurate, and scalable tracking solution lies in not only leveraging the diversity offered by the {\em modality of tracking} (active and passive), but also the diversity offered by the {\em methodology of fusion} --  in particular, figuring out when and how to leverage statistical learning in combination with closed-form algorithms.  
%	understanding how best to fuse the disparate modalities of active and passive tracking, and in particular figuring out when and how to leverage statistical learning in combination with closed-form algorithms for a scalable, accurate, multi-agent tracking solution.  

% our proposal: learning aided fusion of passive and active tracking
	{\bf \system:}  To this end, we propose \system (Fig.~\ref{fig:systemaandapplications}): a novel, accurate and robust multi-agent tracking solution that embodies effective fusion through diversity at two layers: it brings together the complementary benefits of active (RF - WiFi/UWB) and passive (visual - stereo cameras) tracking modalities, through an intelligent combination of both algorithmic and data-driven techniques. % to ensure high scalability and tracking accuracy across multiple agents.
 \system envisions a system, wherein agents carry a tracking device (e.g. headset, smart device) that houses an embedded stereo camera\footnote{Our framework and its benefits apply to monocular cameras as well, albeit with a slightly reduced accuracy, inherent to the limited visual input.} and a RF interface -- while the stereo camera enables visual odometry-based relative tracking, the RF interface enables absolute tracking by estimating ranges (and angles, AoA) to one or more access points (anchors) in the environment. RF technologies like WiFi and more so UWB offer a good balance between tracking resolution (160 Mhz with 802.11mc, 500 MHz with UWB) and robust NLoS operation, and are already appearing in our commodity access points and smartphones (Apple iPhone12, Samsung Galaxy S21, etc.)~\cite{appleu1chip, sammobileuwbchip}.  While \system employs UWB as its RF technology, its approach is equally applicable to WiFi as well, with its mmWave incarnation (60 GHz) offering access to much wider bandwidths. 
	
	\system leverages algorithmic solutions to estimate the absolute location estimate from RF (e.g. multi-lateration~\cite{cheung2006constrained, hua2014geometrical} or range+AoA~\cite{herath2013optimal} approaches) and the relative translation estimate from visual (e.g. ORB-SLAM3~\cite{campos2021orb}), while data-driven models assist with data filtering, feature composition and the fusion itself, as follows: (i) {\em data filtering} plays a significant role in isolating RF range estimates that are impacted by NLOS and significantly degrade the localization accuracy; (ii) {\em feature composition} enables estimating the certainty of the absolute and relative position estimates delivered by the individual RF and visual sensor algorithms by accounting for their  environmental and sensor artifacts, and together form their respective sensor features; and (iii) {\em fusion} allows for the model to jointly consider the sensor streams and automatically attend to the appropriate sensor estimates based on their features and relative importance (deficiencies) at any given instant to provide robustness, and maintain a high tracking accuracy consistently. Allowing the individual sensor algorithms to provide estimates along with their certainty to the sensor fusion model, leverages the physics and geometry inherent to these localization problems. This eliminates the burden on the fusion model from capturing this complex problem structure purely from data, allowing it to focus solely on effective fusion and accurately predicting the absolute position estimate. This also reduces the compute and latency requirements for running \system on the target device significantly, allowing for real-time operation on resource-constrained devices, in contrast to compute-intensive data-driven approaches. Predicting an absolute (compared to relative) position estimate directly from the raw features is especially challenging for a model (i.e. a black-box approach), forcing it to rely heavily on the input data, and significantly limits its ability to generalize. In contrast, \system's approach contributes to a robust model that brings the best of both worlds, allowing the solution to generalize well and be deployed in unseen environments that it has not been trained for.    
	
% implementation and evaluation highlights
	\system is built as a hand-held prototype comprising  a UWB beacon, stereo-camera, and portable RFID reader (for ground-truth) and 
  experimented under diverse environments spanning 4500 sq.ft. area at 5 different places for a 
  total of 232,000 tracked data points across 3 agents. Comprehensive evaluations reveal the 
  importance of \system's proposed dual-layer diversity framework, where active RF tracking 
  eliminates the accumulation of errors, while leveraging the high resolution offered by the 
  visual sensor, to provide median tracking accuracy of {\texttt 15 cm}. This is in contrast to 
  {\texttt 40} and {\texttt 32 cm} accuracy offered by RF and visual tracking solutions respectively 
  in isolation.  A high median accuracy of {\texttt 30 cm} even in unseen, challenging environments, 
  further emphasizes the robustness delivered by \system's hybrid fusion approach in everyday environments, 
  compared to the {\texttt 60} and {\texttt 80 cm} accuracies offered by its algorithmic and pure 
  data-driven counterparts. \system incurs a memory footprint of \texttt{5 MB}, 60\% less training data, 
  and end-to-end execution latency of \texttt{70 msec} (a \texttt{5} fold improvement) over a pure data-driven 
  approach, enabling real-time operation on mobile platforms such as Jetson TX2.
% contributions
	Our contributions in this work are multi-fold:
%\noindent \textbf{(1)} We advocate the need for dual-layer diversity in both {\em tracking modality} (active + passive) and {\em fusion methodology} (algorithmic + data-driven) to enable accurate, robust, and scalable tracking in everyday environments (Sec.~\ref{MOTIV}). 
%
%\noindent \textbf{(2)} We design and build \system as an instantiation of our framework that embodies the dual-layer diversity approach to fusion of visual and RF sensing (Sec.~\ref{DESIGN}). 
%
%\noindent \textbf{(3)}  We comprehensively evaluate and showcase the benefits of \system's framework and its ability to track multiple agents robustly in unseen environments (Sec.~\ref{EVAL}).  
	\begin{itemize}
	\item{} We advocate the need for dual-layer diversity in both {\em tracking modality} (active + passive) and {\em fusion methodology} (algorithmic + data-driven) to enable accurate, robust, and scalable tracking in everyday environments (Sec.~\ref{MOTIV}). 
	\item{} We design and build \system as an instantiation of our framework that embodies the dual-layer diversity approach to fusion of visual and RF sensing (Sec.~\ref{DESIGN}). 
	\item{} We comprehensively evaluate and showcase the benefits of \system's framework and its ability to track multiple agents robustly in unseen environments (Sec.~\ref{EVAL}).  
	\end{itemize}

We discuss directions for how \system can reduce RF infrastructure overhead, extend to incorporate inertial sensors, and deliver absolute pose in Sec.~\ref{DISC}.
We also plan to release our unique, time-synced, rich dataset of UWB, camera and RFID (ground-truth) sensor streams, hoping it brings value to the community in fostering research in this space. 


==> intro1.tex <==
%intro
% Needs of growing services
	Industrial and enterprise automation, fueled by the pandemic, has contributed to a rapid
  growth in interactive and immersive applications such as augmented (AR) and virtual reality (VR)~\cite{jung2018augmented, munoz2020augmented} that are available not only on dedicated devices (e.g. headsets) but potentially even our smartphones. 
  These applications go beyond gaming to unlock significant value for various tasks like industrial training, collaborative robotics, remote 
  operation, etc.~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual} in the broader Industry 4.0 ecosystem.
 % are not just targeted at gaming, but are well-poised to deliver significant value 
  %in several other verticals in industry 4.0 ranging from logistics and supply chain to hospitality and
  %healthcare, for various tasks relating to industrial training, collaborative robotics, remote 
  %operation, etc.~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual}.  
  A key primitive central to delivering these applications is the ability 
  to provide accurate, cost-effective and robust tracking  of multiple agents (humans and robots) 
  involved in every-day, challenging environments. 

%current solutions and technical gaps in meeting needs
	{\bf Technical gaps in current solutions.}  The growing availability of visual (cameras), inertial (IMUs), and RF (WiFi, BLE, UWB) sensors on our everyday devices provides a rich substrate for effective tracking. Existing tracking solutions fall into two categories: passive and active (infrastructure-assisted) tracking. Passive tracking solutions~\cite{campos2021orb, bloesch2015robust, zhang2014loam, solin2018inertial} are largely odometry-based, a popular variant of which is visual inertial odometry (VIO) that combines and fuses cameras (stereo or mono) and inertial sensors. While this approach is cost-effective and can track to within few tens of cm accuracy  under favorable visual conditions, they are significantly vulnerable (1m+ error), when facing everyday environmental conditions like dim-light, texture-less surfaces, etc.~\cite{feigl2020localization, saputra2018visual}. Further, their inherent notion of {\em relative} tracking prevents them from robustly recovering from such unfavorable events, while also  limiting them from catering to multi-agent tracking within a global frame of reference. On the other hand, active tracking approaches~\cite{ni2017accurate, palacios2017jade, ibrahim2018verification, ruiz2017comparing} that involve the planned deployment of one or more anchors to locate agents, easily enable multi-agent tracking through {\em absolute} localization that eliminates error accumulation. However, notwithstanding the associated deployment overhead, they face a tradeoff in operational range and accuracy -- while high-resolution ( cm-level) tracking technologies (e.g. IR~\cite{kumar2014improving, jung2004ubitrack}, mmWave~\cite{zeng2016human, palacios2018communication}, acoustic~\cite{lollmann2018locata, fallon2011acoustic}) are restricted in range to LoS and room-level tracking, low-resolution (meter-level) tracking technologies (e.g. WiFi~\cite{venkatnarayan2020leveraging, ibrahim2018verification}, BLE~\cite{chen2017locating}) can handle NLoS and longer operational range but at the expense of reduced tracking accuracies.
  
\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/ravar-applications.png}
      \vspace{-0.6cm}
      \caption{Proposed system and its applications.}
     \label{fig:systemaandapplications}
\vspace{-0.5cm}
\end{figure} 
  
% case for a hybrid approach, that fuses active and passive tracking to enable robust, multi-agent tracking, and the challenges in making it happen
	{\bf Need for Dual-layer Diversity.} We advocate the need for a hybrid approach, that can effectively bring 
 together the complementary benefits of active (absolute, multi-agent) and passive (relative, high resolution) 
 tracking to enable {\em scalable and accurate multi-agent} tracking\footnote{We consider 2D position tracking in this work 
 to focus on the fusion methodology. In \S~\ref{DISC} we discuss how our approach can be extended %to include orientation and hence pose
 for 3D tracking in the future.}. While this forms the first layer that leverages 
 diversity in the sensor tracking {\em modalities}, this is not sufficient. Conventional
 {\em algorithmic} sensor-fusion approaches (e.g. RF-IMU fusion~\cite{venkatnarayan2019enhancing, 
 venkatnarayan2019measuring}) that offer this first layer of diversity are robust to operate in 
 various environments in the wild, but are unable to effectively sift out the 
 %environmental artifacts as well  and the 
 erroneous artifacts of individual sensors and provide effective 
 fusion that can deliver high accuracies sustainably. On the other hand, while the recent 
 {\em data-driven}  approaches (e.g. visual-IMU~\cite{clark2017vinet}, mmwave-IMU~\cite{lu2020milliego} fusion) 
 show promise for much better fusion, they have thus far targeted passive tracking with a black-box 
 learning approach, leaving the problem of robust (generalizable to unseen environments) and 
 scalable (multi-agent) tracking open. Hence, the fundamental challenge in realizing our vision 
 for a robust, accurate, and scalable tracking solution lies in not only leveraging the diversity
 offered by the two {\em modality of tracking} (active and passive), but also the diversity offered 
 by the {\em methodology of fusion} --  in particular, figuring out when and how to leverage statistical 
 learning in combination with closed-form algorithms.  
%	understanding how best to fuse the disparate modalities of active and passive tracking, and in particular figuring out when and how to leverage statistical learning in combination with closed-form algorithms for a scalable, accurate, multi-agent tracking solution.  

% our proposal: learning aided fusion of passive and active tracking
{\bf \system:}  To this end, we propose \system (Fig.~\ref{fig:systemaandapplications}): a novel, 
accurate and robust multi-agent tracking solution that embodies effective fusion through diversity 
at two layers: it brings together the complementary benefits of active (RF - WiFi/UWB) and passive 
(visual - stereo cameras) tracking modalities through an intelligent combination of both algorithmic 
and data-driven techniques. % to ensure high scalability and tracking accuracy across multiple agents.
 \system envisions a system, wherein agents carry a tracking device (e.g. headset, smart device) that houses an embedded stereo camera\footnote{Our framework and its benefits apply to monocular cameras as well, albeit with a slightly reduced accuracy, inherent to the limited visual input.} and a RF interface -- while the stereo camera enables visual odometry-based relative tracking, the RF interface enables absolute tracking by estimating ranges (and angles, AoA) to one or more access points (anchors) in the environment. RF technologies like WiFi and more so UWB offer a good balance between tracking resolution (160 Mhz with 802.11mc, 500 MHz with UWB) and robust NLoS operation, and are already appearing in our commodity access points and smartphones (Apple iPhone12, Samsung Galaxy S21, etc.)~\cite{appleu1chip, sammobileuwbchip}.  While \system employs UWB as its RF technology, its approach is equally applicable to WiFi as well, with its mmWave incarnation (60 GHz) offering access to much wider bandwidths. 
	
	\system leverages algorithmic solutions to estimate the absolute location estimate from RF (e.g. multi-lateration~\cite{cheung2006constrained, hua2014geometrical} or range+AoA~\cite{herath2013optimal} approaches) and the relative translation estimate from visual (e.g. ORB-SLAM3~\cite{campos2021orb}), while data-driven models assist with data filtering, feature composition and the fusion itself, as follows: (i) {\em data filtering} plays a significant role in isolating RF range estimates that are impacted by NLOS and significantly degrade the localization accuracy; (ii) {\em feature composition} enables estimating the certainty of the absolute and relative position estimates delivered by the individual RF and visual sensor algorithms by accounting for their  environmental and sensor artifacts, and together form their respective sensor features; and (iii) {\em fusion} allows for the model to jointly consider the sensor streams and automatically attend to the appropriate sensor estimates based on their features and relative importance (deficiencies) at any given instant to provide robustness, and maintain a high tracking accuracy consistently. Allowing the individual sensor algorithms to provide estimates along with their certainty to the sensor fusion model, leverages the physics and geometry inherent to these localization problems. This eliminates the burden on the fusion model from capturing this complex problem structure purely from data, allowing it to focus solely on effective fusion and accurately predicting the absolute position estimate. This also reduces the compute and latency requirements for running \system on the target device significantly, allowing for real-time operation on resource-constrained devices, in contrast to compute-intensive data-driven approaches. Predicting an absolute (compared to relative) position estimate directly from the raw features is especially challenging for a model (i.e. a black-box approach), forcing it to rely heavily on the input data, and significantly limits its ability to generalize. In contrast, \system's approach contributes to a robust model that brings the best of both worlds, allowing the solution to generalize well and be deployed in unseen environments that it has not been trained for.    
	
% implementation and evaluation highlights
	\system is built as a hand-held prototype comprising  a UWB beacon, stereo-camera, and portable RFID reader (for ground-truth) and 
  experimented under diverse environments spanning 4500 sq.ft. area at 5 different places for a 
  total of 232,000 tracked data points across 3 agents. Comprehensive evaluations reveal the 
  importance of \system's proposed dual-layer diversity framework, where active RF tracking 
  eliminates the accumulation of errors, while leveraging the high resolution offered by the 
  visual sensor, to provide median tracking accuracy of {\texttt 15 cm}. This is in contrast to 
  {\texttt 40} and {\texttt 32 cm} accuracy offered by RF and visual tracking solutions respectively 
  in isolation.  A high median accuracy of {\texttt 30 cm} even in unseen, challenging environments, 
  further emphasizes the robustness delivered by \system's hybrid fusion approach in everyday environments, 
  compared to the {\texttt 60} and {\texttt 80 cm} accuracies offered by its algorithmic and pure 
  data-driven counterparts. \system incurs a memory footprint of \texttt{5 MB}, 60\% less training data, 
  and end-to-end execution latency of \texttt{70 msec} (a \texttt{5} fold improvement) over a pure data-driven 
  approach, enabling real-time operation on mobile platforms such as Jetson TX2.
% contributions
	Our contributions in this work are multi-fold:
%\noindent \textbf{(1)} We advocate the need for dual-layer diversity in both {\em tracking modality} (active + passive) and {\em fusion methodology} (algorithmic + data-driven) to enable accurate, robust, and scalable tracking in everyday environments (Sec.~\ref{MOTIV}). 
%
%\noindent \textbf{(2)} We design and build \system as an instantiation of our framework that embodies the dual-layer diversity approach to fusion of visual and RF sensing (Sec.~\ref{DESIGN}). 
%
%\noindent \textbf{(3)}  We comprehensively evaluate and showcase the benefits of \system's framework and its ability to track multiple agents robustly in unseen environments (Sec.~\ref{EVAL}).  
	\begin{itemize}
	\item{} We advocate the need for dual-layer diversity in both {\em tracking modality} (active + passive) and {\em fusion methodology} (algorithmic + data-driven) to enable accurate, robust, and scalable tracking in everyday environments (Sec.~\ref{MOTIV}). 
	\item{} We design and build \system as an instantiation of our framework that embodies the dual-layer diversity approach to fusion of visual and RF sensing (Sec.~\ref{DESIGN}). 
	\item{} We comprehensively evaluate and showcase the benefits of \system's framework and its ability to track multiple agents robustly in unseen environments (Sec.~\ref{EVAL}).  
	\end{itemize}

We discuss directions for how \system can reduce RF infrastructure overhead, extend to incorporate inertial sensors, and deliver absolute pose in Sec.~\ref{DISC}.
We also plan to release our unique, time-synced, rich dataset of UWB, camera and RFID (ground-truth) sensor streams, hoping it brings value to the community in fostering research in this space. 


==> intro2.tex <==
%intro
% Needs of growing services
	Industrial and enterprise automation, fueled by the pandemic, has contributed to a rapid
  growth in interactive and immersive applications such as augmented (AR) and virtual reality (VR)~\cite{jung2018augmented, munoz2020augmented} that are available not only on dedicated devices (e.g., headsets) but also potentially on
  our smartphones. 
  These applications go beyond gaming to unlock significant value for various tasks like industrial training, collaborative robotics and remote 
  operation~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual}.
 %in the broader Industry 4.0 ecosystem.
 % are not just targeted at gaming, but are well-poised to deliver significant value 
  %in several other verticals in industry 4.0 ranging from logistics and supply chain to hospitality and
  %healthcare, for various tasks relating to industrial training, collaborative robotics, remote 
  %operation, etc.~\cite{ong2013virtual, piumsomboon2017covar, williams2018virtual}.  
  A key primitive central to delivering these applications is the ability 
  to provide robust, accurate and cost-effective tracking  of multiple agents (humans and robots) 
  involved in everyday environments that can often present challenging test cases. 

%current solutions and technical gaps in meeting needs
	{\bf Technical gaps in current solutions.}  The growing availability of visual (cameras), inertial (IMUs), and RF (WiFi, BLE, UWB) sensors on our everyday devices provides a rich substrate for effective tracking. Existing tracking solutions for floor or enterprise-level applications fall into two categories: passive and active (infrastructure-assisted) tracking. Passive tracking solutions~\cite{campos2021orb, bloesch2015robust, zhang2014loam, solin2018inertial} are largely odometry-based methods that use cameras and inertial sensors. While this approach is cost-effective and can track to within few tens of cm accuracy under favorable conditions, they are significantly vulnerable (1m+ error), when facing everyday environmental conditions like dim-light, texture-less surfaces, etc.~\cite{feigl2020localization, saputra2018visual}. Further, their inherent notion of {\em relative} tracking prevents them from robustly recovering from unfavorable events, while also limiting them from multi-agent tracking within a global frame of reference. On the other hand, active tracking approaches~\cite{ni2017accurate, palacios2017jade, ibrahim2018verification, ruiz2017comparing} that involve the planned deployment of one or more anchors to locate agents, easily enable multi-agent tracking through {\em absolute} localization that eliminates error accumulation. Notwithstanding the deployment overhead, they face a tradeoff in operational range and accuracy -- while high-resolution ( cm-level) tracking technologies (e.g. IR~\cite{kumar2014improving}, mmWave~\cite{zeng2016human, palacios2018communication}, acoustic~\cite{lollmann2018locata}) are restricted to LoS and room-level tracking, low-resolution (meter-level) tracking technologies (e.g. WiFi~\cite{venkatnarayan2020leveraging, ibrahim2018verification}, BLE~\cite{chen2017locating}) can handle NLoS and longer operational range but at the expense of reduced tracking accuracy.
  
\begin{figure}[t]
\centering
      \includegraphics[width=\linewidth]{figs/ravar-applications.png}
      \vspace{-0.6cm}
      \caption{Proposed system and its applications.}
     \label{fig:systemaandapplications}
\vspace{-0.5cm}
\end{figure} 
  
% case for a hybrid approach, that fuses active and passive tracking to enable robust, multi-agent tracking, and the challenges in making it happen
{\bf Need for Dual-layer Diversity.} We advocate the need for a hybrid approach, that can effectively bring 
together the complementary benefits of active (absolute, multi-agent) and passive (relative, high resolution) 
tracking to enable {\em scalable and accurate multi-agent} tracking\footnote{We consider 2D position tracking in this work 
to focus on the fusion methodology. Details on extending it to 3D tracking can be found in~\cite{tech-report}.} %to include orientation and hence pose}.
While this forms the first layer that leverages 
diversity in the sensor tracking {\em modalities}, this is not sufficient. Conventional
{\em algorithmic} sensor-fusion approaches (e.g. RF-IMU fusion~\cite{venkatnarayan2019enhancing, 
venkatnarayan2019measuring}) that offer this first layer of diversity are robust to operate in 
various environments in the wild, but are unable to effectively sift out the 
%environmental artifacts as well 
erroneous artifacts of individual sensors and provide effective 
fusion that can deliver high accuracies sustainably. On the other hand, while the recent 
{\em data-driven}  approaches (e.g. visual-IMU~\cite{clark2017vinet}, milliEgo~\cite{lu2020milliego}) 
show promise for much better fusion, they have thus far targeted passive tracking (with a black-box learning approach) or relative tracking in a small area. Hence, the fundamental challenge in realizing our vision 
for a robust, accurate, and scalable tracking solution lies in not only leveraging the diversity
offered by the two {\em modality of tracking} (active and passive), but also the diversity offered 
by the {\em methodology of fusion} --  in particular, figuring out when and how to leverage statistical 
learning in combination with closed-form algorithms.  
%	understanding how best to fuse the disparate modalities of active and passive tracking, and in particular figuring out when and how to leverage statistical learning in combination with closed-form algorithms for a scalable, accurate, multi-agent tracking solution.  

% our proposal: learning aided fusion of passive and active tracking
{\bf \system:}  To this end, we propose \system (Fig.~\ref{fig:systemaandapplications}): a novel, 
accurate and robust multi-agent tracking solution sufficiently lightweight to run 
in real-time on a low-end portable GPU device, that embodies effective fusion through diversity 
at two layers: it brings together the complementary benefits of active (RF - WiFi/UWB) and passive 
%(visual - stereo cameras) tracking modalities through an intelligent combination of both algorithmic 
(visual) tracking modalities through an intelligent combination of both algorithmic 
and data-driven techniques. % to ensure high scalability and tracking accuracy across multiple agents.
\system envisions a system, wherein agents carry a tracking device (e.g. headset, smart device) that
%houses an embedded stereo camera\footnote{\system's framework and its benefits apply to monocular cameras 
houses an embedded camera (either stereo or monocular)
%\footnote{\system's framework and its benefits apply to monocular cameras 
%as well, albeit with a slightly reduced accuracy, inherent to the limited visual input.} 
and an RF interface. While the camera enables visual odometry-based relative tracking, the RF interface 
enables absolute tracking by estimating ranges (and angles, AoA) to one or more access points (anchors)
in the environment. RF technologies like WiFi and more so UWB offer a good balance between tracking 
resolution (160 Mhz with 802.11mc, 500 MHz with UWB) and robust NLoS operation, and are already deployed
in many commodity access points and smartphones (Apple iPhone12, Samsung Galaxy S21, etc.)~\cite{appleu1chip, sammobileuwbchip}. 
While \system employs UWB, its approach is equally applicable to 
other RF technologies (e.g., WiFi).

\system leverages algorithmic solutions to estimate the absolute location estimate from RF 
(e.g. multi-lateration~\cite{cheung2006constrained, hua2014geometrical} or 
range+AoA~\cite{herath2013optimal} approaches) and the relative translation estimate from 
visual (e.g. ORB-SLAM3~\cite{campos2021orb}), while data-driven model assists in data filtering,
feature composition and the fusion itself, as follows: (i) {\em data filtering} plays a significant 
role in isolating RF range estimates that are impacted by NLOS and significantly degrade the 
localization accuracy; (ii) {\em feature composition} enables estimating the certainty of the 
absolute and relative position estimates delivered by the individual RF and visual algorithms 
by accounting for their  environmental and sensor artifacts, and together form their respective 
sensor features; and (iii) {\em fusion} allows for the model to jointly consider the sensor streams 
and automatically attend to the appropriate sensor estimates based on their features and 
relative importance (deficiencies) at any given instant to provide robustness, and maintain a high
tracking accuracy. Allowing individual sensor algorithms to provide estimates 
along with their certainties to the fusion model leverages the physics and geometry inherent to these 
localization problems. This relieves the fusion model from capturing this complex 
problem purely from data, allowing it to focus solely on effective fusion and accurately 
predicting the absolute position estimate. This also reduces the compute and latency requirements 
enabling \system to run in real-time even on 
resource-constrained devices, in contrast to compute-intensive data-driven approaches. Predicting an 
absolute (compared to relative) position estimate directly from the raw features is 
challenging for a model (i.e. a black-box approach), forcing it to rely heavily on the input data
and thus limiting its ability to generalize. In contrast, \system's approach contributes to 
a robust model that brings the best of both worlds, allowing the solution to generalize well and be 
easily deployed in untrained environments.    
	
\system is built as a hand-held prototype comprising a UWB beacon and intel T265 stereo-camera, experimented in diverse environments spanning 4500 sq.ft. area at multiple locations for a 
total of 232,000 tracked data points across 3 agents. Comprehensive evaluations reveal the importance
of \system's proposed dual-layer diversity framework, where active
RF tracking eliminates the accumulation of errors, while leveraging
the high resolution offered by the visual sensor, to provide median
tracking accuracy of 15 cm. This is in contrast to 40 and 32 cm
accuracy offered by RF and visual tracking solutions respectively
in isolation. \system\ requires small memory footprint of
\texttt{5MB}, 60\% less training data, and an end-to-end execution latency of 
of \texttt{72 msec} (a \texttt{5X} improvement) over a pure data-driven 
approach, enabling real-time operation on mobile platforms like Jetson Nano/TX2~\cite{jetsontx2}.
Contributions in this work are multifold:\\
{\bf (1)} We advocate the need for dual-layer diversity in both {\em tracking modality} 
(active + passive) and {\em fusion methodology} (algorithmic + data-driven) for accurate, 
robust, and scalable tracking in everyday environments (\S\ref{MOTIV}). \\
{\bf (2)} We design and build \system as an instantiation of our lightweight, yet robust and accurate framework that embodies the 
dual-layer diversity approach to fuse visual and RF sensing (\S\ref{DESIGN}). \\
{\bf (3)} We comprehensively evaluate and showcase the benefits of \system-style fusion models that enable both robustness and real-time operation\footnote{A real-time demo of \system can be found here~\cite{video-link}. We also plan to release our dataset (UWB, Camera and RFID) streams for the localization community to foster this line of research in UWB+VO based tracking.} (\S\ref{EVAL}).%, paving the way for immersive multi-agent applications in every-day environments (\S~\ref{EVAL}).

==> motivation.tex <==
\subsection{Background}
\% Cover related work and technical gaps as part of background description.
\subsubsection{Active Tracking}
\subsubsection{Passive Tracking} 
\subsubsection{Choice of Tracking Techniques}
\% Comparison between different visual tracking algorithms and our eventual choice. For RF tracking, we can qualitatively  motivate the choice of UWB based on its favorable range/NLOS-accuracy tradeoff (with simple graphs). 

\subsection{Motivation}
\subsubsection{Case for a Hybrid Approach}
\% Results to motivate deficiencies of isolated passive and active tracking approaches. 

\subsubsection{Role of Algorithm-assisted Learning}
\% Results to motivate deficiencies of a pure learning or algorithmic approach.

